Enabling Efficient and Scalable DRAM Read Disturbance Mitigation via New Experimental Insights into Modern DRAM Chips

Increasing storage density exacerbates DRAM read disturbance, a circuit-level vulnerability exploited by system-level attacks. Unfortunately, existing defenses are either ineffective or prohibitively expensive. Efficient mitigation is critical to ensure robust (reliable, secure, and safe) execution in future DRAM-based systems. This dissertation tackles two problems: 1) protecting DRAM-based systems becomes more expensive as technology scaling increases read disturbance vulnerability, and 2) many existing solutions depend on proprietary knowledge of DRAM internals. First, we build a detailed understanding of DRAM read disturbance by rigorously characterizing off-the-shelf modern DRAM chips under varying 1) temperatures, 2) memory access patterns, 3) in-chip locations, and 4) voltage. Our novel observations demystify the implications of large DRAM read disturbance variation on future DRAM read disturbance attacks and solutions. Second, we propose new mechanisms that mitigate read disturbance bitflips efficiently and scalably by leveraging insights into DRAM chip design: 1) subarray-level parallelism and 2) variation in read disturbance across DRAM rows in off-the-shelf DRAM chips. Third, we propose a novel solution that mitigates DRAM read disturbance by selectively throttling unsafe memory accesses that might otherwise cause read disturbance bitflips without proprietary knowledge of DRAM chip internals. We demonstrate that it is possible to mitigate DRAM read disturbance efficiently and scalably with worsening DRAM read disturbance by 1) building a detailed understanding of DRAM read disturbance, 2) leveraging insights into DRAM chips, and 3) devising novel solutions that do not require proprietary knowledge of DRAM chip internals. Our experimental insights and solutions enable future works targeting robust memory systems.

==> mainmatter/05_hammerdimmer/09_related_work.tex <==
\section{Related Work}
\label{hammerdimmer:sec:related_work}
{{To our knowledge, this} is the first work that 
{experimentally studies how reducing {wordline voltage} affects a real DRAM chip's 1)~}RowHammer vulnerability{, 2)~row activation latency, 3)~charge restoration process, and 4)~data retention time.}~{We divide prior work into {three} categories: 1)~{explorations} of reduced-voltage DRAM operation, 2)~experimental characterization studies {of the} RowHammer vulnerability of real DRAM chips, {{and}} 3)~RowHammer attacks and defenses.}
}


{\head{Reduced-Voltage DRAM {Operation}}~Prior works~\cite{david2011memory, deng2011memscale, chang2017understanding} propose operating DRAM {with} reduced \gls{vdd} to improve energy efficiency. {\cite{david2011memory} and \cite{deng2011memscale} propose dynamic voltage and frequency scaling (DVFS) {for DRAM chips} and \cite{david2011memory} provides results in a real system.}
{\cite{chang2017understanding} proposes to scale down \gls{vdd} without reducing DRAM chip frequency. To do so, \cite{chang2017understanding} experimentally demonstrates the interaction between \gls{vdd} and DRAM row access latency in real DDR3 DRAM chips.}
{These three works neither focus on the RowHammer vulnerability nor distinguish {between} \gls{vdd} and \gls{vpp}.} {Unlike {these works}, w}e focus on the impact of \gls{vpp} (isolated from \gls{vdd}) on RowHammer {and reliable operation} characteristics of real DDR4 DRAM chips.}

{\head{{Experimental} RowHammer Characterization} Prior work{s} extensively characterize the RowHammer vulnerability in real DRAM chips\cite{orosa2021adeeper, hassan2021uncovering,kim2020revisiting, kim2014flipping, park2016experiments, frigo2020trrespass}. These works {experimentally demonstrate {(}using real DDR3, DDR4, and LPDDR4 DRAM chips how{)} a DRAM chip's RowHammer vulnerability varies with}
1)~DRAM refresh rate~\cite{hassan2021uncovering,frigo2020trrespass,kim2014flipping}, 2)~the physical distance between aggressor and victim rows~\cite{kim2014flipping,kim2020revisiting}, 3)~DRAM generation and technology node~\cite{orosa2021adeeper,kim2014flipping,kim2020revisiting,hassan2021uncovering}, 4)~temperature~\cite{orosa2021adeeper,park2016experiments}, 5)~the time the aggressor row stays active~\cite{orosa2021adeeper,park2016experiments}, and~6)~physical location of the victim DRAM cell~\cite{orosa2021adeeper}. {N}one of these works analyze how reduced \gls{vpp} {affects} RowHammer vulnerability in real DRAM chips. Our characterization study furthers the analyses in these works by uncovering new insights into RowHammer behavior {and DRAM operation}.}


{\head{RowHammer Attacks and Defenses} 
{Many} prior works~\cite{seaborn2015exploiting, vanderveen2016drammer_deterministic, gruss2016rowhammerjs_a, razavi2016flip, pessl2016drama_exploiting, xiao2016onebit, bosman2016dedup, bhattacharya2016curious, qiao2016anew, jang2017sgxbomb, aga2017when, mutlu2017therowhammer, tatar2018defeating ,gruss2018another, lipp2018nethammer, vanderveen2018guardion, frigo2018grand, cojocar2019exploiting,  ji2019pinpoint, mutlu2019rowhammer_and, hong2019terminal, kwong2020rambleed, frigo2020trrespass, cojocar2020arewe, weissman2020jackhammer, zhang2020pthammer, safari2014rowhammer, yao2020deephammer, deridder2021smash, hassan2021uncovering, jattke2022blacksmith, marazzi2022rega, tol2022toward,burleson2016invited, brasser2017cant,qureshi2021rethinking, orosa2021adeeper, redeker2002aninvestigation, saroiu2022theprice, yang2019trapassisted, walker2021ondram, park2016statistical, kim2020revisiting, kim2014flipping, park2016experiments} show that RowHammer can be exploited to mount system-level attacks to compromise system security {and safety} (e.g., to acquire root privileges {or leak private data}).
To protect against these attacks,
{many prior works~\cite{aichinger2015ddrmemory, apple2015about, aweke2016anvil, kim2014flipping, kim2014architectural,son2017making, lee2019twice, you2019mrloc, seyedzadeh2018mitigating, vanderveen2018guardion, konoth2018zebram, park2020graphene, yaglikci2021blockhammer, kang2020cattwo, bains2015rowhammer, bains2016distributed, bains2016rowhammer, brasser2017cant, gomez2016dram_rowhammer, jedec2020jesd794c,hassan2019crow, devaux2021method, ryu2017overcoming, yang2016suppression, yang2017scanning, gautam2019rowhammering, yaglikci2021security, qureshi2021rethinking, greenfield2012throttling, marazzi2022rega, saileshwar2022randomized} propose RowHammer mitigation {mechanisms} that prevent RowHammer bitflips from compromising a system.}
The novel observations {we make in this work} can be leveraged to reduce RowHammer vulnerability {and} complement existing RowHammer defense mechanisms{,} further increasing their effectiveness and reducing their overheads.
}




==> mainmatter/05_hammerdimmer/11_acknowledgements.tex <==
\section*{Acknowledgments}
We thank our shepherd Karthik Pattabiraman and the anonymous reviewers of DSN~2022 for valuable feedback. We thank the SAFARI Research Group members for valuable feedback and the stimulating intellectual environment they provide. We acknowledge the generous gifts provided by our industrial partners{, including} Google, Huawei, Intel, Microsoft, and VMware{, and support from {the} Microsoft Swiss Joint Research Center}. 


==> mainmatter/05_hammerdimmer/glossary.tex <==
\usepackage{glossaries}

\newacronym{vdd}{$V_{DD}$}{supply voltage}
\newacronym{vpp}{$V_{PP}$}{wordline voltage}
\newacronym{vppmin}{$V_{PPmin}$}{the lowest \gls{vpp} at which the DRAM module can successfully communicate with the FPGA}
\newacronym{vwl}{$V_{PP}$}{wordline voltage}
\newacronym{gnd}{$GND$}{ground}
\newacronym{hcfirst}{$HC_{first}$}{the minimum hammer count \mpo{necessary} to cause a RowHammer bitflip}
\newacronym{rblast}{$r_{Blast}$}{blast radius}
\newacronym{ber}{$BER$}{the fraction of DRAM cells that experience a bitflip in a DRAM row}
\newacronym{nhc}{$N_{HC}$}{hammer count}
\newacronym{hc}{$HC$}{hammer count}
\newacronym{trcd}{$t_{RCD}$}{row activation latency}
\newacronym{tcl}{$t_{CL}$}{column access latency}
\newacronym{tcwl}{$t_{CWL}$}{column write latency}
\newacronym{trp}{$t_{RP}$}{precharge latency}
\newacronym{trcdmin}{$t_{RCDmin}$}{\agycrone{the minimum time delay \omtwo{required}}}
\newacronym{tras}{$t_{RAS}$}{charge restoration latency}
\newacronym{trasmin}{$t_{RASmin}$}{the minimum latency required}
\newacronym{trefw}{$t_{REFW}$}{refresh window}
\newacronym{vgs}{$V_{GS}$}{gate-to-source voltage}
\newacronym{vthresh}{$V_{TH}$}{the voltage threshold that the bitline voltage should exceed for the activation to be reliably completed}
\newacronym{kde}{KDE}{kernel density estimate}
\newacronym{ref}{refresh}{$REF$}

==> mainmatter/05_hammerdimmer/key_results.tex <==
\newcommand{\berdecravg}{\SI{15.2}{\percent}}
\newcommand{\berincravg}{\SI{-15.2}{\percent}}
\newcommand{\berdecrmax}{\SI{66.9}{\percent}}
\newcommand{\berincrmax}{\SI{11.7}{\percent}}

\newcommand{\hcfirstdecravg}{\SI{-7.4}{\percent}}
\newcommand{\hcfirstincravg}{\SI{7.4}{\percent}}
\newcommand{\hcfirstdecrmax}{\SI{9.1}{\percent}}
\newcommand{\hcfirstincrmax}{\SI{85.8}{\percent}}

\newcommand{\fracbersupportingrows}{\SI{81.2}{\percent}}
\newcommand{\fracberopposingrows}{\SI{15.4}{\percent}}
\newcommand{\fracbersmallchangerowsmfrA}{\SI{49.6}{\percent}}
\newcommand{\fracbersupportingrowsmfrA}{\SI{68.6}{\percent}}
\newcommand{\fracbersmallchangerowsmfrB}{\SI{17.0}{\percent}}
\newcommand{\fracbersupportingrowsmfrB}{\SI{75.0}{\percent}}
\newcommand{\fracbersmallchangerowsmfrC}{\SI{0.0}{\percent}}
\newcommand{\fracbersupportingrowsmfrC}{\SI{100.0}{\percent}}
\newcommand{\frachcfirstsupportingrows}{\SI{69.3}{\percent}}
\newcommand{\frachcfirstopposingrows}{\SI{14.2}{\percent}}
\newcommand{\frachcfirstsmallchangerowsmfrA}{\SI{27.1}{\percent}}
\newcommand{\frachcfirstsupportingrowsmfrA}{\SI{50.9}{\percent}}
\newcommand{\frachcfirstsmallchangerowsmfrB}{\SI{12.2}{\percent}}
\newcommand{\frachcfirstsupportingrowsmfrB}{\SI{73.5}{\percent}}
\newcommand{\frachcfirstsmallchangerowsmfrC}{\SI{7.0}{\percent}}
\newcommand{\frachcfirstsupportingrowsmfrC}{\SI{83.5}{\percent}}
\newcommand{\bersmallchange}{\SI{2}{\percent}}
\newcommand{\hcfirstsmallchange}{\SI{0}{\percent}}

\newcommand{\minnormbermfrA}{{0.43}}
\newcommand{\maxnormbermfrA}{{1.11}}
\newcommand{\minnormbermfrB}{{0.33}}
\newcommand{\maxnormbermfrB}{{1.03}}
\newcommand{\minnormbermfrC}{{0.74}}
\newcommand{\maxnormbermfrC}{{0.94}}
\newcommand{\minnormhcfirstmfrA}{{0.94}}
\newcommand{\maxnormhcfirstmfrA}{{1.52}}
\newcommand{\minnormhcfirstmfrB}{{0.92}}
\newcommand{\maxnormhcfirstmfrB}{{1.86}}
\newcommand{\minnormhcfirstmfrC}{{0.91}}
\newcommand{\maxnormhcfirstmfrC}{{1.35}}

\renewcommand{\numchips}{272}
\newcommand{\numreliablechips}{208}
\newcommand{\numunreliablechips}{64}
\newcommand{\numunreliablemodules}{5}
\newcommand{\numreliablemodules}{25}
\renewcommand{\nummodules}{30}
\newcommand{\trcdguardbandreduction}{\SI{21.9}{\percent}}
\newcommand{\trcdguardbandreduced}{\SI{34.1}{\percent}}

==> mainmatter/05_hammerdimmer/macros.tex <==
% Color Definitions
% \usepackage[dvipsnames]{xcolor}
\usepackage{xcolor}
\definecolor{darkamber}{rgb}{0.6, 0.4, 0.0}
\definecolor{amber}{rgb}{1.0, 0.49, 0.0}
\definecolor{dkgreen}{rgb}{0.0,0.6,0.0}
\definecolor{gray}{rgb}{0.5,0.5,0.5}
\definecolor{dkgray}{rgb}{0.3,0.3,0.3}
\definecolor{mauve}{rgb}{0.58,0,0.82}
\definecolor{lightmauve}{rgb}{0.68,0.4,0.92}
\definecolor{chocolate}{rgb}{0.48, 0.25, 0.0}
\definecolor{amber}{rgb}{1.0,0.75,0}
\definecolor{dollarbill}{rgb}{0.52,0.73,0.4}
\definecolor{dkdkgreen}{rgb}{0,0.45,0}
\definecolor{gfored}{rgb}{0.580, 0.050, 0.211}
\definecolor{darkwarmgray}{rgb}{0.15, 0.050, 0.05}
\definecolor{ups-truck}{rgb}{0.53, 0.28, 0.21}
\definecolor{moegi}{rgb}{0.357, 0.537, 0.188}
\definecolor{darkcerulean}{rgb}{0.03, 0.27, 0.49}

\newif\ifrevision
\revisiontrue

\newif\ifcrone
\cronefalse

\newif\ifcrtwo
\crtwofalse

\newif\ifcrthree
\crthreefalse

\newif\ifcrfour
\crfourfalse

\newif\ifcrfive
\crfivefalse

\newif\ifcrsix
\crsixfalse

\newif\ifextone
\extonefalse

\newif\ifexttwo
\exttwofalse

\newif\ifextthree
\extthreefalse

\newif\ifonurready
\onurreadytrue

\ifonurready
    \definecolor{darkamber}{rgb}{0.2, 0.2, 1.0}
    \definecolor{amber}{rgb}{0.2, 0.2, 1.0}
    \definecolor{dkgreen}{rgb}{0.2, 0.2, 1.0}
    \definecolor{gray}{rgb}{0.2, 0.2, 1.0}
    \definecolor{dkgray}{rgb}{0.2, 0.2, 1.0}
    \definecolor{mauve}{rgb}{0.2, 0.2, 1.0}
    \definecolor{lightmauve}{rgb}{0.2, 0.2, 1.0}
    \definecolor{chocolate}{rgb}{0.2, 0.2, 1.0}
    \definecolor{amber}{rgb}{0.2, 0.2, 1.0}
    \definecolor{dollarbill}{rgb}{0.2, 0.2, 1.0}
    \definecolor{dkdkgreen}{rgb}{0.2, 0.2, 1.0}
    \definecolor{gfored}{rgb}{0.2, 0.2, 1.0}
    \definecolor{darkwarmgray}{rgb}{0.2, 0.2, 1.0}
    \definecolor{ups-truck}{rgb}{0.2, 0.2, 1.0}
    \definecolor{moegi}{rgb}{0.2, 0.2, 1.0}
    \definecolor{darkcerulean}{rgb}{0.2, 0.2, 1.0}
\fi

\newcommand{\gfrev}[1]{{#1}}
\newcommand{\agyrev}[1]{{#1}}
\newcommand{\agyrevtwo}[1]{{#1}}
\newcommand{\agycrone}[1]{#1}
\newcommand{\agycronecomment}[1]{}
\newcommand{\hluocrone}[1]{#1}
\newcommand{\hluocronecomment}[1]{}
\newcommand{\omone}[1]{#1}
\newcommand{\omonecomment}[1]{}
\newcommand{\gfo}[1]{#1}
\newcommand{\gfocomment}[1]{}
\newcommand{\mpo}[1]{{#1}}
\newcommand{\atbcrcomment}[1]{}
\newcommand{\mpcronecomment}[1]{}
\newcommand{\hhone}[1]{#1}

\newcommand{\atbcrtwo}[1]{#1}
\newcommand{\agycrtwo}[1]{#1}
\newcommand{\hluocrtwo}[1]{#1}
\newcommand{\omtwo}[1]{#1}
\newcommand{\gfii}[1]{#1}
\newcommand{\gft}[1]{#1}
\newcommand{\mpt}[1]{{#1}}
\newcommand{\hhtwo}[1]{#1}

\newcommand{\agycrtwocomment}[1]{}
\newcommand{\hluocrtwocomment}[1]{}
\newcommand{\omtwocomment}[1]{}
\newcommand{\gftcomment}[1]{}
\newcommand{\atbcrtwocomment}[1]{}
\newcommand{\mpcrtwocomment}[1]{}
\newcommand\gfb[1][0]{}

\newcommand{\agycrthree}[1]{#1}
\newcommand{\agycrthreecomment}[1]{}
\newcommand{\omthree}[1]{#1}
\newcommand{\omthreecomment}[1]{}
\newcommand{\mpcrthree}[1]{#1}
\newcommand{\mpcrfour}[1]{#1}

\newcommand{\agycrfour}[1]{#1}
\newcommand{\agycrfourcomment}[1]{}
\newcommand{\omfour}[1]{#1}
\newcommand{\omfourcomment}[1]{}

\newcommand{\agycrfive}[1]{#1}
\newcommand{\agycrfivecomment}[1]{}
\newcommand{\mpcrfive}[1]{#1}
\newcommand{\mpcrfivecomment}[1]{}
\newcommand{\omfive}[1]{#1}
\newcommand{\omfivecomment}[1]{}

\newcommand{\agycrsix}[1]{#1}
\newcommand{\agycrsixcomment}[1]{}
\newcommand{\mpcrsix}[1]{#1}
\newcommand{\mpcrsixcomment}[1]{}
\newcommand{\omsix}[1]{#1}
\newcommand{\omsixcomment}[1]{}

\newcommand{\agyextone}[1]{#1}
\newcommand{\hluoextone}[1]{#1}
\newcommand{\agyextonecomment}[1]{}
\newcommand{\mpextone}[1]{#1}
\newcommand{\mpextonecomment}[1]{}
\newcommand{\omextone}[1]{#1}
\newcommand{\omextonecomment}[1]{}

\newcommand{\agyexttwo}[1]{#1}
\newcommand{\hluoexttwo}[1]{#1}
\newcommand{\agyexttwocomment}[1]{}
\newcommand{\mpexttwo}[1]{#1}
\newcommand{\mpexttwocomment}[1]{}
\newcommand{\omexttwo}[1]{#1}
\newcommand{\omexttwocomment}[1]{}

\newcommand{\agyextthree}[1]{#1}
\newcommand{\hluoextthree}[1]{#1}
\newcommand{\agyextthreecomment}[1]{}
\newcommand{\mpextthree}[1]{#1}
\newcommand{\mpextthreecomment}[1]{}
\newcommand{\omextthree}[1]{#1}
\newcommand{\omextthreecomment}[1]{}

%%% Put CamReady First Round coloring here %%%

\ifextthree
  \renewcommand{\mpextthree}[1]{\textcolor{blue}{#1}}
  \renewcommand{\agyextthree}[1]{\textcolor{blue}{#1}}
  \renewcommand{\hluoextthree}[1]{\textcolor{blue}{#1}}
  \renewcommand{\agyextthreecomment}[1]{\todo[linecolor=green,backgroundcolor=green!25,bordercolor=green, size=\tiny]{\textbf{@gy:} #1}}
  \renewcommand{\omextthree}[1]{\textcolor{gfored}{#1}}
  \renewcommand{\omextthreecomment}[1]{\todo[linecolor=red,backgroundcolor=red!25,bordercolor=red, size=\tiny]{\textbf{@om:} #1}}
\fi

\ifexttwo
  \renewcommand{\mpexttwo}[1]{\textcolor{blue}{#1}}
  \renewcommand{\agyexttwo}[1]{\textcolor{blue}{#1}}
  \renewcommand{\hluoexttwo}[1]{\textcolor{blue}{#1}}
  \renewcommand{\agyexttwocomment}[1]{\todo[linecolor=green,backgroundcolor=green!25,bordercolor=green, size=\tiny]{\textbf{@gy:} #1}}
  \renewcommand{\omexttwo}[1]{\textcolor{gfored}{#1}}
  \renewcommand{\omexttwocomment}[1]{\todo[linecolor=red,backgroundcolor=red!25,bordercolor=red, size=\tiny]{\textbf{@om:} #1}}
\fi

\ifextone
  \renewcommand{\mpextone}[1]{\textcolor{blue}{#1}}
  \renewcommand{\agyextone}[1]{\textcolor{blue}{#1}}
  \renewcommand{\hluoextone}[1]{\textcolor{blue}{#1}}
  \renewcommand{\agyextonecomment}[1]{\todo[linecolor=green,backgroundcolor=green!25,bordercolor=green, size=\tiny]{\textbf{@gy:} #1}}
  \renewcommand{\omextone}[1]{\textcolor{gfored}{#1}}
  \renewcommand{\omextonecomment}[1]{\todo[linecolor=red,backgroundcolor=red!25,bordercolor=red, size=\tiny]{\textbf{@om:} #1}}
\fi

\ifcrsix
  \renewcommand{\mpcrsix}[1]{\textcolor{blue}{#1}}
  \renewcommand{\agycrsix}[1]{\textcolor{blue}{#1}}
  \renewcommand{\agycrsixcomment}[1]{\todo[linecolor=green,backgroundcolor=green!25,bordercolor=green, size=\tiny]{\textbf{@gy:} #1}}
  \renewcommand{\omsix}[1]{\textcolor{gfored}{#1}}
  \renewcommand{\omsixcomment}[1]{\todo[linecolor=red,backgroundcolor=red!25,bordercolor=red, size=\tiny]{\textbf{@om:} #1}}
\fi


\ifcrfive
  \renewcommand{\mpcrfive}[1]{\textcolor{blue}{#1}}
  \renewcommand{\agycrfive}[1]{\textcolor{blue}{#1}}
  \renewcommand{\agycrfivecomment}[1]{\todo[linecolor=green,backgroundcolor=green!25,bordercolor=green, size=\tiny]{\textbf{@gy:} #1}}
  \renewcommand{\omfive}[1]{\textcolor{gfored}{#1}}
  \renewcommand{\omfivecomment}[1]{\todo[linecolor=red,backgroundcolor=red!25,bordercolor=red, size=\tiny]{\textbf{@om:} #1}}
\fi


\ifcrfour
  \renewcommand{\mpcrfour}[1]{\textcolor{blue}{#1}}
  \renewcommand{\agycrfour}[1]{\textcolor{blue}{#1}}
  \renewcommand{\agycrfourcomment}[1]{\todo[linecolor=green,backgroundcolor=green!25,bordercolor=green, size=\tiny]{\textbf{@gy:} #1}}
  \renewcommand{\omfour}[1]{\textcolor{gfored}{#1}}
  \renewcommand{\omfourcomment}[1]{\todo[linecolor=red,backgroundcolor=red!25,bordercolor=red, size=\tiny]{\textbf{@om:} #1}}
\fi


\ifcrthree
  \renewcommand{\mpcrthree}[1]{\textcolor{blue}{#1}}
  \renewcommand{\agycrthree}[1]{\textcolor{blue}{#1}}
  \renewcommand{\agycrthreecomment}[1]{\todo[linecolor=green,backgroundcolor=green!25,bordercolor=green, size=\tiny]{\textbf{@gy:} #1}}
  \renewcommand{\omthree}[1]{\textcolor{gfored}{#1}}
  \renewcommand{\omthreecomment}[1]{\todo[linecolor=red,backgroundcolor=red!25,bordercolor=red, size=\tiny]{\textbf{@om:} #1}}
\fi


\ifcrone
\renewcommand{\agycrone}[1]{\textcolor{blue}{#1}}
\renewcommand{\agycronecomment}[1]{\todo[linecolor=green,backgroundcolor=green!25,bordercolor=green, size=\tiny]{\textbf{@gy:} #1}}
\renewcommand{\gfo}[1]{\textcolor{blue}{#1}}
\renewcommand{\hhone}[1]{\textcolor{blue}{#1}}
\renewcommand{\gfocomment}[1]{\todo[linecolor=green,backgroundcolor=green!25,bordercolor=green, size=\tiny]{\textbf{@gy:} #1}}
\renewcommand{\hluocrone}[1]{{\textcolor{moegi}{#1}}}
\renewcommand{\hluocronecomment}[1]{\todo[linecolor=blue,backgroundcolor=blue!25,bordercolor=blue, size=\tiny]{\textbf{@hluo:} #1}}
\renewcommand{\omone}[1]{\textcolor{blue}{#1}}
\renewcommand{\omonecomment}[1]{\todo[linecolor=red,backgroundcolor=red!25,bordercolor=red, size=\tiny]{\textbf{@om:} #1}}
\renewcommand{\atbcrcomment}[1]{\todo[linecolor=gray,backgroundcolor=gray!25,bordercolor=gray, size=\tiny]{\textbf{@atb:} #1}}
\renewcommand{\mpcronecomment}[1]{\todo[linecolor=amber,backgroundcolor=amber!25,bordercolor=amber, size=\tiny]{Minesh: #1}}
\renewcommand{\mpo}[1]{\textcolor{darkamber}{#1}}
\fi

%%% Put CamReady First Round coloring here %%%
\ifcrtwo
\renewcommand{\agycrtwo}[1]{\textcolor{blue}{#1}}
\renewcommand{\atbcrtwo}[1]{\textcolor{darkamber}{#1}}
\renewcommand{\gft}[1]{\textcolor{blue}{#1}}
\renewcommand{\hhtwo}[1]{\textcolor{blue}{#1}}
\renewcommand{\gftcomment}[1]{\todo[linecolor=green,backgroundcolor=green!25,bordercolor=green, size=\tiny]{\textbf{@gf:} #1}}
\renewcommand{\hluocrtwo}[1]{{\textcolor{moegi}{#1}}}
\renewcommand{\hluocrtwocomment}[1]{\todo[linecolor=blue,backgroundcolor=blue!25,bordercolor=blue, size=\tiny]{\textbf{@hluo:} #1}}
\renewcommand{\omtwo}[1]{\textcolor{gfored}{#1}}
\renewcommand{\gfii}[1]{\textcolor{gfored}{#1}}

\renewcommand{\omtwocomment}[1]{\todo[linecolor=red,backgroundcolor=red!25,bordercolor=red, size=\tiny]{\textbf{@om:} #1}}
\renewcommand{\agycrtwocomment}[1]{\todo[linecolor=green,backgroundcolor=green!25,bordercolor=green, size=\tiny]{\textbf{@gy:} #1}}


\renewcommand{\atbcrcomment}[1]{\todo[linecolor=gray,backgroundcolor=gray!25,bordercolor=gray, size=\tiny]{\textbf{@atb:} #1}}
\renewcommand{\mpcrtwocomment}[1]{\todo[linecolor=amber,backgroundcolor=amber!25,bordercolor=amber, size=\tiny]{Minesh: #1}}
\renewcommand{\mpt}[1]{\textcolor{darkamber}{#1}}

\renewcommand{\gfb}[1]{[{\color{red}GF: #1}]}

\fi


%%% Put REVISION coloring here %%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\ifrevision
\renewcommand{\gfrev}[1]{\textcolor{blue}{#1}}
\renewcommand{\agyrev}[1]{\textcolor{blue}{#1}}
% \renewcommand{\agyrevtwo}[1]{\textcolor{dkdkgreen}{#1}}

\fi

\newif\ifdraft
\draftfalse

\newcommand{\N}{\textcolor{red}{N}}
\newcommand{\inherited}[1]{{#1}}
\newcommand{\td}[1]{}
\newcommand{\head}[1]{\noindent\textbf{#1.}} 

\newcommand{\todot}[1]{\textcolor{red}{#1}}
\newcommand{\param}[1]{{#1}}
\newcommand{\atb}[1]{{#1}}
\newcommand{\agy}[1]{{#1}}
\newcommand{\agycomment}[1]{}
\newcommand{\js}[1]{{#1}}
\newcommand{\jsc}[1]{{#1}}
\newcommand{\gf}[1]{{#1}}
\newcommand{\hluo}[1]{{#1}}
\newcommand{\hluocomment}[1]{}

% \renewcommand{\mpo}[1]{\textcolor{darkamber}{#1}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% Put DRAFT coloring here %%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\ifdraft
\renewcommand{\param}[1]{\textcolor{red}{#1}}
\renewcommand{\atb}[1]{\textcolor{ups-truck}{#1}}
\renewcommand{\agy}[1]{\textcolor{gfored}{#1}}
\renewcommand{\agycomment}[1]{\textcolor{gfored}{\textbf{[@gy:}#1\textbf{]}}}
\renewcommand{\js}[1]{\textcolor{darkamber}{#1}}
\renewcommand{\jsc}[1]{\js{[\textit{\textbf{JS:} #1}]}}
\renewcommand{\gf}[1]{\textcolor{blue}{#1}}
\renewcommand{\inherited}[1]{\textcolor{dkgray}{#1}}
\renewcommand{\td}[1]{\textcolor{gfored}{\textbf{[TODO:}#1\textbf{]}}}
\renewcommand{\hluo}[1]{{\textcolor{moegi}{#1}}}
\renewcommand{\hluocomment}[1]{\textcolor{moegi}{\textbf{[@hluo: }#1\textbf{]}}}
\fi
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% MINESH: versioning
\usepackage{tikz}
\usepackage{fancyhdr}
\usepackage{datetime} 

\settimeformat{ampmtime}

\newif\ifuseversions
\ifdraft
\useversionstrue
\fi
\newcommand{\versionnum}[0]{1.5}
\ifuseversions
  \def\parsepdfdatetime#1:#2#3#4#5#6#7#8#9{%
    \def\theyear{#2#3#4#5}%
    \def\themonth{#6#7}%
    \def\theday{#8#9}%
    \parsepdftime
  }

  \def\parsepdftime#1#2#3#4#5#6#7\endparsepdfdatetime{%
    \def\thehour{#1#2}%
    \def\theminute{#3#4}%
    \def\thesecond{#5#6}%
    \ifstrequal{#7}{Z}
    {%
      \def\thetimezonehour{+00}%
      \def\thetimezoneminute{00}%
    }%
    {%
      \parsepdftimezone#7%
    }%
  }

  \def\parsepdftimezone#1'#2'{%
    \def\thetimezonehour{#1}%
    \def\thetimezoneminute{#2}%
  }

  \newcommand*{\thetimezone}{\thetimezonehour:\thetimezoneminute}
  \expandafter\parsepdfdatetime\pdfcreationdate\endparsepdfdatetime

  \settimeformat{ampmtime}
  \newcommand{\version}[1]{\emph{Version #1 (Built:~\today~@ \currenttime~UTC\thetimezone)}}
  \AtBeginShipout
  {\AtBeginShipoutAddToBox{
      \begin{tikzpicture}[overlay, remember picture]
      \node[anchor=north] at (current page.north) {\textcolor{blue}{\vspace{3em}\version{\versionnum}}};    
      \end{tikzpicture}
  }}
\fi

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Cross-references
\newcommand{\figref}[1]{Fig.~\ref{#1}}
\newcommand{\secref}[1]{§\ref{#1}}
\newcommand{\secsref}[1]{§§{#1}}
\newcommand{\obsvref}[1]{Obsv.~\ref{#1}}
\newcommand{\obsvsref}[1]{Obsvs.~\ref{#1}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Observations
\newcounter{obs}
\setcounter{obs}{0}
\newcommand\observation[1]{%
   %\leavevmode\par
   %\stepcounter{obs}
   \refstepcounter{obs}
   \noindent
   \textbf{Observation \theobs.} \emph{#1}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%% Squished List
\newcommand{\squishlist}{
 \begin{list}{$\circ$}
  { \setlength{\itemsep}{0pt}
     \setlength{\parsep}{0pt}
     \setlength{\topsep}{0pt}
     \setlength{\partopsep}{0pt}
     \setlength{\leftmargin}{1em}
     \setlength{\labelwidth}{1em}
     \setlength{\labelsep}{0.5em} } }
\newcommand{\squishsublist}{
\begin{list}{$\rightarrow$}
 { \setlength{\itemsep}{0pt}
    \setlength{\parsep}{0pt}
    \setlength{\topsep}{-10em}
    \setlength{\partopsep}{-3pt}
    \setlength{\leftmargin}{1em}
    \setlength{\labelwidth}{1em}
    \setlength{\labelsep}{0.5em} } }
\newenvironment{squishenum}
{\begin{enumerate}[leftmargin=*]
  \setlength{\itemsep}{0em}
  \setlength{\parskip}{0pt}
  \setlength{\parsep}{0pt}
  \setlength{\topsep}{3pt}
  \setlength{\partopsep}{0pt}}
{\end{enumerate}}
\newcommand{\squishend}{
  \end{list}  }
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%% Figure Margins
\makeatletter
\g@addto@macro{\normalsize}{%
  \setlength{\abovedisplayskip}{2pt plus 1pt minus 1pt}
  \setlength{\belowdisplayskip}{2pt plus 1pt minus 1pt}
  \setlength{\abovedisplayshortskip}{0pt}
  \setlength{\belowdisplayshortskip}{0pt}
  \setlength{\intextsep}{2pt plus 1pt minus 1pt}
  \setlength{\textfloatsep}{3pt plus 1pt minus 1pt}
  \setlength{\dbltextfloatsep}{3pt plus 1pt minus 1pt}
  \setlength{\skip\footins}{4pt plus 1pt minus 1pt}}
  \setlength{\abovecaptionskip}{2pt plus 1pt minus 1pt}
\makeatother
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommandx{\unsure}[2][1=]{\todo[linecolor=red,backgroundcolor=red!25,bordercolor=red,#1, size=\tiny]{#2}}
 \newcommandx{\change}[2][1=]{\todo[linecolor=blue,backgroundcolor=blue!25,bordercolor=blue,#1,size=\scriptsize]{#2}}
 \newcommandx{\feedback}[2][1=]{\todo[linecolor=yellow,backgroundcolor=yellow!25,bordercolor=yellow,#1]{#2}}
 \newcommandx{\improvement}[2][1=]{\todo[linecolor=Plum,backgroundcolor=Plum!25,bordercolor=Plum,#1]{#2}}
\newcommandx{\thiswillnotshow}[2][1=]{\todo[disable,#1]{#2}}
\newcommandx{\completedRevision}[2][1=]{\todo[disable,backgroundcolor=red,#1]{#2}}
\newcommandx{\dataSource}[2][1=]{\todo[disable,backgroundcolor=red,#1]{#2}}
 \newcommandx{\info}[2][1=]{\todo[linecolor=dollarbill,backgroundcolor=dollarbill!25,bordercolor=dollarbill,#1, size=\tiny]{#2}}


        
\definecolor{lightyellow}{rgb}{0.980, 0.956, 0.623}

\newcommand{\yboxbegin} {
	\begin{tcolorbox}[breakable, enhanced, frame hidden, colback=yellow!50]
}

\newcommand{\yboxend} {
	\end{tcolorbox}
}

\hyphenation{Row-Ham-mer mul-ti-pro-gram-med Block-Ham-mer Row-Ham-mer-induced Zeb-RAM per-for-mance}
\def\UrlBreaks{\do\/\do-\/\do.\/\do:}

\expandafter\def\expandafter\UrlBreaks\expandafter{\UrlBreaks
  \do\a\do\b\do\c\do\d\do\e\do\f\do\g\do\h\do\i\do\j
  \do\k\do\l\do\m\do\n\do\o\do\p\do\q\do\r\do\s\do\t
  \do\u\do\v\do\w\do\x\do\y\do\z\do\A\do\B\do\C\do\D
  \do\E\do\F\do\G\do\H\do\I\do\J\do\K\do\L\do\M\do\N
  \do\O\do\P\do\Q\do\R\do\S\do\T\do\U\do\V\do\W\do\X
  \do\Y\do\Z}

==> mainmatter/06_svard/glossary.tex <==
\newcommand{\hcfirst}[0]{HC_{first}}
\newacronym{hcfirst}{$\hcfirst$}{the minimum {hammer count} {required to induce the first bitflip}} 
% \newacronym{taggon}{$t_{AggOn}$}{the time period during which the aggressor row is kept active}
% \newacronym{nrh}{$N_{RH}$}{}
\newacronym{ber}{$BER$}{bit error rate}
\newacronym{wcdp}{$WCDP$}{worst-case data pattern}
\newcommand{\nummodules}{\param{15}}
\newcommand{\numchips}{\agy{2}{144}}
\newcommand{\numworkloadmixes}{\agy{4}{120}}
\newcommand{\wlcnt}{\numworkloadmixes{}}
\newacronym{taggon}{$t_{AggOn}$}{the time that an aggressor row stays active}
\newacronym{taggoff}{$t_{AggOff}$}{the time that an aggressor row stays precharged}
\newacronym{tras}{$t_{RAS}$}{charge restoration latency}
\newacronym{trp}{$t_{RP}$}{precharge latency}
\newcommand{\trc}[0]{t_{RC}}
\newacronym{trc}{$\trc{}$}{row activation cycle}
\newacronym{trcd}{$t_{RCD}$}{row activation latency}
\newacronym{tcl}{$t_{CL}$}{column access latency}
\newacronym{tcwl}{$t_{CWL}$}{column write latency}
\newcommand{\tfaw}[0]{t_{FAW}}
\newacronym{tfaw}{$\tfaw{}$}{four row activation window}
\newcommand{\trefw}[0]{t_{REFW}}
\newacronym{trefw}{$\trefw{}$}{refresh window}
\newcommand{\trefi}[0]{t_{REFI}}
\newacronym{trefi}{$\trefi{}$}{refresh interval}
\newacronym{trrslack}{$t_{RefSlack}$}{{the maximum delay between the time a {periodic}/{preventive} refresh is generated and the time the refresh is performed}}
\newacronym{tapa}{$t_{APA}$}{the latency of issuing $ACT-PRE-ACT$ command sequence}
\newacronym{ref}{$REF$}{refresh}
\newacronym{act}{$ACT$}{activate}
\newacronym{pre}{$PRE$}{precharge}
\newcommand{\trfc}[0]{t_{RFC}}
\newacronym{trfc}{$\trfc{}$}{refresh latency}
\newacronym{iqr}{$IQR$}{interquartile range}
\newacronym{cv}{$CV$}{the coefficient of variation}
\newacronym{hc}{$HC$}{hammer count}
\newcommand{\pth}[0]{p_{th}}
\newacronym{pth}{$\pth{}$}{{PARA's probability threshold}}
\newcommand{\pf}[0]{p_{failure}}
\newacronym{pf}{$\pf{}$}{failure probability over a sufficiently long time}
\newcommand{\prh}[0]{p_{RH}}
\newacronym{prh}{$\prh{}$}{reliability target for a \gls{trefw}}

\newcommand{\cchip}[0]{D_{chip}}
\newacronym{cchip}{$\cchip{}$}{chip density}

\newcommand{\rbcpki}[0]{RBCPKI}
\newacronym{rbcpki}{$\rbcpki{}$}{row buffer conflicts per kilo instruction}

\newcommand{\mpki}[0]{MPKI}
\newacronym{mpki}{$\mpki{}$}{misses per kilo instruction}

\newcommand{\vdd}[0]{V_{DD}}
\newacronym{vdd}{$\vdd{}$}{supply voltage}

\newcommand{\gnd}[0]{GND}
\newacronym{gnd}{$\gnd{}$}{ground}

\newcommand{\rd}[0]{RD}
\newacronym{rd}{$\rd{}$}{read}

\newcommand{\dramwr}[0]{WR}
\newacronym{wr}{$\dramwr{}$}{write}

==> mainmatter/06_svard/hpca-template.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%% -- DO NOT MODIFY -- %%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\author{
  \ifdefined\hpcacameraready
    \IEEEauthorblockN{\hpcaauthors{}}
      \IEEEauthorblockA{
        \hpcaaffiliation{} \\
        \hpcaemail{}
      }
  \else
    \IEEEauthorblockN{\normalsize{HPCA \hpcayear{} Submission
      \textbf{\#\hpcasubmissionnumber{}}} \\
      \IEEEauthorblockA{
        Confidential Draft \\
        Do NOT Distribute!!
      }
    }
  \fi 
}

% Heading and footer for title page
\fancypagestyle{camerareadyfirstpage}{%
  \fancyhead{}
  \renewcommand{\headrulewidth}{0pt}
  \fancyhead[C]{
    \ifdefined\aeopen
    \parbox[][12mm][t]{13.5cm}{\hpcayear{} IEEE International Symposium on High-Performance Computer Architecture (HPCA)}    
    \else
      \ifdefined\aereviewed
      \parbox[][12mm][t]{13.5cm}{\hpcayear{} IEEE International Symposium on High-Performance Computer Architecture (HPCA)}
      \else
      \ifdefined\aereproduced
      \parbox[][12mm][t]{13.5cm}{\hpcayear{} IEEE International Symposium on High-Performance Computer Architecture (HPCA)}
      \else
      \parbox[][0mm][t]{13.5cm}{\centering
      \hpcayear{} IEEE International Symposium on High-Performance Computer Architecture (HPCA)\\
      \textcolor{blue}{\textbf{Version~\theversion{}~---~\today, \ampmtime{}}}}
    \fi 
    \fi 
    \fi 
    \ifdefined\aeopen 
      \includegraphics[width=12mm,height=12mm]{ae-badges/open-research-objects.pdf}
    \fi 
    \ifdefined\aereviewed
      \includegraphics[width=12mm,height=12mm]{ae-badges/research-objects-reviewed.pdf}
    \fi 
    \ifdefined\aereproduced
      \includegraphics[width=12mm,height=12mm]{ae-badges/results-reproduced.pdf}
    \fi
  }
  %\fancyfoot[L]{\hpcapubid{} \copyright \hpcayear{} IEEE}
  \fancyfoot[C]{}
}
% Heading and footer for remaining pages
\fancyhead{}
\renewcommand{\headrulewidth}{0pt}
%\fancyhead[C]{\hpcayear{} IEEE International Symposium on
% High-Performance Computer Architecture (HPCA)}

% \renewcommand{\citepunct}{,\penalty\citepunctpenalty\,} \renewcommand{\citedash}{--}

\makeatletter
\def\bstctlcite{\@ifnextchar[{\@bstctlcite}{\@bstctlcite[@auxout]}}
\def\@bstctlcite[#1]#2{\@bsphack
 \@for\@citeb:=#2\do{%
   \edef\@citeb{\expandafter\@firstofone\@citeb}%
   \if@filesw\immediate\write\csname #1\endcsname{\string\citation{\@citeb}}\fi}%
 \@esphack}
\makeatother


  


==> mainmatter/06_svard/macros.tex <==
% \def\BibTeX{{\rm B\kern-.05em{\sc i\kern-.025em b}\kern-.08em
%     T\kern-.1667em\lower.7ex\hbox{E}\kern-.125emX}}

\renewcommand*{\glstextformat}[1]{\textcolor{black}{#1}}

\hyphenation{Row-Ham-mer mul-ti-pro-gram-med Block-Ham-mer Row-Ham-mer-induced Zeb-RAM per-for-mance}
\def\UrlBreaks{\do\/\do-\/\do.\/\do:}

\expandafter\def\expandafter\UrlBreaks\expandafter{\UrlBreaks
  \do\a\do\b\do\c\do\d\do\e\do\f\do\g\do\h\do\i\do\j
  \do\k\do\l\do\m\do\n\do\o\do\p\do\q\do\r\do\s\do\t
  \do\u\do\v\do\w\do\x\do\y\do\z\do\A\do\B\do\C\do\D
  \do\E\do\F\do\G\do\H\do\I\do\J\do\K\do\L\do\M\do\N
  \do\O\do\P\do\Q\do\R\do\S\do\T\do\U\do\V\do\W\do\X
  \do\Y\do\Z}
  
\lstset {     language=Matlab,
        basicstyle=\footnotesize,    numbers=left,
    xleftmargin=2em,
    frame=single,
    framexleftmargin=2em,
        keywordstyle     = \bfseries,
    identifierstyle  = \color{blue},
    commentstyle     = \color{olive},
    moredelim        = [s][\color{ForestGreen}]{/**}{*/},
    stringstyle      = \color{magenta},
    showstringspaces = false,
    columns          = fullflexible,
    escapechar       = {|}
}  

\definecolor{amber}{rgb}{1.0, 0.49, 0.0}
\definecolor{awesome}{rgb}{1.0, 0.13, 0.32}
\definecolor{dollarbill}{rgb}{0.52,0.73,0.4}
\definecolor{moegi}{rgb}{0.357, 0.537, 0.188}
\definecolor{burgundy}{rgb}{0.5, 0.0, 0.13}
\definecolor{ballblue}{rgb}{0.13, 0.67, 0.8}
\definecolor{ups-truck}{rgb}{0.53, 0.28, 0.21}
\definecolor{airforceblue}{rgb}{0.36, 0.54, 0.66}
\definecolor{cadmiumgreen}{rgb}{0.0, 0.42, 0.24}
\definecolor{darkcyan}{rgb}{0.0, 0.55, 0.55}
\definecolor{caribbeangreen}{rgb}{0.0, 0.8, 0.6}
\definecolor{flamingopink}{rgb}{0.99, 0.56, 0.67}
\definecolor{jazzberryjam}{rgb}{0.65, 0.04, 0.37}
\definecolor{mediumpersianblue}{rgb}{0.0, 0.4, 0.65}
\definecolor{coolblack}{rgb}{0.0, 0.18, 0.39}
\definecolor{bleudefrance}{rgb}{0.19, 0.55, 0.91}
\definecolor{ao}{rgb}{0.0, 0.0, 1.0}
\definecolor{babyblueeyes}{rgb}{0.63, 0.79, 0.95}
\definecolor{darkwarmgray}{rgb}{0.2,0,0}
\definecolor{brightpink}{rgb}{1.0, 0.0, 0.5}

\newcommand{\circled}[1]{{\tikz[baseline=(char.base)]{\node[shape=circle,inner sep=1pt,fill=black, text=white] (char) {\footnotesize \textbf{#1}};}}}
\newcommand{\circledletter}[1]{\tikz[baseline=(char.base)]{\node[shape=circle,inner sep=1pt,fill=black, text=white] (char) {\tiny \textbf{#1}};}}
\newcommand{\coloredcircledletter}[2]{\tikz[baseline=(char.base)]{\node[shape=circle,inner sep=1pt,fill=#1, text=white] (char) {\footnotesize \textbf{#2}};}}

\DeclareRobustCommand{\bgyellow}[1]{\textbf{{\sethlcolor{soulyellow}\hl{#1}}}}
\DeclareRobustCommand{\bgblue}[1]{\textbf{{\sethlcolor{babyblueeyes}\hl{#1}}}}
\DeclareRobustCommand{\bgred}[1]{\textbf{{\sethlcolor{red}\hl{#1}}}}
\DeclareRobustCommand{\bgpink}[1]{\textbf{{{\sethlcolor{flamingopink}{\hl{#1}}}}}}


\newcommand{\squishlist}{
 \begin{list}{$\circ$}
  { \setlength{\itemsep}{0pt}
     \setlength{\parsep}{0pt}
     \setlength{\topsep}{0pt}
     \setlength{\partopsep}{0pt}
     \setlength{\leftmargin}{1em}
     \setlength{\labelwidth}{1em}
     \setlength{\labelsep}{0.5em} } }

\newcommand{\squishsublist}{
\begin{list}{$\rightarrow$}
 { \setlength{\itemsep}{0pt}
    \setlength{\parsep}{0pt}
    \setlength{\topsep}{-10em}
    \setlength{\partopsep}{-3pt}
    \setlength{\leftmargin}{1em}
    \setlength{\labelwidth}{1em}
    \setlength{\labelsep}{0.5em} } }

\newenvironment{squishenum}
{\begin{enumerate}[leftmargin=*]
  \setlength{\itemsep}{0em}
  \setlength{\parskip}{0pt}
  \setlength{\parsep}{0pt}
  \setlength{\topsep}{3pt}
  \setlength{\partopsep}{0pt}}
{\end{enumerate}}

\newcommand{\squishend}{
  \end{list}  }

\newcommand{\head}[1]{\noindent\textbf{#1.}} 

\newcounter{obs}
\setcounter{obs}{0}
\newcommand\observation[1]{         \refstepcounter{obs}
   \noindent
   \colorbox{gray!20}{\textbf{Observation \theobs.}} \emph{#1}}
   
\newcounter{take}
\setcounter{take}{0}
\newcommand\takebox[1]{\refstepcounter{take}
    \begin{tcolorbox}[colback=white!25!white,colframe=black!65!white, arc=1pt, boxrule=0.5pt, left=2pt,right=2pt,top=0pt,bottom=0pt,  title=\textbf{{Takeaway \thetake.}}]
        \emph{{#1}}
   \end{tcolorbox}
}

\newcommand{\gf}[2]{\ifnum#1=\value{version}\textcolor{red}{#2}\else{#2}\fi}
\newcommand{\agy}[2]{\ifnum#1=\value{version}\textcolor{blue}{#2}\else{#2}\fi}
\newcommand{\yct}[2]{\ifnum#1=\value{version}\textcolor{purple}{#2}\else{#2}\fi}
\newcommand{\om}[2]{\ifnum#1=\value{version}\textcolor{red}{#2}\else#2\fi}
\newcommand{\agytodo}[2]{\ifnum#1=\value{version}\todo[size=\scriptsize, linecolor=orange, bordercolor=orange, backgroundcolor=white]{\textcolor{blue}{TODO:~#2}}\else{}\fi}
\newcommand{\agycomment}[2]{\ifnum#1=\value{version}\todo[size=\scriptsize, linecolor=orange, bordercolor=orange, backgroundcolor=white]{\textcolor{blue}{Giray:~#2}}\else{}\fi}
\newcommand{\omcomment}[2]{\ifnum#1=\value{version}\todo[size=\scriptsize, linecolor=orange, bordercolor=orange, backgroundcolor=white]{\textcolor{red}{Onur:~#2}}\else{}\fi}

% \newcommand{\omcomment}[2]{\ifnum#1=\value{version}\todo[size=\scriptsize, linecolor=orange, bordercolor=orange, backgroundcolor=white]{\textcolor{red}{Onur:~#2}}\else{}\fi}
\newcommand{\ominlinecomment}[2]{\ifnum#1=\value{version}{\textcolor{red}{\textbf{[Onur:}~#2\textbf{]}}}\else{}\fi}
\newcommand{\versionedparam}[2]{\ifnum#1=\value{version}\textcolor{red}{#2}\else{#2}\fi}
% \newcommand{\param}[1]{\versionedparam{\value{version}}{#1}}
\newcommand{\param}[1]{\versionedparam{0}{#1}}
\newcommand{\N}[0]{\versionedparam{\value{version}}{XX}}
\newcommand{\X}[0]{Svärd}



\newcommand{\equ}[2]{
\vspace{-0.75em}
\begin{equation}
    \footnotesize
    #1
    \label{#2}
    \vspace{0.25em}
\end{equation}
}

% \newcommand{\footref}[1]{\textsuperscript{\ref{#1}}}
\newcommand{\secref}[1]{§\ref{#1}}
\newcommand{\secsref}[1]{§§\ref{#1}}
\newcommand{\tabref}[1]{Table~\ref{#1}}
\newcommand{\algref}[1]{Alg.~\ref{#1}}
\newcommand{\figref}[1]{Fig.~\ref{#1}}
\newcommand{\figsref}[1]{Figs.~\ref{#1}}
\newcommand{\expref}[1]{Exp.~\ref{#1}}
\newcommand{\expsref}[1]{Exps.~\ref{#1}}
\newcommand{\obsref}[1]{Obsv.~\ref{#1}}
\newcommand{\obssref}[1]{Obsvs.~\ref{#1}}
% \renewcommand{\figref}[1]{Fig.~\ref{#1}}
% \renewcommand{\figsref}[1]{Figs.~\ref{#1}}
% \renewcommand{\expref}[1]{Exp.~\ref{#1}}
% \renewcommand{\expsref}[1]{Exps.~\ref{#1}}
% \renewcommand{\figurename}{Fig.}
% \renewcommand{\secref}[1]{§\ref{#1}}

\newcommand{\revtag}[1]{}
\newcommand{\copied}[2]{#2}
\ifcameraready
    \renewcommand{\copied}[2]{#2}
\else
    \ifrev 
        \renewcommand{\revtag}[1]{\todo{\footnotesize #1}}
    \else
        \renewcommand{\copied}[2]{\todo{Copied from #1}\textcolor{gray}{#2}}
    \fi
\fi

\newcommand{\rhmemisolationrefs}[0]{\cite{fournaris2017exploiting, poddebniak2018attacking, tatar2018throwhammer, carre2018openssl, barenghi2018softwareonly, zhang2018triggering, bhattacharya2018advanced, seaborn2015exploiting, kim2014flipping, safari2014rowhammer_, seaborn2015exploiting, vanderveen2016drammer_deterministic, gruss2016rowhammerjs_a, razavi2016flip, pessl2016drama_exploiting, xiao2016onebit, bosman2016dedup, bhattacharya2016curious, burleson2016invited, qiao2016anew, brasser2017cant, jang2017sgxbomb, aga2017when, mutlu2017therowhammer, tatar2018defeating, gruss2018another, lipp2018nethammer, vanderveen2018guardion, frigo2018grand, cojocar2019exploiting,  ji2019pinpoint, mutlu2019rowhammer_and, hong2019terminal, kwong2020rambleed, frigo2020trrespass, cojocar2020arewe, weissman2020jackhammer, zhang2020pthammer, yao2020deephammer, deridder2021smash, hassan2021uncovering, jattke2022blacksmith, tol2022toward, kogler2022halfdouble, orosa2022spyhammer, zhang2022implicit, liu2022generating, cohen2022hammerscope, zheng2023trojvit, fahrjr2022when, tobah2022spechammer, rakin2022deepsteal, park2016statistical, park2016experiments,lim2017active, ryu2017overcoming, yun2018study, yang2019trapassisted, walker2021ondram, kim2020revisiting, orosa2021adeeper, yaglikci2022understanding, khan2018analysis, agarwal2018rowhammer_for, li2014write, ni2018write, genssler2022onthe, mutlu2023fundamentally}}

\newcommand{\exploitingRowHammerAllCitations}[0]{\cite{fournaris2017exploiting, poddebniak2018attacking, tatar2018throwhammer, carre2018openssl, barenghi2018softwareonly, zhang2018triggering, bhattacharya2018advanced, seaborn2015exploiting, kim2014flipping, safari2014rowhammer_, seaborn2015exploiting, vanderveen2016drammer_deterministic, gruss2016rowhammerjs_a, razavi2016flip, pessl2016drama_exploiting, xiao2016onebit, bosman2016dedup, bhattacharya2016curious, burleson2016invited, qiao2016anew, brasser2017cant, jang2017sgxbomb, aga2017when, mutlu2017therowhammer, tatar2018defeating, gruss2018another, lipp2018nethammer, vanderveen2018guardion, frigo2018grand, cojocar2019exploiting,  ji2019pinpoint, mutlu2019rowhammer_and, hong2019terminal, kwong2020rambleed, frigo2020trrespass, cojocar2020arewe, weissman2020jackhammer, zhang2020pthammer, yao2020deephammer, deridder2021smash, hassan2021uncovering, jattke2022blacksmith, tol2022toward, kogler2022halfdouble, orosa2022spyhammer, zhang2022implicit, liu2022generating, cohen2022hammerscope, zheng2023trojvit, fahrjr2022when, tobah2022spechammer, rakin2022deepsteal, aydin2022cyber, mus2022jolt, wang2022research, lefforge2023reverse,fahr2022theeffects, kaur2022workinprogress, cai2022onthe, li2022cyberradar, li2023fphammer, roohi2022efficient, staudigl2022neurohammer, yang2022sociallyaware, islam2022signature, tomita2022extracting, france2022modeling}}

\newcommand{\understandingRowHammerAllCitations}[0]{\cite{redeker2002aninvestigation, kim2014flipping, park2014activeprecharge, park2016statistical, yang2016suppression, park2016experiments,lim2017active, ryu2017overcoming, yang2017scanning, lim2018study, yun2018study, yang2019trapassisted, gautam2019rowhammering, walker2021ondram, kim2020revisiting, orosa2021adeeper, jiang2021quantifying, orosa2022spyhammer, cohen2022hammerscope, yaglikci2022understanding, khan2018analysis, agarwal2018rowhammer_for, li2014write, ni2018write, genssler2022onthe, mutlu2023fundamentally, he2023whistleblower, baeg2022estimation, frigo2020trrespass, mutlu2017therowhammer, mutlu2018rowhammer, mutlu2019rowhammer_and, olgun2023anexperimental, olgun2023dram_bender, zhou2023doublesided, zhou2024unveiling, zhou2024understanding, li2023understanding, luo2023rowpress}}

\newcommand{\understandingRowHammerNVMCitations}[0]{\cite{khan2018analysis, agarwal2018rowhammer_for, li2014write, ni2018write, genssler2022onthe}}

\newcommand{\mitigatingRowHammerAllCitations}[0]{\cite{apple2015about, rh-hp,rh-lenovo,greenfield2016throttling, kim2014flipping, kim2014architectural, bains14d, bains2015method, jedec2020jesd794c, aichinger2015ddrmemory, aweke2016anvil, bains2015rowhammer, bains2015rowhammer, bains2016distributed, bains2016rowhammer, gomez2016dram_rowhammer, yang2016suppression, son2017making, seyedzadeh2018mitigating, irazoqui2016mascat, ryu2017overcoming, yang2017scanning, you2019mrloc, lee2019twice, park2020graphene, yaglikci2021security, yaglikci2021blockhammer, frigo2020trrespass, kang2020cattwo, hassan2021uncovering, qureshi2022hydra, saileshwar2022randomized, brasser2017cant, konoth2018zebram, vanderveen2018guardion, vig2018rapid, hassan2019crow, gautam2019rowhammering, kim2022mithril, lee2021cryoguard, marazzi2022rega, zhang2022softtrr, joardar2022learning, juffinger2023csirowhammercryptographic, yaglikci2022hira, saxena2022aqua, manzhosov2022revisiting, ajorpaz2022evax, naseredini2022alarm, joardar2022machine, hassan2024acase, zhang2020leveraging,loughlin2021stop, devaux2021method, han2021surround, fakhrzadehgan2022safeguard, saroiu2022theprice, saroiu2022howto, loughlin2022moesiprime, zhou2022ltpim, hong2023dsac, mutlu2023fundamentally, marazzi2023protrr, didio2023copyonflip, sharma2022areview, woo2023scalable, park2022rowhammer_reduction, wi2023shadow, kim2023a11v, guderamarao2023defending, guha2022criticality, france2022modeling, france2022reducing, bennett2021panopticon, enomoto2022efficient, arikan2022processor, tomita2022extracting, saxena2023ptguard, zhou2023dnndefender, bostanci2024comet, olgun2024abacus}}

\newcommand{\hwBasedRowHammerMitigations}[0]{\cite{apple2015about, rh-hp,rh-lenovo,greenfield2016throttling, kim2014flipping, kim2014architectural, bains14d, bains2015method, aichinger2015ddrmemory, aweke2016anvil, bains2015rowhammer, bains2015rowhammer, bains2016distributed, bains2016rowhammer, son2017making, irazoqui2016mascat, ryu2017overcoming, yang2017scanning, seyedzadeh2017counterbased, you2019mrloc, lee2019twice, park2020graphene, yaglikci2021blockhammer, frigo2020trrespass, kang2020cattwo, hassan2021uncovering, qureshi2022hydra, saileshwar2022randomized, brasser2017cant, konoth2018zebram, vanderveen2018guardion, vig2018rapid, gautam2019rowhammering, kim2022mithril, lee2021cryoguard, zhang2022softtrr, joardar2022learning, juffinger2023csirowhammercryptographic, yaglikci2022hira, saxena2022aqua, enomoto2022efficient, manzhosov2022revisiting, ajorpaz2022evax, joardar2022machine, hassan2024acase, zhang2020leveraging, loughlin2021stop, devaux2021method, han2021surround, fakhrzadehgan2022safeguard, saroiu2022theprice, saroiu2022howto, loughlin2022moesiprime, zhou2022ltpim, mutlu2023fundamentally, didio2023copyonflip, sharma2022areview, woo2023scalable, park2022rowhammer_reduction, wi2023shadow, kim2023a11v, guderamarao2023defending, guha2022criticality, france2022modeling, france2022reducing, arikan2022processor, tomita2022extracting, saxena2023ptguard, zhou2023dnndefender, yang2016suppression, bostanci2024comet, bennett2021panopticon, seyedzadeh2018mitigating, gomez2016dram_rowhammer, gautam2019rowhammering, wang2021discreetpara, hassan2019crow, yaglikci2021security, woo2023scalable, zhou2022ltpim, olgun2024abacus, marazzi2022rega}}

\newcommand{\swBasedRowHammerMitigations}[0]{
\cite{enomoto2022efficient, konoth2018zebram, vanderveen2018guardion, brasser2017cant, bock2019riprh, aweke2016anvil, zhang2022softtrr}
}

\newcommand{\mcBasedRowHammerMitigations}[0]{\cite{apple2015about, rh-hp,rh-lenovo,greenfield2016throttling, kim2014flipping, kim2014architectural, bains14d, bains2015method, aichinger2015ddrmemory, aweke2016anvil, bains2015rowhammer, bains2015rowhammer, bains2016distributed, bains2016rowhammer, son2017making, irazoqui2016mascat, ryu2017overcoming, yang2017scanning, seyedzadeh2017counterbased, you2019mrloc, lee2019twice, park2020graphene, yaglikci2021blockhammer, frigo2020trrespass, kang2020cattwo, hassan2021uncovering, qureshi2022hydra, saileshwar2022randomized, brasser2017cant, konoth2018zebram, vanderveen2018guardion, vig2018rapid, gautam2019rowhammering, kim2022mithril, lee2021cryoguard, zhang2022softtrr, joardar2022learning, juffinger2023csirowhammercryptographic, yaglikci2022hira, saxena2022aqua, enomoto2022efficient, manzhosov2022revisiting, ajorpaz2022evax, joardar2022machine, hassan2024acase, zhang2020leveraging, loughlin2021stop, devaux2021method, han2021surround, fakhrzadehgan2022safeguard, saroiu2022theprice, saroiu2022howto, loughlin2022moesiprime, zhou2022ltpim, mutlu2023fundamentally, didio2023copyonflip, sharma2022areview, woo2023scalable, park2022rowhammer_reduction, wi2023shadow, kim2023a11v, guderamarao2023defending, guha2022criticality, france2022modeling, france2022reducing, arikan2022processor, saxena2023ptguard, zhou2023dnndefender}}

\newcommand{\inDRAMRowHammerMitigations}[0]{\cite{jedec2020jesd794c, gomez2016dram_rowhammer, seyedzadeh2018mitigating, yang2016suppression, yaglikci2021security, marazzi2022rega, hassan2019crow, hong2023dsac, marazzi2023protrr, bennett2021panopticon}}


\newcommand{\deterministicRowHammerDefenseCitations}[0]{\cite{lee2019twice, yaglikci2021blockhammer, seyedzadeh2017counterbased, seyedzadeh2018mitigating, kang2020cattwo, park2020graphene, kim2022mithril, saileshwar2022randomized, saxena2022aqua, kim2014architectural, bains2016rowhammer}}

\newcommand{\probabilisticRowHammerDefenseCitations}[0]{\cite{kim2014flipping, you2019mrloc, son2017making}}

\newcommand{\refreshBasedRowHammerDefenseCitations}[0]{\cite{rh-lenovo, rh-hp, bains2015method, bains14d, bains2015rowhammer, lee2019twice, seyedzadeh2017counterbased,vig2018rapid, irazoqui2016mascat, seyedzadeh2018mitigating, kang2020cattwo, park2020graphene, kim2022mithril, kim2014architectural, bains2015rowhammer, bains2016distributed, bains2016rowhammer, aweke2016anvil, apple2015about, kim2014flipping, son2017making, you2019mrloc, yaglikci2021security, frigo2020trrespass, hassan2021uncovering, loughlin2021stop, qureshi2022hydra, devaux2021method, wang2021discreetpara, marazzi2022rega, zhang2022softtrr, joardar2022learning, yaglikci2022hira, saroiu2022howto, bostanci2024comet, olgun2024abacus, joardar2022machine}}

\newcommand{\throttlingBasedRowHammerDefenseCitations}[0]{\cite{greenfield2016throttling, yaglikci2021blockhammer}}

\newcommand{\integrityBasedRowHammerDefenseCitations}[0]{\cite{saxena2023ptguard, juffinger2023csirowhammercryptographic, fakhrzadehgan2022safeguard, ajorpaz2022evax, didio2023copyonflip, manzhosov2022revisiting, guderamarao2023defending}}

\newcommand{\isolationBasedRowHammerDefenseCitations}[0]{\cite{saileshwar2022randomized, wi2023shadow, loughlin2021stop, zhou2023dnndefender, woo2023scalable, bock2019riprh,konoth2018zebram, vanderveen2018guardion, brasser2017cant, saxena2022aqua, woo2023scalable, hassan2019crow}}

\newcommand{\circuitBasedRowHammerDefenseCitations}[0]{\cite{park2022rowhammer_reduction, kim2023a11v, gautam2019rowhammering, yang2016suppression, hassan2019crow, gomez2016dram_rowhammer, han2021surround, ryu2017overcoming, yang2017scanning, zhou2022ltpim, lee2021cryoguard, hassan2024acase, gautam2019rowhammering}}

\newcommand{\detectionOnlyCitations}[0]{\cite{zhang2020leveraging, arikan2022processor, france2022reducing, zhou2022ltpim}}

\newcommand{\surveyCitations}[0]{\cite{mutlu2023fundamentally, sharma2022areview, saroiu2022theprice, aichinger2015ddrmemory}}

\newcommand{\systemImprovementBasedDefenseCitations}[0]{\cite{loughlin2022moesiprime, guha2022criticality, loughlin2021stop}}

%,,,,,,,,,,,,,,,,,,,,,,,,,,,,,,,

\newcommand{\rowHammerGetsWorseCitations}[0]{\cite{kim2014flipping, kim2020revisiting, frigo2020trrespass, yaglikci2022understanding, orosa2021adeeper, mutlu2017therowhammer, mutlu2018rowhammer, mutlu2019rowhammer_and, cojocar2020arewe, mutlu2023fundamentally, luo2023rowpress}}

\newcommand{\rowHammerDefenseScalingProblemsCitations}[0]{\cite{kim2020revisiting, yaglikci2021blockhammer, park2020graphene, mutlu2017therowhammer, mutlu2018rowhammer, mutlu2019rowhammer_and, mutlu2023fundamentally, hassan2021uncovering}}

\newcommand{\rhdefinition}[0]{\cite{kim2014flipping, kim2020revisiting, mutlu2017therowhammer, yang2019trapassisted, mutlu2019rowhammer_and, walker2021ondram, park2016experiments, park2016statistical, yaglikci2022understanding}}
\newcommand{\rhdefrefresh}[0]{\cite{apple2015about, kim2014flipping, kim2014architectural, bains2015rowhammer, aweke2016anvil, bains2016rowhammer, bains2016distributed, son2017making, seyedzadeh2018mitigating, you2019mrloc, lee2019twice, park2020graphene, yaglikci2021security, frigo2020trrespass, kang2020cattwo, hassan2021uncovering, qureshi2022hydra, kim2022mithril, devaux2021method, lee2021cryoguard, marazzi2022rega, zhang2022softtrr, joardar2022learning}}
\newcommand{\rhdef}[0]{\cite{apple2015about, kim2014flipping, kim2014architectural, aweke2016anvil, bains2015rowhammer, bains2016rowhammer, bains2016distributed, son2017making, seyedzadeh2018mitigating, you2019mrloc, lee2019twice, park2020graphene, yaglikci2021security, yaglikci2021blockhammer, frigo2020trrespass, kang2020cattwo, hassan2021uncovering, qureshi2022hydra, saileshwar2022randomized, brasser2017cant, konoth2018zebram, vanderveen2018guardion, greenfield2016throttling, kim2022mithril, lee2021cryoguard, marazzi2022rega, zhang2022softtrr, joardar2022learning, juffinger2023csirowhammercryptographic}}
\newcommand{\perrefreshscaling}[0]{\cite{nguyen2018nonblocking, liu2012raidr, baumann2005radiationinduced, liu2013anexperimental, chang2014improving, kang2014coarchitecting, mukundan2013understanding, nair2014refresh, nair2013archshield}}
\newcommand{\rhsafe}[0]{\cite{frigo2020trrespass, lee2014green, micron2014sdram}}
\newcommand{\rhworse}[0]{\cite{kim2014flipping,mutlu2017therowhammer,mutlu2019rowhammer_and,kim2020revisiting, frigo2020trrespass, hassan2021uncovering, orosa2021adeeper, jattke2022blacksmith, yaglikci2022understanding, deridder2021smash}}
\newcommand{\rhdefworse}[0]{\cite{kim2020revisiting,hassan2021uncovering, orosa2021adeeper, yaglikci2021security, yaglikci2021blockhammer, park2020graphene, qureshi2022hydra}}
\newcommand{\rhattacks}[0]{\cite{seaborn2015exploiting, vanderveen2016drammer_deterministic, gruss2016rowhammerjs_a, razavi2016flip, pessl2016drama_exploiting, xiao2016onebit, bosman2016dedup, bhattacharya2016curious, qiao2016anew, jang2017sgxbomb, aga2017when, mutlu2017therowhammer, tatar2018defeating, gruss2018another, lipp2018nethammer, vanderveen2018guardion, frigo2018grand, cojocar2019exploiting,  ji2019pinpoint, mutlu2019rowhammer_and, hong2019terminal, kwong2020rambleed, frigo2020trrespass, cojocar2020arewe, weissman2020jackhammer, zhang2020pthammer, safari2014rowhammer_, yao2020deephammer,deridder2021smash,
hassan2021utrr, jattke2022blacksmith, tol2022toward,burleson2016invited, brasser2017can, kim2014flipping, kogler2022half}}
\newcommand{\salprefs}[0]{\cite{kim2012acase, chang2014improving, wang2020figaro, zhang2014cream}}


% \titlespacing\section{0pt}{5pt plus 2pt minus 2pt}{0pt plus 2pt minus 2pt}
% \titlespacing\subsection{0pt}{5pt plus 2pt minus 2pt}{0pt plus 2pt minus 2pt}
% \titlespacing\subsubsection{0pt}{5pt plus 2pt minus 2pt}{0pt plus 2pt minus 2pt}


 % \makeatletter
 % \g@addto@macro{\normalsize}{%
 %   \setlength{\abovedisplayskip}{2pt plus 0.5pt minus 1pt}
 %   \setlength{\belowdisplayskip}{2pt plus 0.5pt minus 1pt}
 %   \setlength{\abovedisplayshortskip}{0pt}
 %   \setlength{\belowdisplayshortskip}{0pt}
 %   \setlength{\intextsep}{2pt plus 1pt minus 1pt}
 %   \setlength{\textfloatsep}{2pt plus 1pt minus 1pt}
 %   \setlength{\skip\footins}{2pt plus 1pt minus 1pt}}
 %   \setlength{\abovecaptionskip}{2pt plus 1pt minus 1pt}
 % \makeatother

==> mainmatter/06_svard/sections/00_abstract.tex <==
\begin{abstract}
Read disturbance in modern DRAM chips is a widespread \om{2}{phenomenon} and is reliably used for breaking memory isolation, \om{2}{a} fundamental building block \om{2}{for building robust systems}. RowHammer and RowPress are two examples of read disturbance in DRAM where repeatedly accessing (hammering) or keeping active (pressing) a memory location induces bitflips in other memory locations. Unfortunately, shrinking technology node size exacerbates read disturbance in DRAM chips over generations. As a result, existing defense mechanisms suffer from significant performance \om{2}{and} energy overheads, limited effectiveness, or prohibitively high hardware complexity. 
    
In this \agy{3}{chapter}, we tackle these shortcomings by leveraging the spatial variation in read disturbance across different memory locations in real DRAM chips.
To do so, we
1)~present the first rigorous real DRAM chip characterization study of spatial variation of read disturbance and
2)~propose Svärd, a new mechanism that dynamically adapts the aggressiveness of existing solutions based on the \agy{2}{row-level} read disturbance profile. 
Our experimental characterization on \numchips{} real DDR4 DRAM chips representing 11 die revisions demonstrates a large variation in read disturbance vulnerability across different memory locations\om{4}{:} \agy{4}{in the part of memory with the worst read disturbance vulnerability, 1)~up to $2\times$ the number of bitflips can occur and 2)~bitflips can occur at an order of magnitude fewer accesses, compared to the memory locations with the least vulnerability to read disturbance.} 
Svärd \om{2}{leverages \om{4}{this} variation to reduce} the overheads of \param{five} state-of-the-art read disturbance \agy{4}{solutions}, \om{2}{and thus significantly increases system performance.} 
% by $2.4\times/2.7\%/1.6\times/3.0\times$, on average, across several multiprogrammed workloads.
\end{abstract}

==> mainmatter/06_svard/sections/01_introduction.tex <==
%!TEX root =  main.acmart.tex
\section{Introduction}
\label{sec:introduction}

{To ensure system \om{2}{robustness (including} reliability, security, and safety\om{2}{)}, it is critical to {maintain} {memory isolation: accessing a memory address should not cause unintended side-effects on data stored on other addresses~\cite{kim2014flipping}. {Unfortunately}, with aggressive technology scaling, DRAM~\cite{dennard1968fieldeffect}, the prevalent {main} memory technology}, suffers from increased \emph{read disturbance}: accessing (reading) a row of DRAM cells (\om{2}{i.e., a} DRAM row) degrades the data integrity of other physically close but \emph{unaccessed} DRAM rows.}
\emph{RowHammer} and \emph{RowPress} are two prime examples of \om{2}{the} {DRAM read {disturbance} phenomenon {where} a DRAM row (i.e., victim row) can experience bitflips when a nearby DRAM row (i.e., aggressor row) is} 1)~repeatedly opened (i.e., hammered)~\rhmemisolationrefs{} or 2)~kept open for a long period (i.e., pressed)~\cite{luo2023rowpress}, respectively.

Many prior works demonstrate attacks on a wide range of systems \om{4}{that} exploit read disturbance {to escalate {privilege}, leak private data, and manipulate critical application outputs~\exploitingRowHammerAllCitations{}.
To make matters worse, \om{2}{various} experimental studies~\cite{kim2014flipping, mutlu2017therowhammer, mutlu2019rowhammer_and, frigo2020trrespass, cojocar2020arewe, kim2020revisiting, kim2014flipping, luo2023rowpress} \om{2}{find} that {newer DRAM chip generations are more susceptible to read disturbance}. {For example,} chips manufactured in {2018-2020} can experience RowHammer {bitflips} at an order of magnitude fewer row activations compared to the chips manufactured in {2012-2013}~\cite{kim2020revisiting}. As {read disturbance \agy{2}{in} DRAM chips} worsens, ensuring \om{2}{robust (i.e.,} \agy{2}{reliable, secure, and safe}\om{2}{)} operation {becomes} more expensive in terms of performance overhead, energy consumption, and hardware complexity~\cite{kim2020revisiting, yaglikci2021blockhammer, park2020graphene}. Therefore, it is {critical} to understand {the read disturbance \om{4}{vulnerabilities of} DRAM chips} in greater detail with in-depth insights \om{2}{in order}
to develop more effective and {efficient} solutions for current and future DRAM-based {memory} systems.}
To this end, prior works study \om{2}{various} characteristics of DRAM read disturbance~\understandingRowHammerAllCitations{}. Unfortunately, \emph{no} prior work rigorously studies the spatial variation {of} DRAM read disturbance and its implications on future solutions.

Our \emph{goal} in this \agy{3}{chapter} is to build a detailed understanding of the spatial variation in read disturbance across DRAM rows and leverage this understanding to improve the existing solutions.
To this end, in this \agy{3}{chapter}, we 1)~present the first rigorous experimental characterization of the spatial variation in read disturbance \agy{4}{vulnerabilities of} \om{2}{real} DRAM \om{2}{chips}, and 2)~propose \X{}, a new mechanism that dynamically adapts the aggressiveness of existing solutions based on the \om{2}{observed} variation.

\head{Characterization} We test \numchips{} modern real DDR4 DRAM chips representing \om{4}{\param{11}} different die revisions from three major manufacturers.\footnote{We test DRAM chips from Samsung, SK Hynix, and Micron, which hold the largest market shares of  40.7\%, 28.8\%, and 26.4\% respectively~\cite{alsop2023dram_manufacturers, wang2022dueto}.} Our experimental results show that the \agy{4}{read disturbance vulnerabilities of DRAM chips vary} \emph{significantly} and \emph{irregularly} across 1)~DRAM rows within a DRAM subarray, i.e., a two-dimensional DRAM array that consists of hundreds of DRAM rows~(\secref{sec:background}) and 2)~subarrays within a DRAM bank, i.e., a group of many subarrays that share an I/O circuitry~(\secref{sec:background}).
\agy{2}{We \agy{4}{make two key observations from our characterization: 1)~the} fraction of erroneous DRAM cells, i.e., \gls{ber}, \om{4}{varies by a factor of $2\times$ and 2)~\gls{hcfirst} varies} by an order of magnitude across DRAM rows in a subarray.} 

\agy{4}{We} investigate \om{4}{the} correlations between a victim DRAM row's spatial features (i.e., physical location within the corresponding subarray and bank) and read disturbance vulnerability \agy{4}{in two steps. First,} we reverse engineer the organization of a DRAM bank. 
% \om{4}{(\secref{sec:background}).} 
\agy{4}{Second, we} perform \om{4}{extensive} statistical analyses based on \agy{4}{1)}~reverse-engineered spatial features and \agy{4}{2)}~observed \gls{hcfirst} values. \agy{4}{We make the key observation} that the variation in read disturbance vulnerability across DRAM rows correlates well with the spatial features of DRAM rows \emph{only} in four out of \param{15} tested DRAM modules. \agy{4}{Therefore, we conclude that read disturbance vulnerability irregularly varies across DRAM rows, and thus, row-level spatial features \om{5}{we evaluate} are insufficient to predict read disturbance vulnerability.}

\head{Improving existing solutions} 
\om{4}{Based on the understanding we develop via our rigorous experimental characterization,} we propose \X{}\om{2}{,} a new mechanism that dynamically adapts the aggressiveness of existing solutions \agy{2}{to the read disturbance vulnerability level of \om{5}{each} potential victim row. \X{} forces an existing solution to react more aggressively to an aggressor row activation (e.g., preventively refresh the potential victim row) if \om{4}{a} potential victim row is more vulnerable to read disturbance.} \X{} is implemented together with existing solutions, which can be either 1)~in the memory controller within the processor chip \om{4}{(i.e.,} without \om{2}{modifications to} the DRAM chip \om{2}{or \om{4}{DRAM} interface}\om{4}{)} or 2)~within the DRAM chip \om{4}{(i.e.,} \om{4}{transparent} to the rest of the system\om{4}{)}.
\agy{4}{We evaluate the performance benefits of \X{} on \param{five} state-of-the-art solutions,}
\agy{5}{AQUA~\cite{saxena2022aqua},} {BlockHammer~\cite{yaglikci2021blockhammer},} Hydra~\cite{qureshi2022hydra}, PARA~\cite{kim2014flipping}, and RRS~\cite{saileshwar2022randomized}
\agy{4}{using three representative spatial distribution profiles of read disturbance that we generate based on our experimental characterization \om{5}{of real DRAM chips} (i.e., one for each manufacturer). Our performance evaluation results show that}
% We showcase that 
\X{} significantly \om{2}{reduces the performance overheads} of 
% these \param{four} state-of-the-art solutions,
{\agy{5}{AQUA}, BlockHammer,} Hydra, PARA, and RRS, \om{4}{leading to system performance improvements of} \agy{5}{$1.23\times$,} {$2.65\times$}, $1.03\times$, $1.57\times$, and $2.76\times$, \agy{2}{respectively,} on average across \wlcnt{} multiprogrammed memory-intensive workloads.
%and three different read disturbance profiles from real DRAM chips.

{We make the following contributions:}
\begin{itemize}
    \item We present the first rigorous characterization of the spatial variation \om{4}{of} read disturbance in \om{2}{modern} DRAM \om{2}{chips}. Our experimental results on \numchips{} real \om{2}{DDR4} DRAM chips {spanning 11 different die revisions} show a \agy{2}{significant and irregular} variation \om{2}{in} read {disturbance} vulnerability across DRAM rows. 
    \item We propose \X{}, a new mechanism that dynamically adapts the aggressiveness of an existing read disturbance solution \agy{2}{to the vulnerability level of the potential victim row.}
    \item We showcase \X{}'s integration with \param{five} different state-of-the-art read disturbance \agy{4}{solutions}. \om{2}{Our results} show that \X{} reduces the performance overhead of \om{2}{these four state-of-the-art} solutions, \om{4}{leading to large system performance benefits.} 
\end{itemize}





==> mainmatter/06_svard/sections/02_background.tex <==
\section{Background}
\label{sec:background}
This section provides a concise overview of 1)~DRAM organization and operation
and 2)~DRAM read disturbance.
For more detail, we refer the reader to prior works {on DRAM and read disturbance}~\cite{ipek2008selfoptimizing,zhang2014halfdram, qureshi2015avatar, liu2012raidr, liu2013anexperimental, keeth2001dram_circuit, mutlu2007stalltime, moscibroda2007memory, mutlu2008parallelismaware, kim2010atlas, subramanian2014theblacklisting, kim2012acase, kim2014flipping,
hassan2016chargecache, chang2016understanding, lee2017design,  chang2017understanding,  patel2017reaper,kim2018dram, kim2020revisiting, hassan2019crow, frigo2020trrespass, chang2014improving, chang2016low, ghose2018vampire, hassan2017softmc, khan2016parbor, khan2016case, khan2014efficacy, seshadri2015gather, seshadri2017ambit, kim2018solar, kim2019d, patel2019understanding, patel2020beer, lee2013tiered, lee2015decoupled, seshadri2013rowclone, luo2020clrdram, seshadri2019dram, wang2020figaro}.
\agycomment{4}{Non-SAFARI references: \cite{keeth2001dram_circuit, ipek2008selfoptimizing,zhang2014halfdram, qureshi2015avatar}}


% This section describes the background required to understand the rest of the paper. For a more comprehensive description of DRAM organization and operation, we refer the reader to~\cite{kim2012acase,liu2012raidr,lee2013tieredlatency,keeth2001dram_circuit}.

\subsection{DRAM {Organization and Operation}}
\label{sec:dram_background}

\head{Organization}
{\figref{fig:dram_organization}a shows the organization of DRAM-based memory systems. A memory channel connects the processor (CPU) to a set of DRAM chips, called \agy{4}{\emph{DRAM rank}}.}
\agy{4}{Chips in a DRAM rank operate in lock-step.}
\agy{0}{Each chip has multiple DRAM banks, each consisting of multiple DRAM cell arrays \om{4}{(called \emph{subarrays})} and their local I/O circuitry. \om{4}{Within a subarray,} DRAM cells are organized as a two-dimensional array \om{4}{of} DRAM rows and columns.}
% DRAM cells in a DRAM row are connected to a wire, called wordline; and cells in a DRAM column are connected to another wire called bitline. 
{A} DRAM cell {stores one bit of data} {in the form of} electrical charge in {a} capacitor, which can be accessed through an access transistor.  
A wire called \om{4}{wordline} drives the gate of all DRAM cells' access transistors in a DRAM row\om{4}{. A} wire called \om{4}{\emph{bitline}} connects all DRAM cells in a DRAM column to a common differential sense amplifier. Therefore, when a wordline is asserted, each DRAM cell in the DRAM row is connected to its corresponding sense amplifier. The set of sense amplifiers in a subarray is called \om{4}{\emph{the row buffer}}, where the data of \om{4}{an activated} DRAM row is buffered \agy{4}{to serve a column access.}
% {An access transistor, controlled by the wordline, conducts the cell capacitor to the bitline.}}
% {To access a DRAM row, the row decoder asserts a wire called wordline.}
% {DRAM cells in the same column are connected to a set of differential sense amplifiers called row buffer via a shared wire called bitline.}

\begin{figure}[h]
    \centering
    \includegraphics[width=\linewidth]{figures/background.png}
    \caption{DRAM organization}
    \label{fig:dram_organization}
\end{figure}

\head{Operation}
\copied{ABACUS}{
The memory controller serves memory access requests by issuing DRAM commands, e.g., row activation ($ACT$), bank precharge ($PRE$), data read ($RD$), data write ($WR$), and refresh ($REF$) \gf{0}{while respecting certain timing parameters to guarantee correct operation~\cite{jedec2020jesd795,jedec2020jesd2095a,jedec2017jesd2094b, jedec2021jesd235d,jedec2008jesd79f,jedec2020jesd794c,jedec2012standard}.}
To read or write data\om{4}{;} the memory controller first \om{4}{needs to activate the corresponding row. To do so, it} issues an $ACT$ command alongside the bank address and row address corresponding to the memory request's address. 
%and opens a row corresponding to the memory request's address. 
When a row is activated, its data is copied \gf{0}{to and temporarily stored at} the row buffer.
\gf{0}{The latency from the start of a row activation until the data
is reliably readable\om{4}{/writable} in the row buffer is called \om{4}{the} \emph{\gls{trcd}}.}
\gf{0}{During the row activation process, a DRAM cell loses its charge, and thus, its initial charge needs to be restored (\om{4}{via} a process called \emph{charge restoration}). 
The latency from the start of a row activation until the completion of the DRAM cell's charge restoration is called \agy{4}{the \emph{\gls{tras}}}.%DRAM manufacturers provide a built-in safety margin in the nominal timing parameters to account for the worst-case latency in \gls{trcd} and \gls{tras} operations~\cite{}.
}
The memory controller can read/{write} data from/to the row buffer using $RD$/$WR$ commands.
The changes are propagated to the DRAM cells in the open row. 
Subsequent accesses to the same row can be served quickly \om{4}{from the row buffer (i.e., called a \emph{row hit})} without issuing another $ACT$ to the same row. 
\gf{0}{The latency of performing a read/write operation is called \gls{tcl}/\gls{tcwl}}. 
To access another row in \om{4}{an already} activated DRAM bank, the memory controller must issue a $PRE$ command \om{4}{to} close the opened row \om{4}{and prepare the bank for a new activation}.
%, creating a \emph{row miss/conflict.} 
\agy{4}{When the $PRE$ command is issued}, the DRAM chip de-asserts the active row's wordline and precharges the bitlines. The timing parameter for precharge is called \om{4}{the \emph{\gls{trp}}}.}


{\om{4}{A} DRAM cell \om{4}{is} inherently leaky and thus \om{4}{loses its} stored electrical charge over time. To maintain data integrity, a DRAM cell {is periodically refreshed} with a {time interval called \agy{4}{the \emph{\gls{trefw}}}, which is typically} \SI{64}{\milli\second} (e.g.,~\cite{jedec2012standard, jedec2020jesd794c, micron2014sdram}) or \SI{32}{\milli\second} (e.g.,~\cite{jedec2017jesd2094b, jedec2020jesd795, jedec2020jesd2095a}) \agy{4}{at normal operating temperature (\om{5}{i.e.}, up to \SI{85}{\celsius}) and half of it for the extended temperature range (\om{5}{i.e.}, above \SI{85}{\celsius} up to \SI{95}{\celsius})}.  
To {timely} refresh all cells, the memory controller {periodically} issues a refresh {($REF$)} command with {a time interval called} \agy{4}{the \emph{\gls{trefi}}}, {which is typically} \SI{7.8}{\micro\second} {(e.g.,~\cite{jedec2012standard, jedec2020jesd794c, micron2014sdram}) or} \SI{3.9}{\micro\second} (e.g.,~\cite{jedec2017jesd2094b, jedec2020jesd795, jedec2020jesd2095a}) \agy{4}{at normal operating temperature.} When a rank-/bank-level refresh command is issued, the DRAM chip internally refreshes several DRAM rows, during which the whole rank/bank is busy. This operation's latency is called \agy{4}{the \emph{\gls{trfc}}}.} 
% in DDR4~\cite{jedec2020jesd794c}/DDR5~\cite{jedec2020jesd795}.


% \head{DRAM Timing Parameters} 
% \copied{ABACUS}{The memory controller schedules DRAM commands according to certain timing parameters to guarantee correct operation~\cite{jedec2020jesd795,jedec2020jesd2095a,jedec2017jesd2094b, jedec2021jesd235d,jedec2008jesd79f,jedec2020jesd794c,jedec2012standard}.}
% % {In addition to \gls{trefw}, \gls{trefi}, and \gls{trfc},} three {other} timing parameters are important to understand the rest of the paper: i)~\gls{trc} (Fig.~\ref{fig:dram_organization}b), ii)~\gls{trrd}, iii)~\gls{tras}.}
% \agycomment{0}{Add missing timing constraints.}

\subsection{Read Disturbance in DRAM}
\label{sec:background_rowhammer}
Read disturbance is the phenomenon that reading data from a memory or storage device causes physical disturbance (e.g., voltage deviation, electron injection, electron trapping) on another piece of data that is \emph{not} accessed but physically located nearby the accessed data. Two prime examples of read disturbance in modern DRAM chips are RowHammer~\cite{kim2014flipping}, and RowPress~\cite{luo2023rowpress}, where repeatedly accessing (hammering) or keeping active (pressing) a DRAM row induces bitflips in physically nearby DRAM rows, respectively. In RowHammer and RowPress terminology, the row that is hammered or pressed is called the \emph{aggressor} row, and the row that experiences bitflips the \emph{victim} row.
\copied{ABACUS}{For read disturbance bitflips to occur, 1)~the aggressor row needs to be activated more than a certain threshold value, \agy{0}{defined as \gls{hcfirst}~\cite{kim2020revisiting} \om{4}{and/}or 2)~\gls{taggon}~\cite{luo2023rowpress} need to be large-enough~\cite{kim2020revisiting, orosa2021adeeper, yaglikci2022understanding, luo2023rowpress}. To avoid read disturbance bitflips, systems take preventive actions, e.g., \om{4}{they refresh} victim rows~\refreshBasedRowHammerDefenseCitations{}, selectively \om{4}{throttle} accesses to aggressor rows~\cite{yaglikci2021blockhammer, greenfield2016throttling}, and physically \om{4}{isolate} potential aggressor and victim rows~\cite{hassan2019crow, konoth2018zebram, saileshwar2022randomized, saxena2022aqua, wi2023shadow, woo2023scalable}. These \agy{4}{solutions} aim to perform preventive actions before the cumulative effect of an aggressor row's \emph{activation count} and \emph{on time} causes read disturbance bitflips.
% certain threshold. To achieve this, these mechanisms are configured for an activation count threshold called \gls{nrh}, which is strictly smaller than \gls{hcfirst}.
}}

% \copied{ABACUS}{
% \atb{Many prior works demonstrate malicious attacks that can leak private data and take over operating systems using RowHammer~\exploitingRowHammerAllCitations{}.}
% \atb{Recent work~\cite{kim2020revisiting} analyzes the RowHammer phenomenon and demonstrates that \gls{nrh} is smaller in newer DRAM chips compared to older chips, indicating that RowHammer is an increasingly worsening system reliability, security, and safety problem.}\agycomment{elaborate on the quantitative comparison of RowHammer vulnerability across old and new chips provided in intro in a footnote.}}

% \textbf{RowHammer \agy{0}{Mitigation} Mechanisms.}
% \copied{ABACUS}{To prevent RowHammer bitflips and protect computing systems against RowHammer attacks, prior works propose different RowHammer mitigation mechanisms~\mitigatingRowHammerAllCitations{}. These works trigger their counter-measure (e.g., refreshing potential victim rows) based on either i)~the result of a probabilistic procedure or ii)~tracking {the number of times DRAM rows are activated (i.e.,} row activation counts). While probabilistic procedures can be implemented at low chip area cost, they incur prohibitively large performance overheads when configured for sub-1K \gls{nrh} values~\cite{kim2020revisiting, yaglikci2022hira}. Prior works propose several row activation tracking mechanisms that detect the most frequently activated rows. Unfortunately, while providing better performance than the probabilistic mechanisms, the chip area overhead of these mechanisms significantly increases as DRAM chips become more vulnerable to RowHammer.\footnote{Hydra~\cite{qureshi2022hydra} is an exception in this classification as it incurs low area overhead in processor chip area while tracking row activation counts. Hydra achieves this by storing the counters in a DRAM array and caching them in the memory controller. \secref{sec:motivation} discusses Hydra's scalability limitations.}}


% \subsection{Read Disturbance in DRAM}
% \label{sec:background_rowhammer}

% \begin{itemize}
%     \item RowHammer
%     \item{ber}
%     \item \gls{hcfirst} \agycomment{0}{check the definitions in Silver Bullet, which might be more useful}
%     \item RowPress
%     \item \gls{taggon}

% \end{itemize}








==> mainmatter/06_svard/sections/08_limitations.tex <==
\section{Limitations}
\label{svard:sec:limitations}

We acknowledge the limitations of our characterization study i

and \X{} under {{four}} categories.
\begin{itemize}
    \item We tried only a subset of potential hammer counts 
    \item We did not test all the DRAM chips available in the market
    \item We did not test all possible data patterns 
    \item It is not clear whether the variation changes with the effect of aging. 
    \item We showcase \X{}'s performance benefits and discuss two naive implementations. This paper does \emph{not} exhaustively explores \X{}'s design space. We leave designing more effective and efficient implementations to future work.
\end{itemize}

==> mainmatter/06_svard/sections/09_relatedwork.tex <==
\section{Related Work}
\label{svard:sec:related_work}

{This is the first work that 
1)~rigorously and experimentally analyzes the spatial variation \om{4}{of} read disturbance in real DRAM chips
and
2)~provide a new mechanism that can dynamically adapt the aggressiveness of existing read disturbance mitigation solutions based on the variation profile of real DRAM chips. 
We highlight our key contributions by contrasting our characterization analysis and proposed mechanism to previous DRAM read disturbance characterization studies and solutions.} 

\head{Characterization Studies}
{Six major works extensively characterize the read disturbance in real DRAM chips~\cite{kim2014flipping,kim2020revisiting,orosa2021adeeper, yaglikci2022understanding, olgun2023anexperimental, luo2023rowpress}.\footnote{{Other prior works~\cite{park2014activeprecharge, park2016experiments, park2016statistical} present preliminary experimental data from a \om{4}{small number of} (three to five) DDR3 DRAM chips. \om{4}{These works use a} 
% which is \emph{not} conclusive enough due to the extremely 
small sample set of DRAM cells, rows, and chips.}} 
First, Kim et al.~\cite{kim2014flipping} 
1)~investigate the vulnerability of 129 commodity DDR3 DRAM modules to various RowHammer attack models;
2)~demonstrate for the first time that RowHammer is a real problem
for commodity DRAM chips; and
3)~characterize RowHammer's sensitivity to refresh rate and activation rate in terms of \gls{ber}, \gls{hcfirst}, and the physical distance between aggressor and victim rows.
Second, Kim et al.~\cite{kim2020revisiting} conduct comprehensive scaling experiments on a wide range of 1580 DDR3, DDR4, and LPDDR4 commodity DRAM chips from different DRAM generations and technology nodes, demonstrating that RowHammer has become an even more serious problem over DRAM generations \om{4}{and existing solutions would be expensive for future technology nodes}. 
Third, Orosa et al.~\cite{orosa2021adeeper} rigorously characterize various aspects of the RowHammer vulnerability in real DRAM chips, including the effects of temperature, aggressor row active time, and victim DRAM cell's physical location on the RowHammer
vulnerability.  
{Fourth, Ya{\u{g}}l{\i}k{\c{c}}{\i} et al.~\cite{yaglikci2022understanding} investigate RowHammer's sensitivity to wordline voltage and the effects of reducing wordline voltage on DRAM reliability across 272 DRAM chips where 4K rows in a bank is tested in each chip. Fifth, Olgun et al.~\cite{olgun2023anexperimental, olgun2023anexperimental} test \om{5}{an} HBM2 DRAM chip's RowHammer vulnerability and data retention characteristics on a subset of DRAM rows in a DRAM bank with a focus on the spatial variation of RowHammer vulnerability \om{4}{across rows and HBM channels} and the characteristics of on-die target row refresh mechanisms. Sixth, } 
Luo et al.~\cite{luo2023rowpress} are the first to experimentally demonstrate and analyze RowPress, another read disturbance phenomenon, in 164 real DDR4 DRAM chips. They show that RowPress is different \om{4}{from} RowHammer, since it 
1)~affects a different set of DRAM cells from RowHammer and 
2)~behaves differently from RowHammer as temperature and access pattern change.  
{Unfortunately, these} works only analyze \emph{a subset of the DRAM rows.}
% in \emph{a single DRAM bank} in a DRAM rank. 
In contrast, our {paper takes a} step further and {contributes \om{4}{in} three aspects. First, \agy{4}{we} analyze} 1)~\emph{all} DRAM rows in a DRAM bank and \agy{4}{2)~a DRAM bank from \emph{all} four DRAM bank groups} in a DRAM rank, which {demonstrates the variation in read disturbance vulnerability across rows and banks more accurately \om{4}{and comprehensively}. Second, \om{4}{we study} the correlation between a row's spatial features and the row's \agy{4}{read disturbance vulnerability}, which \agy{4}{requires} testing all rows in a DRAM bank. Third, \om{4}{we propose} a \agy{4}{mechanism that leverages our novel experimental observations} to reduce the performance overheads of existing read disturbance solutions.} 
} 

% \begin{itemize}
%     \item Copy from \cite{orosa2021adeeper}
%     \item Include both \cite{orosa2021adeeper} and \cite{luo2023rowpress}
%     \item In contrast, our paper characterizes all of the DRAM rows in a DRAM bank and a bank from all bank groups in a DRAM rank. 
% \end{itemize}

\head{DRAM Read Disturbance Solutions}
\gf{0}{Many prior works propose hardware-based~\hwBasedRowHammerMitigations{} and software-based~\swBasedRowHammerMitigations{} \om{4}{techniques} to prevent RowHammer bitflips, including various approaches, e.g., 
\agy{4}{1)~refreshing potential victim rows \refreshBasedRowHammerDefenseCitations{};
2)~selectively throttling memory accesses \om{5}{that might cause bitflips} \throttlingBasedRowHammerDefenseCitations{};
3)~physically isolating an aggressor row from sensitive data \isolationBasedRowHammerDefenseCitations{}; and}
4)~enhancing DRAM circuitry to mitigate RowHammer effects~\circuitBasedRowHammerDefenseCitations{}. Each approach has different trade-offs \om{5}{in terms of} performance impact, \om{5}{energy overhead, hardware complexity}, and security guarantees. Our goal in this \agy{3}{chapter} is \emph{not} to propose a new read disturbance solution, but rather to provide a \emph{new method} to make the existing solutions more efficient. As we show in \om{5}{\secref{svard:sec:adaptation},} on \agy{4}{\param{five} evaluated} state-of-the-art solutions, Svärd can \emph{significantly} reduce the overheads of read disturbance solutions.}

\head{{\om{5}{RowHammer} Attacks}}
{Many previously proposed RowHammer attacks~\exploitingRowHammerAllCitations{} \om{4}{identify} the rows at the desired vulnerability level (e.g., templating) to increase \agy{4}{the attack's} success probability. This step fundamentally differs from our characterization because it is enough for an attacker to identify a few rows at the desired vulnerability level. In contrast, as a defense-oriented work, we identify the vulnerability level of \om{4}{\emph{all}} DRAM rows \agy{4}{in a DRAM bank} to configure read disturbance solutions correctly without compromising their security guarantees. Therefore, this \agy{3}{chapter} presents a significantly more \om{4}{detailed chip-level} characterization compared to \om{4}{related attack} works.}
% \begin{itemize}
%     \item Copy from \cite{orosa2021adeeper}
%     \item Merge the ones mentioned in \cite{mutlu2023fundamentally}
%     \item Double-check with \cite{yaglikci2022hira}
%     \item This paper does \emph{not} propose a new RowHammer mitigation mechanism but provides a new method of making the existing mechanisms more efficient. 
    
% \end{itemize}

==> mainmatter/06_svard/sections/stale_framework.tex <==
\section{SVÄRD}
\label{svard:sec:svard}
% Use \X{} instead of writing SVÄRD all the time.
\X{} is a framework that performs three steps. First, it profiles the vulnerability of a given module's DRAM rows to read disturbance. Second, it performs a series of data analyses to select a set of row address features that can be correlated with the row's RowHammer vulnerability. Third, it adapts the aggressiveness of existing RowHammer mitigation mechanisms based on the potential victim row's RowHammer vulnerability.



==> mainmatter/07_blockhammer/00_abstract.tex <==
\begin{abstract}
  Aggressive memory density scaling causes modern DRAM devices to suffer from \rowhammer{}, a phenomenon where rapidly {activating} (i.e., {{hammering}}) a DRAM row can cause {bitflips} in physically-{nearby} rows. {Recent studies demonstrate that modern DDR4/LPDDR4 DRAM chips, including chips previously {marketed as} \rowhammer{}-safe, are even more vulnerable to \rowhammer{} than older DDR3 DRAM chips.} {Many works show} that attackers can exploit \rowhammer{} bitflips to reliably mount system-level attacks to escalate privilege and leak private data. 
%   Therefore, it is critical to protect all DRAM-based systems from \rowhammer{} \agy{bitflips.} 
  Therefore, it is critical to {ensure \rowhammer{}-safe operation on all DRAM-based systems as they become increasingly more vulnerable to \rowhammer{}}.
%   {while their \rowhammer{} vulnerability increasingly worsens}.
  Unfortunately, state-of-the-art \rowhammer{} mitigation mechanisms face two {major} challenges.
%   First, recent studies have demonstrated that modern DDR4/LPDDR4 DRAM chips, including chips previously thought to be \rowhammer{}-safe, are even more vulnerable to \rowhammer{} than older DDR3 DRAM chips, yet 
  First, {they} incur {increasingly {higher} performance and/or area {overheads} when {applied to more vulnerable DRAM} chips}.
  Second, {{they}} require {either} closely-guarded proprietary information about the DRAM chips' physical circuit layouts {or modifications to {the} DRAM chip {design}.}
%   \agycomment{Only increasing refresh rate and naive throttling mechanisms do not have the compatibility issues. I think saying ``{all} RH mitigation mechanisms require'' can be an overclaim. I keep state-of-the-art here.}
%   \agycomment{Removing the word `compatibility' from the last sentence makes it harder to connect to the benefits we mention at the end of the abstract.}
  % Unfortunately, modern DRAM chips{, including {chips previously thought to be} \rowhammer{}-safe,} {have been demonstrated to be} more vulnerable to \rowhammer{} than ever. State-of-the-art mitigation mechanisms face two main challenges to be effective and easy-to-adopt for all DRAM-based systems: {(1)~{they scale poorly} with increasing \rowhammer{} vulnerability due to prohibitively large performance overheads in projected future devices; and (2)~{they have} limited compatibility with DRAM chips, {as the mechanisms require proprietary information about the chips}.}

  {In this \agy{3}{chapter}, we show that it is possible to efficiently and scalably prevent RowHammer bitflips without knowledge of or {modification} to DRAM internals.} {To this end, we}
  introduce \blockhammer{}, a low-cost, effective, and easy-to-adopt {RowHammer mitigation} mechanism that prevents all \rowhammer{} bitflips {while overcoming the two key challenges.}
  \blockhammer{} selectively throttles memory accesses that could {otherwise potentially cause} \rowhammer{} bitflips.
  \agyscsc{The key idea of BlockHammer is to (1) {track row activation rates using} area-efficient Bloom filters, and (2) use {the tracking data} to ensure that no row is ever activated rapidly enough to induce RowHammer bitflips.}{SC1}
  %, unlike
  %The key idea of \blockhammer{} is to intelligently track and limit a DRAM row's average access rate and {\emph{proactively}} throttle a {likely} \rowhammer{} attack from within the memory controller{, unlike
  % thereby comprehensively preventing all \rowhammer{} bitflips. Unlike
%   state-of-the-art mechanisms that \emph{reactively} mitigate the disturbance effects of a \rowhammer{} attack only after the attack occurs.
    By guaranteeing that no DRAM row ever {experiences} a {\rowhammer{}-{un}safe} activation rate, \blockhammer{} {(1)} makes it impossible for a \rowhammer{} bitflip to {occur} {and (2) {greatly} reduces a \rowhammer{} attack's impact on the performance of {co-running} benign applications}.
%   , unlike}
%   % thereby comprehensively preventing all \rowhammer{} bitflips. Unlike
%   state-of-the-art mechanisms that {\emph{reactively} mitigate} the disturbance effects of a \rowhammer{} attack {when the attack occurs}.
% , \blockhammer{} proactively prevents any possibility of a \rowhammer{} bitflip by making it impossible to access a DRAM row frequently enough to induce \rowhammer{} failures.
%   \agy{BlockHammer achieves this by effectively throttling an attacker's row activations, which also reduces the attacker's impact on the performance of benign applications.}
%   Because \blockhammer{} prevents \omone{an attacker} from activating rows at a high enough rate to induce \rowhammer{}, \blockhammer{} not only prevents bitflips, but also effectively throttles the attacker, which reduces the attacker's impact on the performance of benign applications.
% mitigates the performance overhead of a \rowhammer{} attack on concurrently running benign applications by throttling the attack.
%   We evaluate \blockhammer{} and show that it is the first mechanism that scales efficiently {as} {DRAM chips {become more vulnerable to}} \rowhammer{} while being compatible with commodity DRAM chips.
%   \agyc{Minesh and I think that commodity seems to be more comprehensive (anything that can be bought and sold) than off-the-shelf (which sounds more restricted to end-user products). Therefore, we prefer just commodity.} DRAM chips.}
{Our evaluations across a comprehensive range of {280~workloads}
% \sgc{need to add in single-thread workload count}\agyc{done}\sgc{undone - that was not what I meant. First, isn't this count (250) inconsistent with Section 7 (which says 125)? Second, you also have single-core results, so it seems weird to just say multiprogrammed workloads here. Is the full number 250+31=281? Third, only use workloads to describe bundles, and applications for single-thread.}\agyc{It is 125 with no RowHammer attack present + 125 RowHammer attack present. You are correct that it makes a total of 281. }
show that, compared to {the best of six} state-of-the-art \rowhammer{} mitigation mechanisms (all of which require knowledge of or {modification} to DRAM internals), \blockhammer{} {provides}}
% \mpl{We evaluate \blockhammer{} relative to state-of-the-art \rowhammer{}-mitigation mechanisms that require knowledge of or modification to DRAM internals. We show that \blockhammer{} achieves} 
  {(1)~competitive performance and energy when the system is not under {a} RowHammer attack and (2)~significantly better performance and energy when the system is under a RowHammer attack. \exttwo{BlockHammer's source code is openly and freely available~\cite{safari2021blockhammer}.}}
% \omp{To our knowledge, this is the first work \agy{that prevents \rowhammer{} bitflips efficiently and scalably without knowledge of or modification to DRAM internals.}}
  
%   \omp{To our knowledge, this is the first work \agy{that prevents \rowhammer{} bitflips efficiently and scalably without knowledge of or modification to DRAM internals.} \mpl{We evaluate our mechanism, BlockHammer, showing that it provides} performance and energy competitive with existing work that requires knowledge of or modification to DRAM internals when the system is not under RowHammer attack and significantly better performance and energy than such work when the system is under a RowHammer attack. }
%   
%   \agyc{I merged scaling and compatibility benefits to make the claim safe. Increased refresh rate and proactive throttling are the only compatible ones but neither of them scales well with increasing vulnerability.} 
%   \agyc{Therefore, these claims are true when we include Graphene among the prior works too because Graphene also relies on reactive refresh operations that brings up the compatibility issue.}
%   (1)~scales efficiently with the increasing \omone{vulnerability of DRAM chips to} \rowhammer{} and (2)~is compatible with all commodity DRAM chips.
\end{abstract}


==> mainmatter/07_blockhammer/01_introduction.tex <==
\section{Introduction}
\label{sec:introduction}

{Improvements to manufacturing process technology {have} increased DRAM storage density by reducing DRAM cell size and cell-to-cell spacing for decades.}
% DRAM storage density has \omone{increased} for decades as improvements to manufacturing process technology \agy{has led} to reductions in DRAM cell size and cell-to-cell spacing.
Although such optimizations improve a DRAM chip's cost-per-bit, they negatively impact {DRAM reliability~\cite{mutlu2013memory, meza2015revisiting}.} Kim et al.~\cite{kim2014flipping} show that modern DRAM chips are susceptible to the \rowhammer{} phenomenon, where opening and closing {(i.e., \emph{activating} and \emph{precharging})} a DRAM row {(i.e., \emph{aggressor row})} at a \emph{high enough} rate (i.e., {\emph{hammering}}{)} can cause {bitflips} in {physically-nearby} rows (i.e., {\emph{victim rows}})~\cite{redeker2002aninvestigation, mutlu2017therowhammer, yang2019trapassisted, mutlu2019rowhammer_and}.
% stale citations: konishi1989analysis, kim2015architectural, mandelman2002challenges
% where accessing a row can disturb stored values in physically nearby rows, and \emph{enough} accesses can cause bitflips in affected cells.
%A \rowhammer{} bitflip can occur in a DRAM row when a physically nearby row is repeatedly opened (activated) and closed (precharged) at a high rate over an extended period of time (i.e., \emph{hammered})~\cite{konishi1989analysis, m2002challenges, redeker2002aninvestigation, kim2015architectural, mutlu2017therowhammer, yang2019trapassisted, mutlu2019rowhammer_and}.
{Many} works demonstrate various system-level attacks using \rowhammer{} to escalate privilege or {leak} private data (e.g.,~\cite{seaborn2015exploiting, vanderveen2016drammer_deterministic, gruss2016rowhammerjs_a, razavi2016flip, pessl2016drama_exploiting, xiao2016onebit, bosman2016dedup, bhattacharya2016curious, qiao2016anew, jang2017sgxbomb, aga2017when,
mutlu2017rowhammer, tatar2018defeating ,gruss2018another, lipp2018nethammer,
van2018guardion, frigo2018grand, cojocar2019eccploit,  ji2019pinpoint, mutlu2019rowhammer, hong2019terminal, kwong2020rambleed, frigo2020trrespass, cojocar2020rowhammer, weissman2020jackhammer, zhang2020pthammer, rowhammergithub, yao2020deephammer}).
% \agyc{added Deephammer~\cite{yao2020deephammer}}
% add yao2020deephammer if there is space
% \agytdinline{Cross-check these references with the references in Onur's HiPEAC talk and add missing ones. See the commented out text for the link}
% https://people.inf.ethz.ch/omutlu/pub/onur-RowHammer-SEHAS-Keynote-HiPEAC-January-19-2021-final.pdf
{Recent} findings {indicate} that \rowhammer{} is a more serious problem than ever and {that} it is {expected to worsen for future DRAM chips}~\cite{mutlu2017therowhammer, mutlu2019rowhammer_and, kim2020revisiting}.
{Therefore,} comprehensively protecting {DRAM} against all types of \rowhammer{} attacks is essential for {the security and reliability of} current and future DRAM-based {computing} systems. 

\setstretch{0.8}
{Although DRAM {vendors} {{currently implement}}} {in-DRAM \rowhammer{} mitigation mechanisms, e.g., target row refresh~\cite{lee2014green, micron2014sdram, jedec2015low, jedec2021jesd235d, jedec2017, frigo2020trrespass}},
% in-situ countermeasures (e.g., TRR~\cite{lee2014green, micron2014sdram, jedec2021jesd235d}),} 
recent works report that commodity {DDR3~\cite{park2016statistical}, DDR4~\cite{pessl2016drama_exploiting, aga2017when, frigo2020trrespass, cojocar2020arewe, kim2020revisiting}, and LPDDR4~\cite{kim2020revisiting}} chips {remain vulnerable to \rowhammer{}}.
In particular,  TRResspass~\cite{frigo2020trrespass} shows that an attacker can still reliably {induce} \rowhammer{} {bitflips} {in commodity (LP)DDRx DRAM chips} by circumventing the in-DRAM mitigation mechanisms. Kim et al.~\cite{kim2020revisiting} show that from 2014 to 2020, DRAM chips {have become} significantly more vulnerable to \rowhammer{} {bitflips}, {with} over an order of magnitude reduction in the required number of {row} activations to induce a {bitflip} (from 139.2k to 9.6k).
% DRAM chips available in the market are \omone{still vulnerable} to \rowhammer{}. 
% \agycomment{Cleaned up citations}
% not only susceptible to \rowhammer{}, but their \rowhammer{} vulnerability significantly increased in the last decade~\cite{kim2020revisiting}. Even worse, {a recent work} reports reliable and successful attacks on the chips that are promoted as \rowhammer{}-safe~\cite{frigo2020trrespass}.
% \omone{C}omprehensively protecting \omone{DRAM} against all types of \rowhammer{} attacks is essential for \omone{the security and reliability of} current and future DRAM-based systems.

% Unfortunately, the state-of-the-art in \rowhammer{} mitigation research faces two major challenges towards building effective and easy-to-adopt \rowhammer{} mitigation mechanisms.
% First, two high-level approaches for mitigating \rowhammer{} are \emph{reactive refresh} that refreshes victim rows as a reaction to venkatesan2006retentionaware row activations from within the processor chip~\cite{kim2014flipping, aweke2016anvil, son2017making, seyedzadeh2018mitigating, you2019mrloc, lee2019twice, kim2020revisiting} and ensuring \emph{physical isolation} between sensitive data and potential attacker's memory space in memory allocation~\cite{konoth2018zebram, vanderveen2018guardion, brasser2016cant}.
Given the severity of \rowhammer{}, {various} mitigation methods have been proposed, which we classify into four {high-level} approaches:
($i$)~\emph{increased refresh rate}, which {refreshes \emph{all}} rows more frequently to reduce the probability of a successful {bitflip}~\cite{apple2015about, kim2014flipping};
($ii$)~\emph{physical isolation}, which {physically separates sensitive data from {any} potential attacker's memory space (e.g., by adding buffer rows between sensitive data regions and other data)~\cite{konoth2018zebram, vanderveen2018guardion, brasser2017cant};}
% ensures \agy{a physical distance between sensitive data and \om{any} potential attacker's memory space such that hammering a row cannot incur \sg{bitflips} in sensitive data~\cite{konoth2018zebram, vanderveen2018guardion, brasser2017cant};} 
% that the system software allocates sensitive data in a memory region that is physically distanced from a potential attacker's memory space
% % \agyc{@Minesh: what is the correct way of saying this? from within? just within? or at?..}
% % which {separates} rows that contain sensitive data from a potential attacker's memory space 
% (e.g., by inserting a buffer row in between {the two regions})~\cite{konoth2018zebram, vanderveen2018guardion, brasser2017cant}; 
($iii$)~\emph{reactive refresh}, which observes row activations
% within the memory controller 
and refreshes the potential victim rows as a reaction to venkatesan2006retentionaware row activations~\cite{kim2014flipping, aweke2016anvil, son2017making, seyedzadeh2018mitigating, you2019mrloc, lee2019twice, park2020graphene}; and
{($iv$)~\emph{proactive throttling}, which {limits} {row activation} rates~\cite{greenfield2016throttling, mutlu2018rowhammer, kim2014flipping} to {\rowhammer{}-safe levels}.}
Unfortunately, each of these four approaches faces at least one of two major challenges towards effectively mitigating \rowhammer{}.
% \agyc{I think the problem is \mpk{that we tried} dismissing the first two approaches immediately here. Instead, we discuss all four approaches for scalability and two for compatibility in this version.}
% % \agycomment{Drafting something here: Unfortunately, despite (3) increased refresh rate was employed in the past, it is not a practical solution for current DRAM chips because it can incur up to 80\% performance overhead when configured for the vulnerability level of current DRAM chips~\cite{kim2020revisiting}. Similarly, (4) proactive throttling incurs prohibitively large overheads with respect to either performance or area because it either unnecessarily throttles benign applications or requires implementing a counter per DRAM row to track its activation rate through the entire refresh window (e.g., \SI{64}{ms}). We discuss these limitations in detail in Section~\ref{sec:qualitative_analysis}.}
% Unfortunately, prior works show that both {(1)} increasing the refresh rate and {(2)} \om{naive} proactive throttling are prohibitively expensive approaches with respect to performance and area
% % \agyc{One implementation of proactive throttling requires implementing a counter per row, which is area expensive.} 
% overheads {at the vulnerability level of current DRAM chips}~\cite{kim2014flipping, kim2020revisiting, mutlu2018rowhammer} 
% % and (3) physical isolation mechanisms have critical weaknesses (e.g., inability to track all DRAM activations) that make them vulnerable to carefully crafted RowHammer attacks~\cite{kim2020revisiting,gruss2016rowhammerjs_a, gruss2018another, cojocar2019exploiting, zhang2019telehammer, kwong2020rambleed,vanderveen2016drammer_deterministic, tatar2018throwhammer} 
% (discussed further in Section~\ref{sec:qualitative_analysis}). 
% Therefore, {(3)} physical isolation and {(4)} reactive refresh {remain as} the {most feasible two approaches} {{today}}. However, {state-of-the-art physical isolation~\cite{vanderveen2018guardion, konoth2018zebram, brasser2017cant} and reactive refresh mechanisms~\cite{kim2014flipping, son2017making, you2019mrloc, seyedzadeh2018mitigating ,lee2019twice, park2020graphene}} 
%in practice}. %only two practical approaches that prior work adopts.
% However, \omone{both} of these two \omone{general} approaches
% {face} two major challenges towards effectively mitigating \rowhammer{}.
% \agycomment{We can also classify these methods such that (3) and (4) are compatible but expensive, while (1) and (2) are not as expensive as (3) and (4), but (1) and (2) intrinsically have compatability problems, and they can have performance costs going to future.} 
% \vspace{0.5em}


\nind
\head{{Challenge} 1: {Efficient Scaling as \rowhammer{} Worsens.}}
% \agyc{We go for noindent everywhere.}
% \mpc{is it okay to say ``as \rowhammer{} worsens''?}
% \textbf{\omone{Challenge} 1: \mpk{Efficient Scaling with \rowhammer{} Vulnerability.}}
% \nind
% \textbf{\omone{Challenge} 1: \agy{Scaling with Worsening RowHammer Trends}.\\}\agytdinline{I dislike the word ``trends''. Can we think of something that means Vulnerability but as short as Trends? One option can be Bug, which is common across SW-level RH papers, but I do't like that as well.}
% As DRAM \agy{vendors} continue to {reduce} the minimum feature size in newer DRAM {generations}, they add in-DRAM \rowhammer{} mitigation mechanisms to compensate for the increased circuit-level interference resulting from \mpj{process technology} scaling~\cite{jedec2015low, jedec2017}.
% \agycomment{Scaling the feature size should not be bounded by an interface standard. Is it important to specify DDR4 here? {Yes it is - many DDR3 chips don't have in-DRAM mechanisms.  It's important for the second half of the sentence more than anything else}}
% with in-DRAM \rowhammer{} mitigation mechanisms
% Despite the existence of in-DRAM mechanisms, recent works~\cite{frigo2020trrespass, kim2020revisiting} demonstrate the ability to induce \rowhammer{} bitflips on off-the-shelf commodity DDR4 DRAM chips.  TRResspass~\cite{frigo2020trrespass} shows that an attacker can still reliably use \rowhammer{} bitflips to circumvent system security measure{s}. 
% Kim et al.~\cite{kim2020revisiting} shows that from 2014 to 2020, DDR4 DRAM chips became significantly more vulnerable to \rowhammer{} bitflips {because} the number of activations required to induce a bitflip decreased by over an order of magnitude (from 139.2k to 4.8k). \agycommment{I think it makes more sense to keep 4.8k here because the relevant experiment in Jeremie's paper hammers each aggressor row for 4.8k times. Per-aggressor row hammer count is important because the state-of-the-art RH mitigation mechanisms somehow measure \emph{per-row} activation rates to trigger their protection mmechanisms. }
% \agycomment{this decrease is just 29x. It is closer to 10x than 100x. {Good point. Reverting.}}
% However, a recent work~\cite{frigo2020trrespass} shows that an attacker can still reliably induce \rowhammer{} bitflips on modern commodity DDR4 DRAM chips from three major vendors that implement these in-DRAM \rowhammer{} mitigation mechanisms.
% % On top of unreliable \rowhammer{} mitigation mechanisms,
% {Another recent work reports that the required hammer count to induce a bitflip has decreased more than an order of magnitude in the last five years (139k in 2014, 4.8k in 2019)~\cite{kim2020revisiting}.}
% These findings show that \rowhammer{} is a more serious problem than ever, and {that} it is {expected to worsen for future DRAM chips}~\cite{mutlu2017therowhammer, mutlu2019rowhammer_and, kim2020revisiting}.
% \agytdinline{Define scalability first. EDIT: minesh did so; check it}\agyc{I think we can define scalability as... [SEE SOURCE - truncated todonote]} 
% CONTINUED NOTE: { ``protecting a DRAM chip with reasonable costs while its \rowhammer{} vulnerability increases''. Of course, reasonable is subjective here, but maybe we can define some target upper bounds for each of performance and area costs based on some observations on design decisions that industry made in the past. Any ideas? Would it be ok to refer to the costs of security extensions like SGX stuff?}
{As DRAM chips become more vulnerable to \rowhammer{} {(i.e., \rowhammer{} {bitflips} can occur at significantly lower row activation {counts} than before)}, {{mitigation mechanisms} need to act more aggressively.}} 
{A} \emph{scalable} mechanism {should} exhibit acceptable performance, energy, and area overheads as its design is reconfigured for more vulnerable DRAM chips. Unfortunately, as chips become more vulnerable to \rowhammer{}, {most} state-of-the-art mechanisms of all four approaches either cannot easily adapt because they are based on fixed design points, or their performance, energy, and/or area overheads become increasingly significant.
%  that cannot easily adapt to different \rowhammer{} vulnerability levels, 
% \agy{Ideally, a \emph{scalable} \rowhammer{} mitigation mechanism's design should efficiently scale with worsening \rowhammer{} vulnerability and its overheads in terms of performance, energy, and area should not become prohibitively expensive. Unfortunately, state-of-the-art mechanisms of all four approaches either propose fixed design points that cannot be scalable, or their performance, energy, and/or area overheads hurt their scalability.}
% Unfortunately, all four types of mitigation approaches...
% {Unfortunately, for all four types of mitigation approaches, the increased \agy{performance, energy, and/or area overheads} to adapt to the increased vulnerability result in significant \emph{scalability limitations}.}
% \mpk{Unfortunately, \sg{for existing mechanisms from all four approaches,} this 
% % impacts each mechanism's \emph{scalability}, necessitating 
% requires provisioning additional resources to 
% % detect\agyc{some of them mitigate without detecting} and 
% mitigate \rowhammer{} attacks. \sg{Each} of the four approaches suffers from different % \emph{scalability limitations} in terms of area and performance.}
% % \agy{Unfortunately, \mpk{each approach suffers from serious limitations as } 
% \agyc{@All, Could you address these two comments: ``of'' and ``to prevent all \rowhammer{} bitflips''. My pdf reader renders them in weird places. I'm not sure where they point at.}
($i$)~{Increasing the refresh rate further {in order to prevent all \rowhammer{} {bitflips}} is 
{prohibitively expensive,}
% intrinsically \emph{not} possible, 
even for {existing} DRAM chips~\cite{kim2020revisiting}, due to the large number of rows that {must} be refreshed within a refresh window.
{($ii$)}~P}hysical isolation mechanisms {must} provide {greater} isolation (i.e., increase the physical distance) between sensitive data and a potential attacker's memory space {as DRAM chips become denser and more vulnerable to \rowhammer{}}. 
% by allocating larger buffers. 
This is because 
% scaling in manufacturing technology reduces both cell size and cell-to-cell spacing, 
denser chip designs bring circuit elements closer together,
which increases the {number of} rows across which the hammering {of} an aggressor row can induce \rowhammer{} {bitflips}~\cite{kim2014flipping, mutlu2017therowhammer, yang2019trapassisted, kim2020revisiting}. {P}roviding {greater} isolation (e.g., increasing the number of buffer rows between sensitive data and an attacker's memory space) both wastes increasing amounts of memory capacity and reduces the fraction of physical memory that can be protected from \rowhammer{} attacks.
% \mpc{I think citing the need for more memory is silly. Most papers show the opposite because a reasonable machine does not overprovision expensive memory.}
% either} increases the \agy{wasted} memory capacity, which is critical for many DRAM-based systems\agytdinline{cite}, \agy{and reduces the fraction of DRAM chip that can be protected from \rowhammer{} attacks.}
%\agycomment{TODO: add citations}
{($iii$)}~Reactive refresh mechanisms need to increase the rate at which they refresh potential victim {rows.} {P}rior {work~\cite{kim2020revisiting}} shows that state-of-the-art {reactive refresh} \rowhammer{} mitigation mechanisms
% either cannot scale with increasing RowHammer vulnerability, or 
{lead to prohibitively large performance overheads with increasing RowHammer vulnerability.}
% \agyc{We should not add energy here because~\cite{kim2020revisiting} does not discuss energy.}
% when used for chips with higher \rowhammer{} vulnerability.}
% , since RowHammer bitflips \jkc{is expected to occur after significantly fewer activations in modern and future DRAM chips.} can occur at significantly lower row activation rates. 
{($iv$)}~{Existing proactive} throttling approaches {must throttle {activations} at a more aggressive rate to counteract the increased \rowhammer{} vulnerability.}
% , which incurs} either significant performance or area overheads
% , \jk{as they} \sg{must throttle at a greater rate. 
{This requires either throttling} row activations of benign applications {as well} or {tracking} per-row activation rates for the entire refresh window, 
% \jk{both of} which make them 
{incurring prohibitively-expensive performance or area overheads} {even {for} existing} DRAM chips~\cite{kim2014flipping, mutlu2018rowhammer}.
% \agyc{@Minesh, is there a flow problem here, or is that ok because we go like 1,2,3...? @Giray: I think it is ugly but OK. I made some edits, and it should be very clear what (1-4) represent.}
% \omc{make it flow}
% \agy{We discuss the scalability challenge in detail for all four approaches in Section~\ref{sec:qualitative_analysis}.}}
% Unfortunately, {as the} \rowhammer{} vulnerability of {a DRAM chip increases}, state-of-the-art \rowhammer{} mitigation mechanisms~\cite{lee2019twice} either no longer apply as originally proposed or suffer prohibitively large performance overheads (up to 80\%)~\cite{kim2020revisiting}.


% \textbf{\omone{Challenge} 2: Compatibility.} Both \emph{reactive \mpj{refresh}} and \emph{physical isolation} require the ability to {either (1)~}identify all possible victim rows that can be affected by
% % experience a \rowhammer{} bitflip after
% hammering a given row, or {(2)~}modify the DRAM chip to perform {mitigation.}
% % (i.e., refreshing victim rows or allocating barriers between memory regions).
% \mpj{Unfortunately, both of these properties prevent applicability to commodity DRAM chips. Identifying the exact victim row(s) affected by a \rowhammer{} attack, i.e., rows physically nearby to aggressor row(s), requires knowing the 
% % so they cannot be applied to commodity DRAM chips whose physical row arrangements are proprietary secrets.}
% % because {the mechanisms} cannot identify victim rows without {knowing the}
% \emph{proprietary} mapping scheme that the chip uses to internally translate memory-controller visible row addresses to physical row addresses}~\cite{smith1981laser, amrutur2001fast, lee2017designinduced}.
% % Row  address  remapping  allows  DRAM  vendors to  optimize  the  physical layout of DRAM chip according to their density, performance, and power demands
% DRAM vendors apply this in-DRAM row address remapping to (1)~optimize their chip design for density, performance, and power demands~\cite{amrutur2001fast}; and (2)~improve the chip's reliability by remapping faulty rows to redundant rows {during post-manufacturing testing}~\cite{keeth2001dram_circuit, smith1981laser}.
% Design-induced remapping is different for every vendor and differs even across different DRAM models and generations. Faulty row remapping is \mpj{necessary due to manufacturing process variation, so} it is different across individual chips within a particular model.
% % Therefore, every vendor, DRAM model, generation, and individual chip can implement a different remapping scheme.
% However, vendors do not share this remapping scheme because it {contains} insights into the chip design and manufacturing quality~\cite{lee2017designinduced}.
% % % Note that this row remapping can contain insights into the density-optimized chip design and vendor's manufacturing quality. \todo{restructure} Also it can vary across DRAM vendors, chip generations, and individual chips.
% % As a result, reactive mitigation and physical isolation approaches are limited to systems that
% % restrict their compatibility to specific (e.g., custom) DRAM modules
% % % either customize their DRAM chips
% % or already possess proprietary information about every possible DRAM chip that they will ever use.
% As a result, reactive mitigation and physical isolation approaches are limited to systems that
% obtain proprietary information or {modify DRAM to support} new commands that internally use this proprietary information.
% % \agycomment{For example, in case a processor vendor agrees with a DRAM vendor on a customized command that refreshes victim rows without revealing the physical layout, the processor vendor does not need to possess the proprietary information, but it restricts itself to this customized DRAM chip/interface. {See Overleaf comments.}}
% % Second, as
% \vspace{0.5em}

\setstretch{0.77}
\nind
\head{{Challenge} 2: Compatibility with Commodity DRAM Chips.} 
Both {($ii$)} physical isolation and {($iii$)} reactive refresh mechanisms require the ability to either (1)~identify \emph{all potential victim rows} that can be affected by hammering a given row or (2)~modify the DRAM chip
% \jkc{such that the potential victim rows are internally isolated within the chip or the RowHammer mitigation mechanism can accurately issue reactive refreshes to a victim row.} 
such that {either} the potential victim rows are internally isolate{d} within the {DRAM} chip or the \rowhammer{} mitigation mechanism can accurately issue reactive refreshes to {all} potential victim {rows}.
% \omc{Fix all instances of row(s)}\agyc{done} 
% {so that the \rowhammer{} mitigation mechanism can ensure isolating or refreshing them.}\agyc{We use \emph{or} here because if they can identify victim rows somehow, they do not need to any modifications to the DRAM chips as they can simply activate victim rows.}
{Identifying all potential victim {rows} requires knowing the mapping {schemes} that {the DRAM chip} uses to internally {translate} memory-controller-visible row addresses to physical row addresses~\cite{kim2014flipping, smith1981laser, horiguchi1997redundancy, keeth2001dram_circuit, itoh2001vlsi, liu2013anexperimental,seshadri2015gatherscatter, khan2016parbor, khan2017detecting, lee2017designinduced, tatar2018defeating, barenghi2018softwareonly, cojocar2020arewe,  patel2020bitexact}}.
% ~\cite{kim2014flipping, smith1981laser, horiguchi1997redundancy, keeth2001dram_circuit, itoh2001vlsi, liu2013anexperimental,seshadri2015gatherscatter, khan2016parbor, lee2017designinduced, tatar2018defeating, cojocar2020arewe, lee2019twice, barenghi2018softwareonly}}. 
{Unfortunately,} DRAM vendors consider their in-DRAM row address mapping schemes to be highly \emph{proprietary} and do not reveal any details in {publicly-available} documentation, as these details contain insights into the chip design and manufacturing quality~\cite{smith1981laser, horiguchi1997redundancy, keeth2001dram_circuit, itoh2001vlsi, lee2017designinduced, patel2020bitexact}
% ~\cite{kim2014flipping, smith1981laser, horiguchi1997redundancy, keeth2001dram_circuit, itoh2001vlsi, liu2013anexperimental,seshadri2015gatherscatter, khan2016parbor, khan2017detecting, lee2017designinduced, tatar2018defeating, barenghi2018softwareonly, cojocar2020arewe,  patel2020bitexact}\agyc{removed SRAM decoder paper from Horowitz} 
(discussed in Section~\ref{sec:background_physicallayout}). 
As a result, both physical isolation and reactive {refresh} are limited to systems that can {(1)}~obtain such proprietary information on {in-}DRAM row address mapping or {(2)}~modify DRAM chips internally. 

% \nind
% \textbf{\omone{Challenge} 2: Compatibility \agy{with Commodity DRAM Chips}.} 
% \agy{Both physical isolation and} reactive refresh \agy{mechanisms} require the ability to either (1)~identify \emph{all potential victim rows} that can be affected by hammering a given row, or (2)~modify the DRAM \omone{chips} to \agy{ensure either (i) physical isolation or (ii) victim row refresh in the DRAM chip}.
% \mpj{Unfortunately, both of these properties prevent applicability to \emph{commodity} DRAM chips. 
% \agy{First,} \omone{i}dentifying \agy{all potential} victim row(s) requires knowing the 
% % so they cannot be applied to commodity DRAM chips whose physical row arrangements are proprietary secrets.}
% % because {the mechanisms} cannot identify victim rows without {knowing the}
% \emph{proprietary} mapping \omone{schemes} that \omone{the DRAM chip} uses to internally \agy{remap} memory-controller-visible row addresses to physical row addresses}~\cite{smith1981laser, amrutur2001fast, lee2017designinduced}.
% \omone{Such} in-DRAM row address remapping \agy{allows DRAM vendors} (1)~to optimize their chip design for density, performance, and power \omone{constraints}~\cite{amrutur2001fast}; and (2)~\agy{to silently replace faulty or weak rows that could have reduced factory yield with redundant rows during post-manufacturing~\cite{keeth2001dram_circuit, smith1981laser, horiguchi1997redundancy}}. \agy{Therefore, in-DRAM row address remapping schemes can vary with DRAM chip design and manufacturing process variation across vendors, models, and even chips within a particular DRAM model.} 
% % \omone{a} chip's reliability by remapping faulty rows to redundant rows during post-manufacturing testing~\cite{keeth2001dram_circuit, smith1981laser, horiguchi1997redundancy}.
% DRAM vendors \agy{consider their in-DRAM row address remapping schemes to be highly proprietary and ensure not to reveal remapping details in any public documentation}
% % different for every vendor and differs even across different DRAM models and generations. Faulty row remapping is \mpj{necessary due to manufacturing process variation, so} it is different across individual chips within a particular model.
% % Therefore, every vendor, DRAM model, generation, and individual chip can implement a different remapping scheme.
% % However, vendors do not share this remapping scheme 
% because \agy{in-DRAM row address remapping} contains insights into the chip design and manufacturing quality~\cite{smith1981laser, horiguchi1997redundancy, keeth2001dram_circuit, amrutur2001fast, lee2017designinduced}. 
% % \agy{Therefore,} \omone{such DRAM-internal} remapping \agy{can be different across vendors, DRAM models, and chips \agy{due to variation in both design and  manufacturing process}.} 
% % % Note that this row remapping can contain insights into the density-optimized chip design and vendor's manufacturing quality. \todo{restructure} Also it can vary across DRAM vendors, chip generations, and individual chips.
% % As a result, reactive mitigation and physical isolation approaches are limited to systems that
% % restrict their compatibility to specific (e.g., custom) DRAM modules
% % % either customize their DRAM chips
% % or already possess proprietary information about every possible DRAM chip that they will ever use.
% As a result, both physical isolation and reactive \agy{refresh} approaches are limited to systems that \omone{can (1)}
% obtain \omone{such} proprietary information or \omone{(2)} modify DRAM \omone{chips internally.}
% % to support new commands that internally use this proprietary information.
% % \agycomment{For example, in case a processor vendor agrees with a DRAM vendor on a customized command that refreshes victim rows without revealing the physical layout, the processor vendor does not need to possess the proprietary information, but it restricts itself to this customized DRAM chip/interface. {See Overleaf comments.}}
% % Second, as

\head{Our goal} in this \agy{3}{chapter} is to design a {low-cost, effective,} and easy-to-adopt \rowhammer{} mitigation mechanism that (1)~scales efficiently with worsening \rowhammer{} vulnerability to prevent \rowhammer{} {bitflips} in current and future DRAM chips,
% highly-vulnerable DRAM chips against all \rowhammer{} attacks, 
and (2)~is {seamlessly} compatible with \emph{commodity} DRAM chips{,} without requiring {proprietary information about or} modifications to {DRAM chips}.
To this end, we propose BlockHammer, a new {proactive throttling-based} RowHammer mitigation mechanism, \exttwo{which is openly and freely available~\cite{safari2021blockhammer}}.
% \mpj{that achieves both of our design goals}. 
{\blockhammer{}'s key idea is} to track row activation rates using area-efficient Bloom filters and use the tracking data to ensure that no row is ever activated rapidly enough to induce RowHammer {bitflips}.
Because \blockhammer{} requires no proprietary information about or modifications to DRAM chips, it can be implemented completely within the {memory controller}.
% \mpl{Because \blockhammer{} is fully implemented within the processor die, it does not require any proprietary information about or modifications to DRAM chips.} 
Compared to prior works that require proprietary information or DRAM chip modifications, \blockhammer{} {provides} (1)~competitive performance and energy when the system is not {under a {\rowhammer{}}} attack and (2)~significantly better performance and energy {({average/maximum} of 45.0\%{/61.9\%} and 28.9\%{/33.8\%}, respectively)} when the system {\emph{is}} {under a \rowhammer{}} attack. To our knowledge, this is the first work that prevents \rowhammer{} {bitflips} efficiently and scalably without {knowledge} of or modification to DRAM internals.

% \agyscsc{To this end, we propose BlockHammer, a new RowHammer mitigation mechanism based on proactive throttling with a novel design that reduces the high performance and area costs of prior proactive throttling mechanisms.
% The \textbf{key idea} of BlockHammer is to track per-row activation rates using area-efficient Bloom filters and throttle activations to rows such that no row is ever activated rapidly enough to induce RowHammer bitflips.}{SC1}
% \textbf{Our goal} in this \agy{3}{chapter} is to design an effective and easy-to-adopt \rowhammer{} mitigation mechanism that (1)~is \emph{compatible with all} commodity DRAM chips, and (2)~{scales efficiently to \emph{comprehensively} protect}
% % systems with
% highly-vulnerable DRAM chips against all \rowhammer{} attacks.
% \agyprpr{To this end, we propose BlockHammer, a new mechanism for proactive throttling that avoids the high costs of prior throttling mechanisms.
% The \textbf{key idea} of BlockHammer is to enable efficient proactive throttling of a RowHammer attack, by tracking per-row activation rates using area-efficient Bloom filters and using data from the filters to ensure that no row is ever activated rapidly enough to induce RowHammer bitflips.}{PR1}
% The \textbf{key idea} of BlockHammer is to track per-row activation rates by leveraging area-efficient Bloom filters and to enable \emph{proactive throttling} of a RowHammer attack's memory accesses, such that no attack can activate a row at a high enough rate to hammer a DRAM row or waste memory bandwidth.}{PR1}
% The \textbf{key idea} of \blockhammer{} is to track per-row activation rates by leveraging area-efficient Bloom filters and to enable \emph{proactive throttling} of a \rowhammer{} attack's memory accesses, such that the attack can neither activate a row at a high enough rate to hammer a DRAM row nor waste memory bandwidth.}{PR1}
% Stale version of the key idea
% The \textbf{key idea} of \blockhammer{} is to \emph{proactively throttle} the memory accesses of a \rowhammer{} attack,
% % at the memory controller (which resides on the processor chip),
% such that the attack can never activate a row at a high enough rate to hammer a DRAM cell.
% Unlike \agy{state-of-the-art RowHammer mitigation} mechanisms, \blockhammer{} needs \emph{no knowledge} of
% % the physical DRAM layout, avoiding the need for 
% proprietary information from \agy{vendors or no modifications to DRAM chip/protocol}, and scales efficiently with \rowhammer{} vulnerability.\agycomment{@Minesh, is this sentence too complicated?}
% {\blockhammer{} is fully implemented within the processor die 
% % (i.e., in the memory controller with minor changes to last level cache (LLC) and direct memory access (DMA) controller that we discuss in Section~\ref{sec:hammerthrottler}), 
% and does not require any proprietary information about or modifications to DRAM chips.}
% \agycomment{Consistency check! within the memory controller -> within the processor die.}
% {Unlike state-of-the-art \rowhammer{} mitigation mechanisms, \blockhammer{} both
% % \agyc{This claim is true even when considering Graphene because we say ``both''.} 
% (1) scales efficiently with increasing \rowhammer{} vulnerability of DRAM chips and (2) {is compatible with} commodity DRAM chips.}

% \textbf{The key idea} of \blockhammer{} is to \emph{proactively throttle} the memory accesses of a \rowhammer{} attack from within the memory controller in the processor chip such that the attack cannot activate a row at a high enough rate to disturb any DRAM cell.
% % {\blockhammer{} prevents any possibility of a \rowhammer{} bitflip occurring in a victim row without identifying it}
% \blockhammer{} comprehensively observes all memory accesses, limits each row's activation rate, and proactively throttles all \rowhammer{} attacks{. Thus, \blockhammer{}} both mitigates the performance and energy overheads of a \rowhammer{} attack, and avoids wasting memory bandwidth and capacity that reactive refresh and physical isolation approaches would waste respectively. Therefore, \blockhammer{} provides a comprehensive protection to systems with highly vulnerable DRAM chips against all \rowhammer{} attacks.
% Since \blockhammer{} does not need to identify victim rows, it does not require any proprietary information, and it is compatible with all DRAM chips. \agycomment{is ``it'' clear in the previous sentence?}

\nind
\head{Key Mechanism.} {\blockhammer{} consists of two components: \emph{\rowblocker{}} and \emph{\hammerthrottler{}}.}
% \blockhammer{} consists of two {components}: \emph{\rowblocker{}} and \emph{\hammerthrottler{}}.
\emph{\rowblocker{}} {tracks and limits the activation rates of DRAM rows {to a rate lower than %the minimum rate}\agyc{Minesh could you help fixing this?}
% that are being hammered
% tracks each DRAM row that is being hammered and limits 
% the maximum number of activations the row can experience 
% to below the minimum row activation count within a single refresh window,} 
at} which \rowhammer{} bitflips begin to occur, i.e., the \emph{\rowhammer{} threshold} (\nrh{}).}
% \mpc{I rewrote this to define \nrh{} more fluidly. doublecheck.}
% tracks and limits the activation rates of DRAM rows that are being hammered \mpm{so that no row's activation count can reach a large enough value to induce \rowhammer{} bitflipsthe minimum value necessary to induce a \rowhammer{} bitflip, i.e., \emph{\rowhammer{} threshold} (\nrh{}), before all potential victim rows are refreshed.}\agyc{I define \rowhammer{} threshold here. A bit convoluted... Any suggestions?}
% To be able to track each row's activation rate in an area-efficient way,
{To track activation rates in an area-efficient manner,}
% \mpc{make ``rate'' and ``count'' consistent here}
\rowblocker{} employs {a false-negative-free variant of} counting Bloom filters~\cite{fan2000summary, li2012compression} {that eliminates the need for per-row counters.}
% {Instead, a counting Bloom filter maintains a limited number of counters and uses a hash function to map each DRAM row address to a small subset of these counters.}
% extend conventional Bloom filters by replacing each element with a counter.
% A counting Bloom filter lookup returns {an} upper bound {for} the number of activations {to a given row}. 
% \rowblocker{} \agy{\agytwo{identifies} a row to throttle \agytwo{its} further activations (i.e., \emph{blacklists}) \mpc{this makes no sense - unclear antecedents. rephrase?}\agyc{Is it any better now?} if the row's activation count 
% \rowblocker{} {\emph{blacklists}} {a} row \agy{(i.e., marks \mpj{the row to throttle} further activations targeting the row)} whose \agy{activation count}, within a given \agy{time} interval, exceeds a predefined threshold 
{When \rowblocker{} observes that a row's activation count} {within a given time interval exceeds a predefined threshold} {(which we set to be smaller than 
{\nrh{}})},
% the minimum number of activations required to trigger a \rowhammer{} {bitflip})},
% {\rowblocker{} \emph{blacklists} the row, throttling subsequent activations that target the row to within a \rowhammer{}-safe activation rate.}\agytdinline{poor writing, revise}
% \omc{Something about this sentence became worse.
% Blacklisting is in the title, so it is fine to define here.
% ``Throttles all activations'' gives the feeling that all activations are prevented. We should not give that feeling to the reader.}
% \agyc{I defined blacklisting again in this version. To me this seems correct.}
{\rowblocker{} {\emph{blacklists} the row, i.e.,}
{flags the row as a potential {aggressor row} and limits further activations to the row}
% marks the row to} throttle \agy{its activation rate}
% \om{the rate of} subsequent activations {to} the row 
until the end of the time interval, {ensuring that} the row's overall activation rate {never reaches} a \rowhammer{}-unsafe level.}
% Any subsequent activations to a blacklisted row are throttled {(i.e., delayed by a certain amount of time)} to stay within a {\rowhammer{}-safe activation} rate.
% that guarantees to never exceed the \rowhammer{} activation threshold.  
As a result, \rowblocker{} ensures that a successful {\rowhammer{}} attack is impossible. 
% \rowblocker{} is implemented fully in the memory controller, and does not require \agy{any proprietary information about or changes to DRAM chips.}  

% \rowblocker{} blacklists a DRAM row when its activation rate reaches a predefined threshold value and limits its activation rate by delaying {successive} activations targeting the blacklisted row. This ensures that all rows observe a safe average activation rate, {thereby} always preventing all \rowhammer{} bitflips. We implement \rowblocker{} entirely in the memory controller {within} the processor {die} so that (1) \blockhammer{} does not require any modifications to DRAM chips or any piece of their proprietary information {because} it does not need to identify victim rows, and (2) it \emph{comprehensively} observes all memory accesses and protect a DRAM chip from all \rowhammer{} attacks.
% While \rowblocker{} slows down a workload that attempts to perform a \rowhammer{} attack (in order to prevent the attack from occurring), it results in less than 1\% performance overhead for benign (i.e., non-attacking) workloads, as benign workloads' per-row activation rates rarely exceed the blacklisting threshold.

{\emph{\hammerthrottler{}} alleviates the performance degradation {a \rowhammer{} attack {imposes on} benign applications.} 
To do so, \hammerthrottler{} reduces the memory bandwidth usage of an attacker thread by applying a quota to the thread's total number of in-flight memory requests for {a determined} time {period}. \hammerthrottler{} {sets} the quota for each thread inversely proportional to the rate at which the thread activates a blacklisted row. As a result, \hammerthrottler{} reduces the memory bandwidth consumed by an attacker, thereby allowing concurrently-running benign applications to have {higher {performance}} when accessing memory.} {To further mitigate the performance impact of \rowhammer{} attacks, \hammerthrottler{} can optionally} expose {the rate at which each thread activates a blacklisted row}
% \agy{each thread's blacklisted row activation rate} 
% information 
to the operating system {(OS)}. {{This information can} be used as a {dependable} indicator of a thread's likelihood of performing a \rowhammer{} attack, enabling the OS to} employ more sophisticated {thread} scheduling and quality-of-service support.
% \agycomment{I think this can be a sufficient explanation of what \hammerthrottler{} is. I commented out the old text in the source file. I basically omitted the definitions like RH likelihood and attacker process. Do you feel a lack of essential information? }
% \emph{\hammerthrottler{}} reduces the memory bandwidth usage of a \rowhammer{} attack, and alleviates the performance degradation that the attack would cause to concurrently-running benign applications. 
% To do so, \hammerthrottler{} models a process's \emph{\rowhammer{} likelihood} as proportional to the rate at which it activates blacklisted rows.
% An attacking process (i.e., a process that causes a DRAM row to be blacklisted) is assigned a quota to the total number of memory requests it can make to any row for an upcoming window of time.
% As a process's \rowhammer{} likelihood increases, \hammerthrottler{}
% reduces the \mpj{process's} quota. By reducing the quota of a likely attacker, the system's memory bandwidth is freed up, allowing concurrently-running benign applications to have better quality-of-service when accessing memory.
% applies a smaller quota to the on-the-fly memory request count of the process. Therefore, concurrently running benign applications can benefit from the memory bandwidth that a \rowhammer{} attack would {otherwise} waste. Our evaluation shows

We evaluate \blockhammer{}'s (1)~security guarantees via a mathematical proof in \secref{mech_security}; (2)~area, {{static} power, access energy,} and latency overheads for storing and accessing metadata by using circuit models~\cite{muralimanohar2009cacti, synopsyssynopsys} in \secref{blockhammer_areaoverhead}; {and} (3)~performance and {DRAM} energy {overheads} using {cycle-level}
% \agyc{changed everywhere in the paper} 
simulations~\cite{Kim2016Ramulator, safariramulator, chdrampower_opensource} {in \secref{evaluation}}.
% and (4) energy overhead by using a DRAM power model~\cite{chdrampower_opensource} in~\secref{evaluation}.
{Our evaluations {for a realistic \rowhammer{} threshold (32K activations {within a \SI{64}{\milli\second} refresh window}~\cite{kim2020revisiting})} show that \blockhammer{} guarantees \rowhammer{}-safe operation with {only} 0.06\% area, {0.7\% performance}, and {0.6\%} {DRAM} energy overheads for benign (i.e., non-attacking) workloads,
% \agyc{do we need to indicate somehow that perf and energy are average numbers, or is it already obvious?} 
compared to a baseline system with no \rowhammer{} mitigation}.
% \agytdinline{update these numbers}
When a \rowhammer{} attack {exists} within a multiprogrammed workload, \blockhammer{} successfully identifies and throttles {the} attacker's {row activations} with 99.98\% accuracy,
% \omc{Identifies an attacker with 99.98\% accuracy and throttles its memory requests
% Is what I wrote more accurate?
% What is currently written can be misinterpreted or not understood}\agyc{This accuracy is based on identifying a row activation rather than the attacker itself} 
{resulting} in a 45.0\% {average}
% \agytdinline{update}
improvement in the performance of concurrently-running benign applications.
% \omc{Are these values across all HCfirst values?}\agyc{These values come from \nrh{}=32K.}
% compared to a system without throttling.
% \agycomment{I replaced the 90\%tile result with 100\%tile to make it easier to understand}
% By \agy{reducing the memory bandwidth usage of the threads that are detected to be \rowhammer{} attacks,}
% % and freeing up bandwidth,
% \hammerthrottler{} improves the performance of benign applications by 17.8\%, on average, when an attack is attempted, compared to a system without throttling.
% \agycomment{``while the attacker is running'' part can be a bit confusing. One can get the takeaway like we throttle the attack, but the attack is running. Also, ``performance improvement'' without a ``compared to'' confused a reviewer before, causing that guy to focus too much on the evaluation. {Any better?}}
{We show that} 
% \blockhammer{}'s Bloom filter-based \rowhammer{} detection mechanism and throttling-based prevention mechanism allow \blockhammer{} to 
\blockhammer{} {more efficiently scales} {with increasing \rowhammer{} vulnerability} {than six state-of-the-art \rowhammer{} mitigation mechanisms,} {without requiring knowledge of or {modification} to the internals}
of DRAM chips.
% {while remaining} compatible with commodity DRAM chips.
% {By doing so,} \blockhammer{} {mitigates} the performance {degradation that} an attack {can inflict upon} benign applications, avoiding the scalability issues of prior mechanisms
% {that negatively impact} performance by {performing} refresh operations {on potential} victim rows.
% the attack, \hammerthrottler{} mitigates a \rowhammer{} attack's {negative impact on the} performance {of} concurrently running benign applications by 17.81\% on average.
% {By proactively throttling the attacker, \blockhammer{}} scales better with increasing \rowhammer{} vulnerability {than state-of-the-art mechanisms that reactively refresh victim rows}.


% \blockhammer{} provides an optional interface to the operating system (OS)
% % and fairness or quality-of-service (QoS) concerning mechanisms
% so that {the OS} can use each process's \rowhammer{} likelihood to enable \rowhammer{}-aware process scheduling to improve system-wide performance, fairness, and quality of service.
% \agycomment{We don't mention the interface to the OS at all in this version. I'm not a big fan of promoting it while we don't discuss in detail in the rest of the paper, however, I'd like to state it somehow to give a message like: ``This paper is not a cut-and-dry mechanism paper. On the contrary, there already is some future research in this direction.'' There was a question like: ``Does this \agy{3}{chapter} enable future research?'' in some review forms if I remember. {See Overleaf comment.}}

% To evaluate \blockhammer{}, we{, first,}
% \agy{We evaluate \blockhammer{}'s (1) security guarantees (\secref{mech_security}), area and latency overheads, (\secref{blockhammer_areaoverhead}), and performance and energy overheads (\secref{evaluation}). 
% We demonstrate that \blockhammer{} guarantees \rowhammer{}-safe operation through a mathematical proof. We estimate the area and latency overheads of \blockhammer{} by using CACTI SRAM model~\cite{muralimanohar2009cacti} and Synopsys DC~\cite{synopsyssynopsys}.  
% We evaluate \blockhammer{}'s performance by performing \om{cycle-level} simulations, using Ramulator~\cite{Kim2016Ramulator},  and estimate its impact on DRAM energy consumption by using DRAMPower~\cite{chdrampower_opensource}.}

% simulation results with state-of-the-art \rowhammer{} mitigation mechanisms~\cite{kim2014flipping,son2017making, you2019mrloc, seyedzadeh2018mitigating, lee2019twice}.}\agycomment{TODO: Graphene}

% We show that \blockhammer{} is compatible with all commodity DRAM chips and scales better than prior mechanisms \agy{by improving benign workload performance by 17.8\% on average} as the \rowhammer{} vulnerability of DRAM chips increases.\agycomment{@Minesh: I think this whole paragraph can be removed because it is redundant with the evaluation information we share individually for rowblocker and hammerthrottler in their paragraphs. What do you think? Is it better to keep both, or remove one or another?}

{{Building} on analyses done by prior work on \rowhammer{} mitigation~\cite{kim2014flipping, gruss2018another, mutlu2017therowhammer, mutlu2018rowhammer, mutlu2019rowhammer_and, kim2020revisiting}, we {describe} in \secref{qualitative_analysis} that a low-cost, effective, and easy-to-adopt \rowhammer{} mitigation mechanism must:}
% To thoroughly compare \blockhammer{} to prior work, we study
% five key properties that determine whether or not each mechanism is \agy{\emph{low-cost}, \emph{effective}, and \emph{easy-to-adopt}} across all DRAM-based systems: 
(1)~{address} a \emph{comprehensive threat model}, (2)~{be {seamlessly} compatible} with {\emph{commodity}} DRAM chips {(i.e., {require no knowledge of or modifications to} DRAM chip internals)}, (3)~\emph{scale} {efficiently} with increasing \rowhammer{} vulnerability, {and} (4)~\emph{deterministically} {prevent} all \rowhammer{} attacks. 
% \agytdinline{Properties are consistent with Sec 9, but the wording has slight differences, e.g., when we talk about  @All, please double-check if that is ok or we should change them.} 
% \agyc{Fifth property was low-cost, which is redundant with scalability. I cut it.}
% , and (5)~{be} \emph{low cost} in terms of performance, energy, \agy{and area} overheads.
We find that, among all {14}
% \agyc{Note that this 15 includes \blockhammer{}}
\rowhammer{} mitigation mechanisms that we examine, \blockhammer{} is the \emph{only} {one} that satisfies all {four} key properties. 

We make the following contributions in this work:
% \omc{Redo. Focus on insights. Do not be verbose or mech. centric}\agyc{I drafted a new version. @All, please express your opinions.}
% \agyc{Minesh, can/should we try merging the first two bullet points to save some space?}:
\squishlist
 \item{{{We introduce the first mechanism that} efficiently and scalably {prevents} \rowhammer{} bitflips \emph{without} knowledge of or {modification} to DRAM internals.
 % We show this with a novel, effective, and low-cost mechanism, BlockHammer, which 
 {Our mechanism,} \blockhammer{}, 
 provides {competitive} performance and energy  with {existing {\rowhammer{} mitigation} mechanisms} when the system is \emph{not} under {a} RowHammer attack, and \emph{significantly} better performance and energy {than} existing {mechanisms} when the system \emph{is} {under a RowHammer} attack.}}
 \item {We show that a proactive throttling approach {to prevent} \rowhammer{} bitflips can be implemented efficiently using Bloom filters. We employ a variant of counting Bloom filters that {(1)~avoids} the area and energy overheads of per-row counters used by prior {proactive throttling mechanisms}, and {(2)~never} fails to detect a \rowhammer{} attack.}
%  \omc{This is in the right direction but written carelessly. Proofread and revise.}
 % \item{\agy{We introduce a low-cost and effective \rowhammer{} detection and prevention mechanism, \rowblocker{}, which uses area-efficient Bloom filters to distinguish benign row activations from potential aggressor row activations. \rowblocker{} blacklists and throttles activations targeting potential aggressor rows with a false positive rate less than 0.012\%.}}
 \item {We show that we can {greatly} reduce the performance {degradation} {and energy wast{ag}e} a \rowhammer{} attack {inflicts on benign threads} {and the system} by {accurately identifying the \rowhammer{} attack thread and reducing its memory bandwidth usage. {We introduce a new metric called the {\emph{\rowhammer{} likelihood index}}, {which} enables the memory controller to distinguish a \rowhammer{} attack from a benign thread.}}}
%  \agyc{I think this conveys the essential message. @Saugata, could you check if this draft misses any info that you put before? Please see Onur's comments in the source.}
%  throttling the memory accesses of threads that attempt to hammer a DRAM row.  
%  \rowhammer{} attack throttling reduces the memory interference experienced by co-running benign applications. 
%  To enable \rowhammer{} attack throttling, we provide the first mechanism that can accurately identify \rowhammer{} attackers before a bitflip takes place.}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%ONUR'S COMMENTS ARE HERE
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%  \omc{I think you are still confusing the throttling that is done in contribution 2 and the throttling that is done here. We need to more carefully distinguish them. 
%  Last contribution is about identifying RowHammer attack threads accurately and much more aggressively preventing them from destroying the performance of benign threads. That is it.  Now massage this into good writing,
%  If you start talking about throttling memory accesses in the last contribution, like you are doing now, then you create a mess because one would say that is exactly contribution 2...
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

 % \item{\agy{We introduce a memory access throttling mechanism, \hammerthrottler{}, to alleviate the performance degradation a \rowhammer{} attack inflicts on co-running benign applications. \hammerthrottler{} leverages the blacklisting information and throttles memory accesses of threads that attempt to hammer a DRAM row. By doing so, \hammerthrottler{} improves the performance of benign workloads by 45.0\% on average during a \rowhammer{} attack compared to a baseline with no \rowhammer{} mitigation.}}
%  \item {We {introduce} \rowblocker{}, a new \rowhammer{} detection and prevention mechanism that tracks {row activation} rates using area-efficient Bloom filters. {\blockhammer{} {identifies} and blacklists} {rows with high activation rates}. {\rowblocker{} ensures} that each DRAM row observes a RowHammer-safe activation rate {by throttling activations to blacklisted rows}.
%  {By doing so, \rowblocker{} prevents \rowhammer{} bitflips entirely, at low performance and area costs, and without any proprietary information about or changes to DRAM chips.}}
%  By doing so, \rowblocker{} prevents potential attackers from inducing {\rowhammer{}} bitflips in DRAM. \rowblocker{} is {low-cost} in terms of both area {($<0.06\%$)}
% %  \agyc{@Ataberk, another instance is here}
%  and performance {($<1\%$)} \mpl{and prevents} \rowhammer{} without the need for any proprietary information {about} or {changes to DRAM chips}.}
 % \item We propose \blockhammer{}, a new secure and practical \rowhammer{} mitigation mechanism. {\blockhammer{} applies a novel approach called proactive throttling that achieves better scalability with increasing \rowhammer{} vulnerability of DRAM chips and does not require any proprietary data of or modifications to the commodity DRAM chips.}
 % To our knowledge, \blockhammer{} is the first {\rowhammer{} mitigation mechanism that is} effective and easy-to-adopt {for modern and future DRAM chips.}
%  that is compatible with all commodity DRAM chips and scales well with their increasing \rowhammer{} vulnerability.
%  \blockhammer{} prevents \rowhammer{} bitflips by blacklisting DRAM rows that are in potential danger of exceeding their \rowhammer{} threshold, limiting their access rates by imposing delays and throttling the processes that constantly try activating blacklisted rows. \blockhammer{} is implemented fully in the memory controller and is compatible with commodity DRAM chips.
%  \item {We {introduce} \hammerthrottler{}, a mechanism that {alleviates the performance degradation} {a} \rowhammer{} attack can {inflict on} benign workloads.
% {\hammerthrottler{} tracks {the number of activations from each thread that target}
% }\mpl{each thread's \sg{activations} that target} 
% blacklisted rows. \hammerthrottler{} throttles a thread's memory requests as the {thread's activation count of blacklisted rows exceeds a predefined threshold.}
% activates blacklisted rows \mpk{a greater} number of times.}
%  \hammerthrottler{} {detects a thread performing \rowhammer{} attack by tracking the rate at which the thread activates the rows blacklisted by \rowblocker{} with high (97.2\%) precision and reduces the memory bandwidth consumption of the thread by applying a quota to the thread's memory requests. 
% By doing so, \hammerthrottler{} improves benign workload performance by 45.0\% on average during a \rowhammer{} attack compared to a {baseline with no \rowhammer{} mitigation.}}}
%  uses the row tracking information from \rowblocker{} to determine which \agy{threads} in a system are likely to be attackers with \agy{high (97.2\%) precision}, and reduces these processes' bandwidth utilization for use by benign applications.}
 % \item We provide an interface by which \blockhammer{} can report a malicious process that is performing a \rowhammer{} attack to the operating system. Our evaluation shows that \blockhammer{} can successfully identify a real \rowhammer{} attack with less-than a 0.2\% false-positive rate across the 90th percentile of all DRAM row activations.
 % \item{\agy{We introduce four properties necessary for a \rowhammer{} mitigation mechanism to be \emph{low-cost}, \emph{effective}, and \emph{easy-to-adopt}. We qualitatively evaluate 15 state-of-the-art \rowhammer{} mitigation mechanisms from four classes and show that \blockhammer{} is the only mechanism that possesses all four properties.}}
%  \item {We show that \blockhammer{}, our proposed {\rowhammer{} mitigation mechanism} that combines \rowblocker{} {and} \hammerthrottler{}, is the only {existing} mechanism that meets the {four} properties necessary for a \rowhammer{} mitigation mechanism to be \emph{low-cost}, \emph{effective}, and \emph{easy-to-adopt}. \blockhammer{} prevents \rowhammer{} {bitflips} {at low performance, energy, and area overheads; scales efficiently with increasing \rowhammer{} vulnerability; and is compatible} with commodity DRAM chips and protocols.} 
%  even as the \rowhammer{} vulnerability of a DRAM chip scales up, with minimal {performance, energy, and area overheads without losing compatibility with commodity DRAM chips and protocols}.}
 % \item We identify five characteristics that a \rowhammer{} mitigation mechanism should satisfy in order to be effective and easy-to-adopt for comprehensively protecting current and future DRAM-based systems against all \rowhammer{} attacks. We demonstrate that \blockhammer{} is the only \rowhammer{} mitigation mechanism that satisfies all five characteristics, while key prior works either incur large performance overheads or cannot be directly applied to the overwhelming majority of systems that use commodity DRAM chips.
\squishend
% \agycomment{I like this version of contributions more than the previous one. My only hesitation is that we mention three mechanism names here. Even though we explicitly say that RowBlocker and HammerThrottler are two components of BlockHammer, I'm a bit worried that an careless reader can get confused which one is which. {I wouldn't worry much. Reviewers aren't that careless, generally.}}




    % Many prior works propose \rowhammer{} mitigation mechanisms, but \om{none {of them} satisf{ies} all of the five characteristics at the same time.}
    % Several of these mitigation techniques patch software-level components (e.g., BIOS, firmware, and operating system)~\cite{kim2014flipping, apple2015about, LenovoRefInc, enterprise2015hp, brasser2016cant, aweke2016anvil, irazoqui2016mascat, vanderveen2018guardion,  konoth2018zebram, li2019detecting}.
    % Such techniques can be deployed in existing systems, as they require no hardware changes.
    % However, their software-only approaches either induce high performance and energy overheads (e.g., 35\% performance overhead for increased refresh rates~\cite{kim2014flipping}), or provide limited security guarantees (e.g., constraining the threat model to only DMA-based attacks~\cite{vanderveen2018guardion}, or assuming a secure hypervisor~\cite{konoth2018zebram}).
    % Other works~\cite{kim2014flipping, son2017making, ghasempour2015armor, you2019mrloc, seyedzadeh2018mitigating, lee2019twice, kang2020cat} propose hardware-level \rowhammer{} mitigation techniques, which, unlike software-only approaches, can accurately observe each individual DRAM row activation. These works mitigate \rowhammer{} by refreshing DRAM rows (i.e., victim rows) that are physically nearby a hammered row (i.e., aggressor row).
    % As a result, they provide an effective and low-cost defense against a comprehensive threat model, where an attacker has the highest order of privileges in all layers of the software stack.
    % Unfortunately, each of these mechanisms suffers from at least one of the following issues:
    % (1)~requires a-priori knowledge of, or the ability to reverse engineer the physical row mapping to identify and refresh victim rows in a \rowhammer{} attack, limiting its compatibility to DRAM chips with known physical mappings,
    % (2)~non-deterministic security guarantees due to a reliance on probabilistic procedures to trigger the mechanism,
    % or (3)~limited scalability {with increasing DRAM density and \rowhammer{} vulnerability} due to significant overheads and {limited} security guarantees~\cite{kim2020revisiting}.
    % We provide an analysis of these limitations in Section~\ref{sec:motivation_practicality}.
    % {We demonstrate that \om{no prior mechanism satisfies all five {characteristics through our analysis in Section~\ref{sec:motivation} (summarized in Table~\ref{table:current_mechanisms})}. The closest one, \twice{}~\cite{lee2019twice} satisfies {three} of them, but misses out on two key {characteristics which are 1) compatibility with commodity DRAM chips and 2) scalability with increasing \rowhammer{} vulnerability.}}}
    %
    % \input{section3/motivation_table_alternative}
    %
    % \textbf{Our goal} in this work is to develop a \om{new} \rowhammer{} mitigation mechanism \om{that satisfies all five characteristics {of an effective, practical, and widely-applicable \rowhammer{} mitigation mechanism}.}
    % \mpf{To this end, we introduce \blockhammer{}, a new \rowhammer{}-mitigation mechanism that satisfies each of these requirements.}
    %
    % \textbf{The key idea} of \blockhammer{} is to {intelligently track and} limit the activation rate \om{of the} DRAM rows that are being hammered by delaying activations to these rows.
    % {Unlike prior \rowhammer{} mitigation mechanisms that are based on fixing potentially affected DRAM rows or physically isolating sensitive data, \blockhammer{} deterministically prevents the possibility of activating a single DRAM row enough times to induce \rowhammer{} failures \emph{without requiring} (1) modification\agy{s} to the DRAM chip or (2) knowledge of the physical organization of DRAM rows.}
    % {\blockhammer{}} \om{modifies the} memory request scheduler to \om{temporarily} block row activations targeting a row that is being hammered (i.e., an aggressor row).
    % {To do so, \blockhammer{} \mpf{monitors DRAM accesses from within the memory controller and tracks all rapidly-activated rows using a hardware-efficient \emph{blacklist}. Then, \blockhammer{} enforces}}
    % {a minimum time delay between consecutive activations \mpf{to all blacklisted rows}. This ensures that no row's total activation count within a refresh window can exceed values at which \rowhammer{} bitflips can occur.}
    %
    % \om{\textbf{Mechanism.}} \blockhammer{} continuously monitors each row's activation {count} at low cost using \emph{counting {Bloom filters}}~\cite{bloom1970spacetime, fan2000summary, bonomi2006animproved}, which extend conventional Bloom filters by replacing each {filter} element with a counter. \blockhammer{} increments the counters that correspond to a given row address when the row is activated. \om{A} row is considered \emph{blacklisted} when its activation count exceeds a configurable threshold. Because counters are monotonically increasing, \blockhammer{} can never miss rows that should be blacklisted (i.e., no false negatives) although small amounts of unnecessary blacklisting (i.e., false positives) may occur due to Bloom filter aliasing. To limit a blacklisted row's activation rate, \blockhammer{} maintains a \emph{first-in-first-out} history buffer that tracks the most recent row activations.
    % {A row activation record remains in this history buffer for as long as the minimum delay that \blockhammer{} enforces for blacklisted DRAM rows.}
    % This ensures that all rows observe a safe average activation rate, deterministically preventing all \rowhammer{} bitflips{.
    % \blockhammer{} protects a system against all \rowhammer{} attacks \mpf{because} it observes and \mpf{controls} all main memory accesses in the memory controller regardless of the system resources an attacker can use to mount a \rowhammer{} attack.}
    % \mpf{Unlike prior \rowhammer{} mitigation mechanisms, \blockhammer{} does not require refreshing victim rows or physically isolating sensitive data because it blocks \rowhammer{} attacks by directly throttling the aggressor row's activations. Therefore, \blockhammer{} does not need to know the physical layout of DRAM rows (which is typically proprietary and unknown), and \blockhammer{} is compatible with all commodity DRAM chips.}
    %
    % {To \mpf{determine \blockhammer{}'s} impact on system performance, we evaluate \mpf{it using} an eight-core system with multiprogrammed SPEC06 workloads with varying main memory access characteristics.}
    % We find that \blockhammer{} incurs an average performance overhead of 0.04\% for benign workloads, while improving their performance by 17.81\% when they are under a \rowhammer{}-attack relative to a system without \rowhammer{} protection. {We evaluate \blockhammer{}'s area costs, showing that they scale linearly with the number of DRAM \emph{banks}, regardless of each bank's capacity. For a 4GB DDR3 configuration, \blockhammer{} requires 0.0376\% of processor chip area within the memory controller.}
    % We quantitatively compare these results against state-of-the-art \rowhammer{} mitigation mechanisms and demonstrate that
    % {\blockhammer{} enables a low-cost, effective, and widely-applicable \rowhammer{} prevention that does not require any proprietary information of DRAM chips.}
    %
    % We make the following \textbf{key contributions}:%
    % \squishlist
    %     \item We propose \blockhammer{}, a new secure and practical \rowhammer{} mitigation mechanism. To our knowledge, \blockhammer{} is the first practical mechanism that provides deterministic security guarantees for a comprehensive threat model without requiring any piece of proprietary information or any changes in DRAM chips. \blockhammer{} prevents \rowhammer{} bitflips by \emph{blacklisting} DRAM rows that are in potential danger of exceeding their \rowhammer{} threshold, and limiting their access rates by imposing delays. \blockhammer{} is implemented fully in the memory controller, and is compatible with commodity DRAM chips.
    %
    %     \item \mpf{We provide an interface by which \blockhammer{} can report a malicious process that is performing a \rowhammer{} attack to the operating system and/or any fairness/quality-of-service concerning mechanisms.} Our evaluation shows that \blockhammer{} can successfully identify a real \rowhammer{} attack with less-than 0.2\% false-positive rate across the 90th percentile of the workloads.
    %
    %     \item We identify {five characteristics} that a \rowhammer{} mitigation mechanism should {satisfy} in order to be effective at protecting against \rowhammer{} across a wide spectrum of current and future DRAM-based systems. {We demonstrate that \blockhammer{} is the only \rowhammer{} mitigation mechanism that satisfies all five characteristics, while \mpf{key} prior works either incur large performance overheads or cannot be \mpf{directly} applied to the overwhelming majority of systems that use commodity DRAM chips.}
    % \squishend


==> mainmatter/07_blockhammer/02_background.tex <==
\section{Background}

This section provides a concise overview of (1)~DRAM organization and operation, (2)~the \rowhammer{} phenomenon, and (3)~in-DRAM row address {mapping}. {{{For more detail, we} refer the reader to p}rior works {on DRAM and \rowhammer{}}~\cite{liu2012raidr, liu2013anexperimental, keeth2001dram_circuit, mutlu2007stalltime, moscibroda2007memory, mutlu2008parallelismaware, kim2010atlas, subramanian2014theblacklisting, kim2012acase, kim2014flipping, qureshi2015avatar,
hassan2016chargecache, chang2016understanding, lee2017design,  chang2017understanding,  patel2017reaper,kim2018dram, kim2020revisiting, hassan2019crow, frigo2020trrespass, chang2014improving, chang2016low, vampire2018ghose, hassan2017softmc, khan2016parbor, khan2016case, khan2014efficacy, seshadri2015gather, seshadri2017ambit, kim2018solar, kim2019d, patel2019understanding, patel2020beer, lee2013tiered, lee2015decoupled, seshadri2013rowclone, luo2020clrdram, seshadri2019dram, wang2020figaro}}.
%\agytdinline{put more citations}

\subsection{DRAM Organization and Operation}
Figure \ref{fig:dram_structure} shows the high-level structure of a typical DRAM{-based system}. At the lowest level of the hierarchy, DRAM {stores data within} \emph{cells} {that each consist} of a single capacitor and an access transistor. Each cell encodes a single bit of data using the ``high'' and ``low'' voltage states of the capacitor. Because a DRAM cell leaks charge over time, each cell's charge is periodically restored (i.e., refreshed) (e.g., every 32 or \SI{64}{\milli\second}~\cite{liu2012raidr, liu2013anexperimental, jedec2017, jedec2015low}) to prevent data loss.
% \js{certain time window (e.g., 32 or 64ms~\cite{jedec2017, jedec2015low})}
% to restore the charge in today's chips.
% Cells are logically connected in a hierarchy of two-dimensional arrays 
{Cells are arranged in two-dimensional arrays to form DRAM \emph{banks}.}

% \mpj{Several banks (e.g., 8 to 16) together form a DRAM chip.}
% \agy{called} \emph{subarrays}. \agy{Multiple subarrays form a \emph{bank}.} 
% that in turn combine to form \emph{banks}. 
% At the highest level of the hierarchy, the \emph{memory controller} \mpj{in the CPU die} interfaces with \agy{multiple banks through} a \emph{memory channel}.
% Each channel connects to one or more DRAM \emph{ranks}, \agy{each of} which \agy{is} composed of multiple banks.

\begin{figure}[t]
    \centering
    % \vspace{-8pt}
    \includegraphics[width=\linewidth]{../figs/fig1-crop.pdf}
    % \includegraphics[width=0.45\textwidth, trim = 0 0 0 25, clip]{../figs/dram_structure.pdf}
    % \vspace{-20pt}
    \caption{{Structure of a typical DRAM-based  system.}}
    \label{fig:dram_structure}
    % \vspace{-2mm}
\end{figure}

{DRAM cells in a bank are addressed using \emph{rows} and \emph{columns}. A \emph{wordline} {drives} all DRAM cells in a \emph{row}, and a \emph{bitline} connects all DRAM cells {in} a \emph{column}.}
%\mpj{Each bank addresses a given cell using \emph{rows} and \emph{columns} connected by \emph{wordlines} and \emph{bitlines}, respectively. 
{All rows} within a bank share the peripheral circuitry, so only one row may be accessed per bank at any given time.
% in a given bank
Each row begins in a \emph{closed} (i.e., \emph{precharged}) state and needs to be \emph{opened} (i.e., \emph{activated}) before any READ or WRITE operations can be performed {on it}.
Activating a row fetches the row's contents into the \emph{row buffer}.
% \agyrm{Once \minp{the data is} fetched, all READ and WRITE operations are served from \minp{the row} buffer.}
The row buffer serves all read and write requests after fetching the data.
The row must be \emph{closed} before further accesses can be made to other rows of the same bank.

{A DRAM chip contains multiple banks that can be accessed in parallel. Multiple chips form a DRAM \emph{rank}.}
% The memory controller must obey a set of 
% \agy{vendor}-\omone{defined}\agycomment{@Minesh, is this really vendor defined? doesn't JEDEC have any word on those?} 
% \mpj{standardized} \emph{timing parameters} to ensure that each operation has enough time to complete before starting the next~\cite{jedec2015low, jedec2017}.\agycomment{We need to mention \trc{} and \trefw{} here.} 
% \agy{Two important timing parameters in the scope of \rowhammer{} are (1) the minimum time window between two consecutive row activations targeting the same bank (\trc{}) and (2) the time window between two r }
% For example, the memory controller must satisfy a minimum latency called \trc{} between two consecutive row activations targeting the same bank~\cite{jedec2015low, jedec2017}.\footnote{\trc{} is particularly important in the scope of the \rowhammer{} phenomenon \agy{because a row's activation rate is bounded by one activation per \trc{} time window.}}
%\agyrm{The memory controller interfaces with DRAM using read and write operations at the granularity of a last-level cache (LLC) cache line (e.g., 64B). Modern systems typically use a complex address mapping scheme to convert an application-level memory access into physical DRAM accesses. This includes virtual-to-physical memory address translation, memory-controller-level address translation (e.g., striping addresses across different DRAM channels), and DRAM-internal address translation (e.g., row address hashing). Each level of translation is successively less documented, and the DRAM-internal address translation is typically proprietary and publicly unknown~\cite{lee2017designinduced}.}
% \agyrm{As with commodity capacitors, \agycomment{I think this is not accurate.}}
%A DRAM cell leaks charge over time. To prevent data loss, each cell is refreshed every 32 or 64~\cite{jedec2017, jedec2015low} milliseconds to restore the charge in today's chips.
% \agyrm{Memory controllers uniformly distribute DRAM row refreshes over time by issuing REF commands every 7.8 microseconds. Each REF command refreshes a subset of all DRAM rows. Under normal operation, this timing provides {a large-enough} margin to ensure that even worst-case charge leakage conditions will not result in errors. \agycomment{I think this part does not contribute much.}}
{At the highest level of the hierarchy, the \emph{memory controller} {in the {CPU die}} interfaces with {a DRAM rank} through a \emph{memory channel}. The memory controller serves memory access requests from various system components by issuing DRAM bus commands (e.g., activate, precharge, read, write, and refresh). The memory controller must schedule commands according to standardized \emph{timing parameters}, which are defined {in DRAM datasheets} to ensure that each operation has enough time to complete before starting the next~\cite{jedec2015low, jedec2017, jedec2021jesd235d, jedec2008jesd79f, micron2014sdram}.
The overall strategy that the memory controller uses to schedule commands is known as a \emph{scheduling policy.}}
% The memory controller is responsible for scheduling DRAM bus commands (e.g., activate, precharge, read, write, and refresh) \agy{to service memory access requests of various system components (e.g., CPU/GPU cores and I/O devices).}
% as requests arrive from various system components (e.g., CPU/GPU cores, I/O devices) into the memory controller's request queues.
% The memory controller \omone{services requests} using a \emph{scheduling policy}
{Typical {policies} seek} to optimize performance, fairness, quality of service (QoS), and energy {across applications running on a system}~\cite{rixner00, mutlu2008parallelismaware, kim2010atlas, kim2010thread, ebrahimi2011parallel,  ausavarungnirun2012staged, subramanian2014theblacklisting, subramanian2016bliss, usui2016dash}.
{Therefore, the} scheduling policy effectively controls all accesses to all DRAM channels, banks, rows, and columns.
% For example, a scheduling policy may prioritize a younger request to the already open row over an older request to a row that is closed, since accessing an open row is faster than accessing a closed row~\cite{rixner00}.

\subsection{The \rowhammer{} Phenomenon}

{\rowhammer{} is a DRAM failure mode in which repeated activations to a single row (i.e., \emph{aggressor} row) cause disturbance capable of inducing bitflips in {\emph{physically-nearby}} rows  (i.e., \emph{victim} rows) that are not being accessed~\cite{kim2014flipping}.}
% \rowhammer{} is a memory read disturbance error mechanism in which repeated row activations to a single row may induce errors in \emph{physically adjacent/nearby} rows that are not being accessed~\cite{kim2014flipping}.
% The row that is being rapidly accessed is called an \emph{aggressor row}, and the rows that are affected by this access pattern are called \emph{victim rows}.
{These bitflips manifest after a row's activation count reaches a certain threshold {value} {within a refresh window}, which we call \emph{\rowhammer{} threshold} (\nrh{}) {({{also} {denoted} 
as $MAC$}~\cite{jedec2017} and \smash{$HC_{first}$}~\cite{kim2020revisiting})}.}
% as $MAC$ by DDR4 specifications}~\cite{jedec2017} and $HC_{first}$ by~\cite{kim2020revisiting})}.}
Prior works {study the error characteristics of} \rowhammer{} {bitflips} and show that 
% a certain \agy{activation count is} required before \agy{bitflips} manifest, which we refer as the \emph{\rowhammer{} threshold} (\nrh{}) \agy{(\mpj{referred to as \emph{MAC} in DDR4 specifications}~\cite{jedec2017})}.
% \agyrm{A recent work~\cite{yang2019trapassisted} illuminates this observation by explaining that \rowhammer{} bitflips occur due to a charge pumping process around a rapidly activated word line when the number of activations exceeds a threshold.}
% \agyrm{According to the characterization works~\cite{kim2014flipping, park2016statistical} this}
% \jk{The number of activations}
\nrh{} {varies across {DRAM} vendors, device models, generations, and chips}~\cite{kim2014flipping, park2016statistical,  frigo2020trrespass, kim2020revisiting, cojocar2020arewe}.
% \nrh{} depends on the fabrication process, vendor, device generation, and device and voltage levels of DRAM cells~\cite{kim2014flipping, park2016statistical}.
% Today, DRAM specifications define this threshold for a DRAM chip as a constraint called \mac{} (i.e., \maclong{}).
% Recent DDR4 DRAM chips already report \
% Today, \nrh{} can be obtained from DRAM vendors' reports (e.g., Maximum Activation Count (MAC) in DDR4 chips~\cite{jedec2017}), enabling
% several \rowhammer{} mitigation mechanisms that are based on counting the number of activations per row~\cite{lin2017handling, bains2016rowhammer}.
% Yang et al.~\cite{yang2019trapassisted} show that \nrh{} directly depends on the physical distance between wordlines. 
{Yang et al.~\cite{yang2019trapassisted} explain this \nrh{} variation based on changing physical distances between adjacent wordlines (i.e., physical DRAM rows).}
Since DRAM chip density increases {at smaller feature sizes, both} Yang et al.'s observation and recent experimental studies~\cite{frigo2020trrespass, kim2020revisiting, kim2014flipping} {clearly demonstrate} that \rowhammer{} {worsens with continued technology scaling~\cite{mutlu2017therowhammer, mutlu2019rowhammer_and}}. {In addition, recent studies {show} that emerging memory technologies also exhibit \rowhammer{} vulnerability~\cite{khan2018analysis, mutlu2017therowhammer, mutlu2019rowhammer_and}}.
% , while they are not guaranteed to have TRR
% \agyc{We removed the remaining part of this subsection (which mentions the reduction on $HC_{first}$ from 2014 to 2020) as it was completely redundant with the introduction.}

% I AM UNCERTAIN IF WE NEED THIS PARAGRAPH AT ALL
% THE INTRO TAKES CARE OF THIS!!!
% \mpj{Significant work~\cite{seaborn2015exploiting, qiao2016nontemporal, vanderveen2016drammer_deterministic, gruss2016rowhammerjs_a, razavi2016flip, xiao2016onebit, aga2017when, tatar2018defeating, gruss2018another, lipp2018nethammer, cojocar2019exploiting,  ji2019pinpoint, mutlu2019rowhammer_and, kwong2020rambleed, frigo2020trrespass, cojocar2020arewe} shows that \rowhammer{} bitflips pose a serious security threat that can be exploited to compromise a wide variety of systems. Unfortunately, system security and reliability will continue to suffer as DRAM chips become increasingly vulnerable to \rowhammer{}.}

% THE REST OF THIS PARAGRAPH IS UNORGANIZED, REDUNDANT, AND WEAK!!
% \textcolor{red}{TODO: the following is badly constructed bg material}
% For example, Kim et al.\ report a \rowhammer{} threshold of 139K in their paper in 2014~\cite{kim2014flipping}, while {more} recent experimental data shows that this threshold is already reduced to 4.8k for {a} double-sided \rowhammer{} attack on DRAM chips manufactured in 2019~\cite{frigo2020trrespass, kim2020revisiting}.
% Furthermore, system security and reliability decrease as \rowhammer{} bitflips become easier to induce. Recent works~\cite{frigo2020trrespass, kim2020revisiting} report scalability issues with existing \rowhammer{} mitigation mechanisms
% % \agyrm{show that existing \rowhammer{} mitigation mechanisms {have scalability issues}}
% % \agyrm{will not be able}
% % to efficiently protect
% for future chips, {as the \rowhammer{} vulnerability continues to increase}.
% Therefore, we need a robust mechanism that is capable of preventing \emph{all} \rowhammer{} bitflips for \emph{all} current and future DRAM devices with insignificant performance/energy/hardware cost.
% Unfortunately, previously-proposed techniques have limitations in providing that.
% We discuss the properties of a desirable \rowhammer{} prevention mechanism, and the limitations of the current techniques in satisfying those properties, in \secref{motivation}.

\subsection{{{In-}DRAM Row Address Mapping}}
\label{sec:background_physicallayout}
% \agyrm{To both optimize {DRAM} circuit designs and improve manufacturing yield,}
DRAM vendors {often use {DRAM-internal} mapping} {schemes} to internally translate memory-controller-visible row addresses to physical row {addresses~\cite{kim2014flipping, smith1981laser, horiguchi1997redundancy, keeth2001dram_circuit, itoh2001vlsi, liu2013anexperimental,seshadri2015gatherscatter, khan2016parbor, khan2017detecting, lee2017designinduced, tatar2018defeating, barenghi2018softwareonly, cojocar2020arewe,  patel2020bitexact} for two reasons:}
%smith1981laser, horiguchi1997redundancy, keeth2001dram, itoh2013vlsi,  liu2013experimental, khan2016parbor, lee2017design, khan2017detecting, patel2020beer
% \agyc{where exactly should these citations be? is here ok? is the end of the sentence better?}}
% \agyc{would adding ~\cite{amrutur2001fast} make sense? It discusses area optimization for SRAM decoders, but I think the same concepts apply to DRAM as well}:}\mpc{I think it is okay as-is, and the SRAM citation could be misleading or confusing without explanation}
(1)~to optimize their chip design for density, performance, and power {constraints}; and (2)~{to improve factory yield by mapping the addresses of faulty rows to more reliable spare rows} {(i.e., post-manufacturing row repair).}
% \cite{keeth2001dram_circuit, smith1981laser, horiguchi1997redundancy}.}
{Therefore, row {mapping} schemes can vary {with} (1) chip design {variation} across different vendors, DRAM models, and generations and (2) manufacturing process variation across different chips of the same design}. 
{State-of-the-art \rowhammer{} mitigation mechanisms must account for {both sources of variation in order to}
% \mpc{How do you like phrasing it this way? ``variation'' is still there, but not in the same way}\agyc{That's good}
% because the mechanisms must 
% know the exact 
% DRAM-internal row address mapping scheme to 
be able to {accurately} identify all potential victim rows that are {physically nearby}
% \sgc{nearby is not an adjective, so no hyphen here} 
an aggressor row.}
{{Unfortunately}, DRAM vendors {consider their in-DRAM row address mapping schemes to be highly proprietary and ensure not to reveal mapping details in any public documentation because exposing the row {address} mapping {scheme} can reveal insights into the chip design and factory yield}~\cite{smith1981laser, horiguchi1997redundancy, keeth2001dram_circuit, itoh2001vlsi, lee2017designinduced, patel2020bitexact}}.
% % from {row addresses on the DRAM interface} to physical rows {within the DRAM cell array}. \mpj{Therefore,} result in \agy{mapping contiguous row addresses to be mapped to different } physically-adjacent rows having non-adjacent or even non-similar row addresses. \mpj{Different mappings allow DRAM vendors} to both (1) optimize the physical layout of a DRAM chip according to \mpj{various} density, performance, and power demands~\cite{amrutur2001fast} and \mpj{(2) perform post-manufacturing row repair using redundant on-chip elements to improve factory yield~\cite{smith1981laser,keeth2001dram_circuit}}. 

% As DRAM interface standards do not define or constrain how rows can be \agy{mapped}~\cite{jedec2008jesd79f, jedec2021jesd235d, jedec2015low, jedec2017}, row \mpj{mapping} schemes can vary across different vendors, DRAM models, generations. \agycomment{why isn't this ``..., and generations.''?} 
% % In-DRAM row remapping also allows DRAM vendors to improve their yield by using row redundancy, where faulty rows are mapped to reliable redundant rows in post-manufacturing~\cite{smith1981laser,keeth2001dram_circuit}. 
% \mpj{In particular, as} each chip can experience faulty rows in different locations, the row \mpj{mapping} scheme can also vary across different chips of the same design.

% % , it is typically proprietary and publicly unknown~\cite{lee2017designinduced}. 
% Therefore, the processor cannot know the victim DRAM row \mpj{address(es)} of a \rowhammer{} attack unless it has access to this information, or is capable of reverse-engineering it for any arbitrary DRAM device the system may use.

% \mpj{Unfortunately, this is particularly problematic for \rowhammer{} mitigation mechanisms that rely on reactive refreshing, which requires knowing the victim row addresses to refresh.}
% Note that a \rowhammer{} attack needs to identify only a few rows that are close enough to each other to be successful, while a \rowhammer{} mitigation technique needs to know the exact row address remapping scheme {for every DRAM row in the memory subsystem}.



% \emph{proprietary} mapping \omone{schemes} that \omone{the DRAM chip} uses to internally \agy{remap} memory-controller-visible row addresses to physical row addresses}~\cite{smith1981laser, amrutur2001fast, lee2017designinduced}.
% \omone{Such} in-DRAM row address remapping \agy{allows DRAM vendors} (1)~to optimize their chip design for density, performance, and power \omone{constraints}~\cite{amrutur2001fast}; and (2)~\agy{to silently replace faulty or weak rows that could have reduced factory yield with redundant rows during post-manufacturing~\cite{keeth2001dram_circuit, smith1981laser, horiguchi1997redundancy}}. \agy{Therefore, in-DRAM row address remapping schemes can vary with DRAM chip design and manufacturing process variation across vendors, models, and even chips within a particular DRAM model.} 
% % \omone{a} chip's reliability by remapping faulty rows to redundant rows during post-manufacturing testing~\cite{keeth2001dram_circuit, smith1981laser, horiguchi1997redundancy}.
% DRAM vendors \agy{consider their in-DRAM row address remapping schemes to be highly proprietary and ensure not to reveal remapping details in any public documentation}
% % different for every vendor and differs even across different DRAM models and generations. Faulty row remapping is \mpj{necessary due to manufacturing process variation, so} it is different across individual chips within a particular model.
% % Therefore, every vendor, DRAM model, generation, and individual chip can implement a different remapping scheme.
% % However, vendors do not share this remapping scheme 
% because \agy{in-DRAM row address remapping} contains insights into the chip design and manufacturing quality~\cite{smith1981laser, horiguchi1997redundancy, keeth2001dram_circuit, amrutur2001fast, lee2017designinduced}. 
% % \agy{Therefore,} \omone{such DRAM-internal} remapping \agy{can be different across vendors, DRAM models, and chips \agy{due to variation in both design and  manufacturing process}.} 
% % % Note that this row remapping can contain insights into the density-optimized chip design and vendor's manufacturing quality. \todo{restructure} Also it can vary across DRAM vendors, chip generations, and individual chips.
% % As a result, reactive mitigation and physical isolation approaches are limited to systems that
% % restrict their compatibility to specific (e.g., custom) DRAM modules
% % % either customize their DRAM chips
% % or already possess proprietary information about every possible DRAM chip that they will ever use.
% As a result, both physical isolation and reactive \agy{refresh} approaches are limited to systems that \omone{can (1)}
% obtain \omone{such} proprietary information or \omone{(2)} modify DRAM \omone{chips internally.}
% % to support new commands that internally use this proprietary information.
% % \agycomment{For example, in case a processor vendor agrees with a DRAM vendor on a customized command that refreshes victim rows without revealing the physical layout, the processor vendor does not need to possess the proprietary information, but it restricts itself to this customized DRAM chip/interface. {See Overleaf comments.}}
% % Second, as

==> mainmatter/07_blockhammer/02_motivation_and_goal.tex <==
\section{Motivation and Goal}
\label{blockhammer:sec:motivation_and_goal}
DRAM read disturbance mitigations face two challenges {\secref{sec:background_mitigation}}. 
First, as DRAM chips become increasingly more vulnerable to read disturbance, it becomes increasingly more expensive to prevent read disturbance bitflips~\rowHammerDefenseScalingProblemsCitations{}.
Second, because previously proposed mitigation mechanisms rely on identifying potential victim rows based on the aggressor row's address, they are limited to a system that can obtain this information. Unfortunately, this is a piece of highly proprietary information as it can reveal insights into proprietary DRAM circuitry design and manufacturing quality~\inDRAMRowAddressMappingCitations{}. 


\head{Our goal} in this \agy{3}{chapter} is to design a {low-cost, effective,} and easy-to-adopt \rowhammer{} mitigation mechanism that 1)~scales efficiently with worsening \rowhammer{} vulnerability to prevent \rowhammer{} {bitflips} in current and future DRAM chips,
% highly-vulnerable DRAM chips against all \rowhammer{} attacks, 
and 2)~is {seamlessly} compatible with \emph{commodity} DRAM chips{,} without requiring {proprietary information about or} modifications to {DRAM chips}.
To this end, we propose BlockHammer, a new {proactive throttling-based} RowHammer mitigation mechanism, {which is openly and freely available~\cite{safari2021blockhammer} and already adopted in Ramulator 2~\cite{safari2023ramulator2}, a cycle-level memory simulator}.
% \mpj{that achieves both of our design goals}. 
{\blockhammer{}'s key idea is} to track row activation rates using area-efficient Bloom filters and use the tracking data to ensure that no row is ever activated rapidly enough to induce RowHammer {bitflips}.
Because \blockhammer{} requires no proprietary information about or modifications to DRAM chips, it can be implemented completely within the {memory controller}.
% \mpl{Because \blockhammer{} is fully implemented within the processor die, it does not require any proprietary information about or modifications to DRAM chips.} 
Compared to prior works that require proprietary information or DRAM chip modifications, \blockhammer{} {provides} 1)~competitive performance and energy when the system is not {under a {\rowhammer{}}} attack and 2)~significantly better performance and energy {({average/maximum} of 45.0\%{/61.9\%} and 28.9\%{/33.8\%}, respectively)} when the system {\emph{is}} {under a \rowhammer{}} attack. To our knowledge, this is the first work that prevents \rowhammer{} {bitflips} efficiently and scalably without {knowledge} of or modification to DRAM internals.


==> mainmatter/07_blockhammer/09_table_failedattempt.tex <==

% Minesh- should add a footnote saying what Astersik means
\newcommand{\astfootnote}[1]{
\let\oldthefootnote=\thefootnote
\setcounter{footnote}{0}
\renewcommand{\thefootnote}{\fnsymbol{footnote}}
\footnote{#1}
\let\thefootnote=\oldthefootnote
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% @Giray: You can find some more details on this \agy{3}{chapter} in the following link:
% https://docs.google.com/spreadsheets/d/130BQ4xrhCNGDC4TF3zOgH4KCYPuc5VYzPblkqi38NHc/edit?usp=sharing
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table}[htb]
\centering
\footnotesize
\renewcommand{\arraystretch}{0.895}
\setlength\tabcolsep{5pt}
% \vspace{-1.5em}
% \resizebox{\linewidth}{!}{
\begin{tabular}{l|l||c|c|c|c}
% \hline
% & & \multicolumn{2}{c|}{\textbf{Effective}}   &  \multicolumn{6}{c|}{\textbf{Easy to Adopt}}  \\
% \hline
% & & &  &           & \multicolumn{2}{c|}{\textbf{Low cost}}    & \multicolumn{2}{c|}{\textbf{Scalable}} \\
 \multicolumn{2}{c||}{} 
    & \multirow{8}{*}{\thead{Comprehensive Protection}}
    & \multirow{8}{*}{\thead{Compatible w/ Commodity\\DRAM Chips}} 
    & \multirow{8}{*}{\thead{Scaling with RowHammer Vulnerability}}
    & \multirow{8}{*}{\thead{Deterministic Protection}} \\
\multicolumn{2}{c||}{} & & & & \\
\multicolumn{2}{c||}{} & & & & \\
\multicolumn{2}{c||}{} & & & & \\
\multicolumn{2}{c||}{} & & & & \\
\multicolumn{2}{c||}{} & & & & \\
 & & & & & \\
\head{Approach} & \textbf{Mechanism} &  & &  &   \\ \hhline{=|=|=|=|=|=}%\hline\hline 
% &\thead{Scaling with DRAM Capacity} \\ \hline
%  Mechanism Name                             Compr.   Scaling    Compat.  Determ  LowPerf   LowEnrg   CapScal.
%                                             Threat   with       with
%                                             Model    RH-vulner  Comm.
\multicolumn{2}{l||}{Increased Refresh Rate~\cite{kim2014flipping, apple2015about}} & \cmark  & \cmark  & \xmark & \cmark  \\ \hline
\multirow{3}*{\setlength\tabcolsep{0pt}\begin{tabular}{l}Physical\\Isolation\end{tabular}} & CATT~\cite{brasser2017cant}      & \xmark & \xmark & {\xmark} & \cmark  \\ %\hline
 & GuardION~\cite{vanderveen2018guardion}    & \xmark & \xmark & {\xmark} & \cmark \\
  & ZebRAM~\cite{konoth2018zebram}   & \xmark & \xmark & {\xmark} & \cmark \\ %\hline
          \hline
          & ANVIL~\cite{aweke2016anvil}     & \xmark & \xmark & \agy{\cmark} & \cmark  \\ %\hline
          & \para{}~\cite{kim2014flipping}  & \cmark & \xmark & \agy{\cmark} & \xmark  \\ %\hline
\multirow{3}*{\setlength\tabcolsep{0pt}\begin{tabular}{l}Reactive\\Refresh\end{tabular}}  & \prohit{}~\cite{son2017making}  & \cmark & \xmark & \xmark & \xmark  \\ %\hline
   & \mrloc{}~\cite{you2019mrloc}    & \cmark & \xmark & \xmark & \xmark \\ %\hline
          % Armor\cite{ghasempour2015armor} & \cmark & \xmark &         &         & \xmark &&         \\ %\hline
          & \cbt{}~\cite{seyedzadeh2018mitigating} & \cmark & \xmark & \agy{\cmark} & \cmark   \\ %\hline
          & \twice{}~\cite{lee2019twice}    & \cmark & \xmark & \agy{\cmark} & \cmark  \\ %\hline
          \ifgraphene
          & \graphene{}~\cite{park2020graphene} & \cmark & \xmark & \agy{\cmark\cmark} & \cmark  \\ \fi
          \hline
\multirow{3}*{\setlength\tabcolsep{0pt}\begin{tabular}{l}Proactive\\Throttling\end{tabular}} & Naive Thrott.~\cite{mutlu2018rowhammer} & \cmark & \cmark & \xmark & \cmark  \\ %\hline
& Thrott. Supp.~\cite{greenfield2016throttling}& \cmark & \xmark & \xmark & \cmark  \\ \cline{2-6}
          & \textbf{\blockhammer{}}                                     & \cmark & \cmark & \agy{\cmark\cmark} & \cmark  \\ \hline
\end{tabular}
% {\footnotesize~`*' indicates {an optimistic} estimate for unreported characteristics.\vspace{-0.5\baselineskip}}
{\footnotesize~`\cmark\cmark' \agy{indicates that the mechanism scales with significantly lower performance, energy, and area overheads than others}.\vspace{-0.3\baselineskip}}
% }
% \vspace{5pt}
\caption{{Comparison of \rowhammer{} mitigation {mechanisms}.}}
% \caption{{Categorization and} characteristics of major \rowhammer{} mitigation mechanisms. `*' indicates {an optimistic} estimate for unreported characteristics. 
% % \agytdinline{Double-line splits the table. Fix.}
% % , while `-' \agy{means} that not enough information \omone{is publicly} available for an accurate estimate.
% }
\label{blockhammer:tab:current_mechanisms}
% \vspace{-1em}
\end{table}


%%%%%%%%%%%%%%%%
% ANVIL:
%%%%%%%%%%%%%%%%
% Energy: Anvil does not report any energy numbers. I think it should be low as they report very low false-positive rates.
% Threat model is comprehensive because it detects an attack based on the LLC misses

%%%%%%%%%%%%%%%%
% ZebRAM:
%%%%%%%%%%%%%%%%
% ZebRAM reports its performance overhead in the order of 5% for benign SPEC2006 benchmarks, 5.5% for a multicore nginx server and 2% for apache server. These are good results in general but other mechanisms induce much less overhead, especially the long-term solutions.
% Threat model is not that strong because it trusts hypervisor.

%%%%%%%%%%%%%%%%
% GuardION:
%%%%%%%%%%%%%%%%
% Performance results look good in the paper due to their weird baseline selection. However, I do not think that it is a low-cost mechanism.
%   They do not show overheads on top of a system that does not have any prevention, but they compare against Google's second patch.
% Threat model is not strong because it limits the attacks to uncached memory. It is a specialized defense for the attacks coming from DMA anyway.

%%%%%%%%%%%%%%%%
% CATT:
%%%%%%%%%%%%%%%%
% I refuse to report that CATT has low performance overhead because
%  (1) the paper itself admits that some measurements are faulty,
%  and (2) as GuardION describes, performance overhead of CATT is likely to increase in realistic scenarios where a user app attacks to another user app.
% I expect CATT to scale very bad with MAC because when rowhammer's effect on further rows increase, this method needs to allocate more gap in between user spaces. This will cost more DRAM capacity overhead.
% Threat model is not strong because it (1) does not prevent bitflips, just the ways to exploit them,
%   and (2) it assumes OS kernel is not vulnerable, (3) attacker is a low-privileged user who has limited
%   access to protected kernel space.


==> mainmatter/07_blockhammer/10_relatedwork.tex <==
\section{Related Work}
\label{blockhammer:sec:relatedwork}

% \textbf{State of \rowhammer{}.}
% The \rowhammer{} phenomenon is a direct result of process technology scaling, which exacerbates circuit-level interference.
% DRAM manufacturers continue reducing their minimum feature sizes and mitigate resulting circuit-level interference with in-DRAM \rowhammer{} mitigation mechanisms~\cite{jedec2015low, jedec2017}, instead of fixing the underlying sources of \rowhammer{}.
% Despite these mitigations, a recent work~\cite{frigo2020trrespass} shows that an attacker can still reliably induce \rowhammer{} bitflips on modern commodity DDR4 DRAM chips from three major vendors that implement in-DRAM \rowhammer{} mitigation mechanisms.
% On top of unreliable \rowhammer{} mitigation mechanisms, {Kim et al. reports that the required hammer count to induce a bitflip decreased more than an order of magnitude in the past decade (139k @2014, 4.8k @2019)~\cite{kim2020revisiting}. Therefore, \rowhammer{} is a more serious problem than ever and it is likely to worsen with future DRAM chips}~\cite{mutlu2017therowhammer, mutlu2019rowhammer_and, kim2020revisiting}.
% This has severe implications for system security and reliability, as many prior works demonstrate various ways of exploiting \rowhammer{} to compromise a system~\cite{seaborn2015exploiting, qiao2016nontemporal, vanderveen2016drammer_deterministic, gruss2016rowhammerjs_a, razavi2016flip, xiao2016onebit, tatar2018defeating, gruss2018another, lipp2018nethammer, cojocar2019exploiting,  ji2019pinpoint,kwong2020rambleed, frigo2020trrespass, kim2020revisiting}. {Therefore, it is important to protect all DRAM-based systems against \rowhammer{} while DRAM chips become more and more vulnerable to \rowhammer{}.}
To our knowledge, \blockhammer{} is the first work that (1)~prevents \rowhammer{} bitflips efficiently and scalably without {requiring} any proprietary knowledge of or {modification} to DRAM internals, (2)~satisfies all four of the desired characteristics for a \rowhammer{} mitigation mechanism (as we describe in Section~\ref{blockhammer:sec:qualitative_analysis}), and (3)~improves benign application performance and system energy when the system is under a \rowhammer{} attack.
% \mpj{To our knowledge,} \blockhammer{} is the first \rowhammer{} mitigation mechanism that is \agy{\emph{low-cost}, \emph{effective}} and \emph{easy-to-adopt} for comprehensively protecting all current and future DRAM-based systems against all \rowhammer{} attacks.
{Sections~\ref{blockhammer:sec:blockhammer_areaoverhead}, \ref{blockhammer:sec:evaluation}, and \ref{blockhammer:sec:qualitative_analysis} already qualitatively and quantitatively {compare} \blockhammer{} {to} the most relevant {prior} mechanisms, {demonstrating \blockhammer{}'s benefits}.
% require no changes to the DRAM chip. 
This section discusses \rowhammer{} mitigation and memory access throttling works that are loosely related to \blockhammer{}.}
% \rowhammer{} mitigation techniques that require modifications to the DRAM chip circuitry} \agy{and other applications of throttling.} 
% {We discuss mechanisms based on three major \rowhammer{} mitigation approaches (increased refresh rate, physical isolation, and reactive mitigation)}
% {We closely study three branches of \rowhammer{} mitigation approaches (i.e., increased refresh rate, physical isolation, and reactive mitigation) as well as key mechanisms implementing them
% {in Section~\ref{blockhammer:sec:qualitative_analysis}.} In this section, we explain in-DRAM \rowhammer{} mitigation methods.

\nind
\head{In-DRAM Reactive Refresh.} A subset of DRAM standards~\dramStandardCitations{} {jedec2015low, jedec2017} support a mode called \emph{target row refresh} (TRR), which refreshes rows that are physically nearby an aggressor row without exposing any information about {the in-DRAM} row address mapping outside of DRAM chips. TRRespass~\cite{frigo2020trrespass} demonstrates that existing proprietary implementations of TRR are not sufficient to mitigate \rowhammer{} bitflips\mpm{:} many-sided \rowhammer{} attacks reliably induce and exploit bitflips in state-of-the-art DRAM chips that already implement {TRR}.
% As an exception, HBM~\cite{jedec2021jesd235d} enhances the DRAM interface to allow the memory controller to specify an aggressor row to issue victim row refreshes. While this is a useful feature, a \rowhammer{} mitigation mechanism should \emph{not} rely on this feature{, as majority of DRAM standards do not provide it.}
% Furthermore, recent studies {show} that emerging memory technologies are susceptible to \rowhammer{}, while they are not guaranteed to have TRR~\cite{khan2018analysis, mutlu2017therowhammer}.

\nind
\head{Making Better DRAM Chips.} A different approach to mitigating \rowhammer{} is to implement
% A separate branch of \rowhammer{} mitigation research 
architecture- and device-level techniques that make DRAM chips stronger against \rowhammer{}. CROW~\cite{hassan2019crow} maps potential victim rows into dedicated \emph{copy rows} and mitigates \rowhammer{} bitflips by serving requests from copy rows. Gomez et al.~\cite{gomez2016dram_rowhammer} place \emph{dummy cells} in DRAM rows that are engineered to be more susceptible to \rowhammer{} than regular cells, and monitor dummy cell charge levels to detect a \rowhammer{} attack. 
% To mitigate \rowhammer{} vulnerability, 
{Three other works~\cite{yang2016suppression, ryu2017overcoming, han2021surround} propose manufacturing process enhancements {or {implantation of} additional dopants in transistors to reduce} wordline {crosstalk}.}
% Ryu et al.~\cite{ryu2017overcoming} propose an annealing process that reduces the traps in a DRAM array, thereby reducing wordline cross-talk. Yang et al.~\cite{yang2016suppression} {implant} phosphorus between wordlines for better isolation {between rows}. 
{Although} these methods mitigate the \rowhammer{} vulnerability of DRAM chips, they {(1)} cannot be applied to already-deployed commodity DRAM chips {and {(2)} can be high cost} {due to {the} required {extensive} chip modifications.}
% as they require modifications in chip design.

% \agyc{This paragraph was at the end of Section 3. I moved it into the Related Work because it was breaking the flow. Does that sound good?} \mpc{agreed. it fits here}

\nind
{\textbf{Other Uses of Throttling.} 
% Throttling is a common approach across 
Prior works on quality-of-service- and fairness-oriented architectures propose selectively throttling main memory accesses to provide latency guarantees and/or improve fairness across applications}
% without concern for system security }}
(e.g., \cite{rixner2000memory, rixner2004memory, moscibroda2007memory, mutlu2007stalltime,  mutlu2008parallelismaware, lee2008prefetchaware, kim2010atlas, kim2010thread,  subramanian2014theblacklisting, subramanian2016bliss, ausavarungnirun2012staged, ebrahimi2011parallel, ebrahimi2010fairness, ebrahimi2011prefetchaware, nychis2012onchip, nychis2010next, chang2012hatheterogeneous, usui2016dash}).
% \agy{These works apply throttling\agycomment{Do all of them do that?} to} provide latency guarantees and/or fairness across applications without concern for system security. 
These mechanisms are \emph{not} designed to prevent \rowhammer{} attacks and thus do not interfere with a \rowhammer{} attack when there is no contention between memory accesses. 
% memory bandwidth is underutilized.} 
In contrast, BlockHammer's primary goal is to 
{prevent \rowhammer{} attacks from inducing bitflips.} As such, \blockhammer{} is {complementary} to these mechanisms, and can work together with them. 
% \todo{om: This RHLI comment is NOT GOOD. BlockHammer can simply work with any other memory scheduling mechanism. Period. Why make your point weaker by focusing on a completely optional part of BlockHammer. I am getting very concerned that the thinking employed in writing the paper is not straight and careful. We need to converge, not diverge.}
% prevent RowHammer attacks, \agy{while it can reduce the performance degradation that a \rowhammer{} attack inflicts upon benign applications.}
% not to provide QoS or fairness. 
% \agy{For instance, \blockhammer{} does not interfere with a thread's memory accesses as long as the thread does not hammer a DRAM row even if the thread creates QoS or fairness problems in the system.}
% These two techniques are distinct, as we demonstrate from two aspects.
% First, a conventional QoS mechanism is not designed to prevent RowHammer attacks. For example, consider the case where a single thread is running and is performing a RowHammer attack. Since there are no concurrently-executing processes, the QoS mechanism would not affect the running process, whereas HammerThrottler would throttle it to prevent it from flipping bits. Preventing malicious attacks is the key advantage of our technique over conventional QoS mechanisms.
% Second, HammerThrottler is not a QoS mechanism. Consider the case where there are multiple threads running, but none of them hammer any row enough times to trigger HammerThrottler. In this case, the threads execute as they would in the baseline, without any changes to the system QoS.






% {In this section, we qualitatively compare \blockhammer{} and key \rowhammer{} mitigation mechanisms that we classify under three high-level approaches:}
% % The large body of prior works on mitigating \rowhammer{} suggests three high-level approaches:
% (1) increasing the refresh rate~\cite{kim2014flipping, apple2015about}, (2) physically isolating the sensitive data~\cite{konoth2018zebram, vanderveen2018guardion, brasser2016cant}, and (3) reactive refresh~\cite{kim2014flipping, son2017making, seyedzadeh2018mitigating, you2019mrloc, lee2019twice}. To evaluate key mechanisms of these three approaches, we study them in terms of five fundamental features that we find necessary for a \rowhammer{} mitigation mechanism to be \emph{effective} and \emph{easy-to-adopt} across all DRAM-based systems. We provide a summary of this evaluation in Table~\ref{blockhammer:tab:current_mechanisms}, and evaluate related work under each feature below.

% % \input{06_relatedwork_table_alternative}

% % \subsection{five features for effectively mitigating \rowhammer{}}
% \\nind
% \textbf{1. Comprehensive protection.} A \rowhammer{} mitigation mechanism should prevent \rowhammer{} bitflips regardless of the methods that an attacker may use to issue a hammering access pattern. Unfortunately several recently proposed \rowhammer{} mitigation mechanisms are only effective against a limited threat model, and published works have already demonstrated methods for bypassing these mechanisms. We describe four of these instances, three of which physically isolate sensitive data and one performs reactive refresh.
% ZebRAM~\cite{konoth2018zebram}, GuardION~\cite{vanderveen2018guardion}, and CATT~\cite{brasser2016cant} physically isolate DRAM rows that an attacker can access and DRAM rows that contain sensitive data. Each of these mechanisms defines a limited threat model. For instance, ZebRAM's threat model trusts the hypervisor which is later exploited by Telehammer~\cite{zhang2019telehammer} to defeat ZebRAM. Similarly, GuardION~\cite{vanderveen2018guardion}'s threat model only considers the DMA-based accesses, while many prior works mount \rowhammer{} attacks without using DMA accesses~\cite{gruss2016rowhammerjs_a, gruss2018another, cojocar2019exploiting, zhang2019telehammer, kwong2020rambleed}. As another example, CATT~\cite{brasser2016cant} physically separates user and kernel memory spaces in DRAM, which \mpf{theoretically limits} bitflips \mpf{to within an} attacker's own user space. However, Gruss et al.~\cite{gruss2018another} reliably perform a \rowhammer{} attack by flipping certain opcode bits in user space that provides an unprivileged process with root privilege.
% As a reactive-refresh-based approach, Anvil~\cite{aweke2016anvil} also provides limited security guarantees by relying on certain hardware performance counters that measures the LLC misses to detect a \rowhammer{} attack. However, several works~\cite{vanderveen2016drammer_deterministic, gruss2018another, tatar2018throwhammer} defeat Anvil by bypassing caches without causing LLC misses.

% \\nind
% \textbf{2. Compatibility with commodity DRAM chips.} Given that prior works~\cite{cojocar2020arewe, frigo2020trrespass, kim2020revisiting} experimentally observe \rowhammer{} bitflips on off-the-shelf modern DRAM devices that are promoted as \rowhammer{}-safe, it is essential for a \rowhammer{} mitigation mechanism to be compatible with all commodity DRAM chips. To achieve this, a \rowhammer{} mitigation mechanism should \emph{not} rely on (1) any proprietary information that DRAM vendors do not share, and (2) it should not expect any modifications to DRAM chip design.
% Unfortunately, physically isolating sensitive data and reactive refresh approaches need to be fully aware of the internal physical organization of DRAM rows, which is proprietary information because it can contain insights into the density-optimized chip design and the chip's reliability. Isolation-based mechanisms require this information to ensure that isolated memory regions are not physically close to each other. Reactive refresh mechanisms need this information to identify victim rows that they need to refresh.
% % The vast majority of the previously proposed mechanisms (e.g., \para{}~\cite{kim2014flipping}, Anvil~\cite{aweke2016anvil}, \prohit{}~\cite{son2017making}, \cbt{}~\cite{seyedzadeh2018mitigating}, \twice{}~\cite{lee2019twice}, and \mrloc{}~\cite{you2019mrloc}) mitigate \rowhammer{} by refreshing victim DRAM rows. Another set of these mechanisms (e.g., CATT~\cite{brasser2016cant}, ZebRAM~\cite{konoth2018zebram}, and GuardION~\cite{vanderveen2018guardion}) isolate DRAM rows that contain sensitive data to keep them far from any potential aggressor row. Both of these methods require being fully aware of the \mpf{internal physical organization} of DRAM rows to determine rows that are physically nearby an aggressor row.
% % Unfortunately, this is proprietary information that DRAM manufacturers do not publicly share because it can contain insights into the vendor's density optimized chip design and the chip's reliability as we describe in Section~\ref{blockhammer:sec:background_physicallayout}.
% % Given that DRAM manufacturers do not share this information, one of two additional steps must be taken to make these mechanisms compatible with commodity DRAM chips. First, a system can extensively reverse-engineer the physical layout of DRAM rows for all banks in all chips, which can take significantly long period of time
% % % \agyrm{increase down-time of a system during maintenance}
% % and requires additional area overhead to store the reverse-engineered layout, as the physical layout of DRAM rows can be any permutation of tens of thousands of DRAM rows per bank per chip.\footnote{Reverse-engineering is not an important concern for an attacker, as (1) an attack requires finding only a few DRAM rows which are nearby a known victim DRAM row instead of reconstructing the whole layout of each bank, each chip and (2) an attacker does not necessarily care about the overhead of reverse-engineering on system performance, availability, and quality of service.}  Second, the DRAM interface should provide additional support in performing operations that require proprietary information on DRAM chip (e.g., refreshing a DRAM row that is adjacent to a provided aggressor row address), which is not supported by the vast majority of DRAM standards~\cite{jedec2015low, jedec2017}.
% The only \rowhammer{} mitigation mechanism that is compatible with all commodity DRAM chips is to refresh \emph{all} rows at a higher frequency~\cite{kim2014flipping, apple2015about}. Unfortunately, this method is not practical due to its large performance overheads (e.g., up to 35\% performance overhead for DDR3 DRAM chips~\cite{kim2014flipping}) and its highly limited scalability preventing it to support modern DRAM chips~\cite{kim2020revisiting}.

% A subset of DRAM standards~\cite{jedec2015low, jedec2017} support a mode called \emph{target row refresh} (TRR), which refreshes rows that are physically adjacent to an aggressor row without exposing physical row placement.
% Unfortunately, TRRespass~\cite{frigo2020trrespass} demonstrates that TRR is not sufficient to mitigate \rowhammer{} bitflips, and it is practical to perform reliable \rowhammer{} attacks on these chips.
% % As an exception, HBM~\cite{jedec2021jesd235d} enhances the DRAM interface to allow the memory controller to specify an aggressor row to issue victim row refreshes. While this is a useful feature, a \rowhammer{} mitigation mechanism should \emph{not} rely on this feature{, as majority of DRAM standards do not provide it.}
% Furthermore, emerging memory technologies are expected to be susceptible to \rowhammer{}. For example, Khan et al.~\cite{khan2018analysis} show that a \rowhammer{} attack may cause read disturbance errors on an STTRAM device.
% Such technologies are not guaranteed to have TRR support~\cite{mutlu2017therowhammer}.

% A separate branch of \rowhammer{} mitigation research suggests architecture- and device-level techniques to make DRAM chips stronger against \rowhammer{}. For example, CROW~\cite{hassan2019crow} replicates a number of rapidly-activated rows into dedicated copy rows and mitigates \rowhammer{} bitflips by serving some requests from these copy rows. Gomez et al.~\cite{gomez2016dram_rowhammer} place dummy cells in DRAM rows that are engineered to be more susceptible to \rowhammer{} than regular cells, and monitor their charge levels to detect a \rowhammer{} attack. To mitigate \rowhammer{} vulnerability, Ryu et al.~\cite{ryu2017overcoming} propose an H2 annealing process that reduces the traps in a DRAM array. Similarly, Yang et al.~\cite{yang2016suppression} propose implanting additional phosphorus between the word lines for better cell isolation. Given that these methods can mitigate the \rowhammer{} vulnerability of DRAM chips, they cannot be applied to commodity DRAM chips as they require modifications in-chip design.

% \\nind
% \textbf{3. Scalability with increasing \rowhammer{} vulnerability.}
% An effective \rowhammer{} mitigation mechanism should be able to scale well while DRAM chips' \rowhammer{} vulnerability increases. Kim et al.~\cite{kim2020revisiting} demonstrate that (1) increasing refresh rate~\cite{kim2014flipping, apple2015about} is not a scalable approach even for off-the-shelf modern DRAM chips, (2) only \para{}~\cite{kim2014flipping} can sustain its security guarantees for projected future devices among reactive-refresh mechanisms~\cite{son2017making, you2019mrloc, lee2019twice}, and its performance overhead can reach up to 80\% to sustain its security. As recent works~\cite{frigo2020trrespass, kim2020revisiting} show that hammering a DRAM row can disturb more number of rows than before, mitigating \rowhammer{} by physically isolating memory regions also requires allocating more rows to build thicker barriers between memory regions, increasing their capacity overhead. Unfortunately, no prior work provides a sufficient characterization to precisely observe this trend, and the key instances of this approach~\cite{konoth2018zebram, vanderveen2018guardion, brasser2016cant} are already defeated by newer attacks as we discuss above. Therefore, we do not quantify the scalability of physically isolating the sensitive data in the scope of this work.

% \\nind
% \textbf{4. Deterministic prevention.} It is important to minimize any chance of experiencing \rowhammer{} bitflips across all DRAM-based systems, because a successful \rowhammer{} attack can be used for compromising the whole system by escalating privilege levels or obtaining private data. Several prior works claim that minimizing the probability of a \rowhammer{} bitflip is secure-enough for many systems. However, as Aven et al. argues~\cite{aven2009identification} success probability of an attack (e.g., a \rowhammer{} attack) should be considered differently than the success probability of a reliability failure (e.g., soft errors due to particle strikes), and it is essential to guarantee zero chance of a \rowhammer{} bitflip for a critical system whose failure or malfunction may result in severe consequences (e.g., related to loss of lives, environmental damage, or economic loss). Unfortunately, PARA~\cite{kim2014flipping}, ProHIT~\cite{son2017making}, and MRLoc~\cite{you2019mrloc} cannot reduce a \rowhammer{} attack's success probability to absolute zero even though they address a comprehensive threat model.

% \\nind
% \textbf{5. Low Performance and Energy Overhead.}
% As data movement throughout the memory hierarchy becomes an increasingly significant limiting factor of overall system performance and
% energy efficiency~\cite{wulf1995hitting, wilkes2001thememory, mckee2004reflections,
% ferdman2012clearing, mutlu2013memory, mutlu2014research, kanev2016profiling,
% wang2014bigdatabench, boroumand2018google, aichinger2015ddr}, a \rowhammer{} mitigation mechanism should not further contribute to this bottleneck in both when the system is under attack and not under attack.

% % \\nind
% % \textbf{6. Scalability with DRAM Capacity.}
% % As DRAM technology shrinks, each DRAM chip's storage capacity increases. This can result in increasing the number of rows and/or the capacity of each DRAM row. To support future DRAM chips, a \rowhammer{} attack needs to scale well with increasing DRAM capacity. While increasing a DRAM row's capacity does not largely affect a \rowhammer{} mitigation mechansim's scalability, increasing the number of rows per bank requires deterministic reactive refresh mechanisms~\cite{seyedzadeh2018mitigating, lee2019twice} to implement larger number of counters. Similarly, increasing the per-bank row count hurts increasing refresh rate method's scalability as it requires performing more refresh operations per unit time.
% %Note that DRAM vendors determine a DRAM row size by considering the power budget for row activation and active-standby consumption of DRAM rows as well as their chip geometry. We observe that a DRAM row size does not increse linearly  Unfortunately, the chip area overhead of state-of-the-art mitigation mechanisms it needs to
% % Furthermore, the mechanism should not consume a large amount of chip area that could otherwise be utilized for other architecture-level improvements (e.g., larger register files, caches, TLBs, or additional accelerators).
% % \mpf{Unfortunately, although increasing the refresh rate across all rows is the previously-proposed \rowhammer{}-mitigation mechanism that provides the highest compatibility with commodity DRAM chips, it is also the most expensive mechanism in terms of performance cost.}


==> mainmatter/07_blockhammer/12_camready_notes.tex <==
\section{Notes on Camera Ready Improvements}
I summarize here the improvements we are planning for the final version of the paper along with improving descriptions. I use todo notes package to mark relevant parts of the texts for each of these improvements. All tags are in the following format: CRX XII-X, meaning Camera Ready improvement number X and the internal description of the improvement is available under Section XII-X. Section number is there to make markers clickable.

\subsection{CR1: Including a Concrete Mechanism Definition for HammerThrottler}
\label{sec:CR1}
In the accepted and shepherded version it is not clear how HammerThrottler can be implemented in a system and what modifications need to be done to handle stalled memory requests without overflowing the buffers. I added a paragraph marked as CR1~\ref{blockhammer:sec:CR1} in page 6.

\subsection{CR2: Evaluating BlockHammer for Many-Sided Attacks}
\label{sec:CR2}
We already have this evaluation but it is not clear in the paper. The way BlockHammer addresses many-sided attacks is through scaling down the RowHammer threshold appropriately. In the current evaluation we have two parts regarding this evaluation:
First, we compare BlockHammer against other mechanisms for double-sided attacks since all prior mechanisms are designed for double-sided attacks.
Second, we evaluate BlockHammer for reduced RowHammer thresholds ($HC_{first}$ in Jeremie’s terminology) (see Figure 7). Therefore, we already share the results for many-sided attacks in Figure 7. However, it is unreasonable for a reader to find the appropriate threshold for many-sided attacks in the current shape. I have put a placeholder text in page 11 to  evaluation, marked with CR2~\ref{blockhammer:sec:CR2}.

\subsection{CR3: Graphene}
\label{sec:CR3}
Graphene is the new state-of-the-art among all reactive-refresh-based mechanisms. We are implementing Graphene in our Ramulator. We will add Graphene's depending on its performance and area overheads. For now I added Graphene into Methodology (marked with CR3~\ref{blockhammer:sec:CR3})

\subsection{CR4: Show that BLISS cannot protect against RowHammer attacks.}
\label{sec:CR4}
BLISS’ blacklisting mechanism deprioritizes memory accesses instead of delaying them until a certain time is passed. Therefore, even a naive RowHammer attack can be successful on a system that uses BLISS. One option is to discuss this in the text (maybe with a figure’s help). Another option is to share experimental data, which can be an overkill. For now, I will include a short discussion for BLISS in Related Work and marked with CR4~\ref{blockhammer:sec:CR4}.

\subsection{CR5: Revisiting Key Limitations of the Mechanism}
\label{sec:CR5}
\head{Area cost for real systems.} One BH instance per bank can be unreasonably costly for a real server system. However, we can share Bloom filters across banks to reduce the area overhead. This can be addressed by CR5~\ref{blockhammer:sec:CR5} as well.

\head{Claim on Compatibility with Commodity DRAM Chips.} BlockHammer is not completely compatible with commodity DRAM chips because it still needs at least three characteristics:
\begin{itemize}
  \item \nrh{}: RowHammer threshold
  \item $d_{max} (blast~radius):$ the maximum distance at which an aggressor row can disturb a victim row
  \item $c_i:$ the impact factor for an aggressor row at $i$-row distance.
\end{itemize}
Our best argument so far is that even if a DRAM vendor does not report these values, one can perform known characterization methods or apply publicly available characterization results with a guardband. Quickly finding these parameters for any given chip is an ongoing research problem, and all other mechanisms still require this anyway. We addded an argument in this direction during the rebuttal period that I marked with CR6~\ref{blockhammer:sec:CR5}.

\subsection{CR6: Area and Performance Tradeoff}
\label{sec:CR6}
No reviewer pointed out this, but I think it will be better to include this analysis in the camera-ready. To sustain the low performance overhead, we need to increase the number of counters in counting Bloom filters while scaling the RowHammer threshold to extreme levels. A plot or table can be sufficient to demonstrate this trade-off. We did not include before due to space constraints. I've put a placeholder with label CR6~\ref{blockhammer:sec:CR6}.

\subsection{CR7: References Fix}
\label{sec:CR7}
References started using et al. after changing the style file. We should avoid et al. Fix them. 

==> mainmatter/07_blockhammer/12_workload_characteristics.tex <==
% \section{\agy{Benign Application Characteristics}}
% \label{blockhammer:sec:benign_application_chars}
\vspace{1em}
{Table~\ref{blockhammer:tab:workload_list} {lists the} 30 benign applications we use for cycle-level simulations. We report last-level cache misses ($MPKI$) and row buffer conflicts ($RBCPKI$) per kilo instructions for each application. Non-temporal data copy, YCSB Disk I/O, and network accelerator applications do not have an $MPKI$ value because they directly access main memory.} 
\vspace{0.8em}
\begin{table}[h!]
    \footnotesize 
    \centering
    \caption{Benign applications used in cycle-level simulations.}
    \label{blockhammer:tab:workload_list}
    \begin{tabular}{l|l|l||rr}
    % \hline
\head{Category}                & \textbf{Benchmark Suite}            & \textbf{Application}    &   \textbf{MPKI} & \textbf{RBCPKI} \\ \hline \hline
\multirow{12}{*}{L}   & \multirow{10}{*}{SPEC2006} & 444.namd       &    0.1 &   0.0  \\
                        &                            & 481.wrf        &    0.1 &   0.0  \\
                        &                            & 435.gromacs    &    0.2 &   0.0  \\
                        &                            & 456.hmmer      &    0.1 &   0.0  \\
                        &                            & 464.h264ref    &    0.1 &   0.0  \\
                        &                            & 447.dealII     &    0.1 &   0.0  \\
                        &                            & 403.gcc        &    0.2 &   0.1  \\
                        &                            & 401.bzip2      &    0.3 &   0.1  \\
                        &                            & 445.gobmk      &    0.4 &   0.1  \\
                        &                            & 458.sjeng      &    0.3 &   0.2  \\ \cline{2-2}
                        & Non-Temp. Data Copy        & movnti.rowmaj  &    -   &   0.2  \\ \cline{2-2}
                        & \multirow{4}{*}{YCSB Disk I/O}      & ycsb.A         &    -   &   0.4  \\ \cline{1-1}\cline{3-5}
\multirow{9}{*}{M} &                            & ycsb.F         &    -   &   1.0  \\
                        &                            & ycsb.C         &    -   &   1.0  \\
                        &                            & ycsb.B         &    -   &   1.1  \\ \cline{2-2}
                        & \multirow{12}{*}{SPEC2006} & 471.omnetpp    &    1.3 &   1.2  \\
                        &                            & 483.xalancbmk  &    8.5 &   2.4  \\
                        &                            & 482.sphinx3    &    9.6 &   3.7  \\
                        &                            & 436.cactusADM  &   16.5 &   3.7  \\
                        &                            & 437.leslie3d   &    9.9 &   4.6  \\
                        &                            & 473.astar      &    5.6 &   4.8  \\ \cline{1-1}\cline{3-5}
\multirow{9}{*}{H}   &                            & 450.soplex     &   10.2 &   7.1  \\
                        &                            & 462.libquantum &   26.9 &   7.7  \\
                        &                            & 433.milc       &   13.6 &  10.9  \\
                        &                            & 459.GemsFDTD   &   20.6 &  15.3  \\
                        &                            & 470.lbm        &   36.5 &  24.7  \\
                        &                            & 429.mcf        &  201.7 &  62.3  \\ \cline{2-2}
                        & Non-Temp. Data Copy        & movnti.colmaj  &  -     &  30.9  \\ \cline{2-2}
                        & \multirow{2}{*}{Network accelerator}   & freescale1     &  -     & 336.8  \\
                        &                            & freescale2     &  -     & 370.4  \\ \hline 

    \end{tabular}
    
\end{table}

==> mainmatter/07_blockhammer/13_blockhammer_configurations.tex <==
\section{{Appendix Tables}}
\label{blockhammer:sec:appendix_tables}
\vspace{0.8em}
{Table \ref{blockhammer:tab:allconfigs} shows BlockHammer's configuration parameters used for each \rowhammer{} threshold (\nrh{}) in Sections~\ref{blockhammer:sec:blockhammer_areaoverhead} and~\ref{blockhammer:sec:evaluation_tech_scaling}.}

\begin{table}[h!]
    \footnotesize
    \centering
    \caption{\blockhammer{}'s configuration parameters used for different $\mathbf{\nrhn{}}$ values.}
    \label{blockhammer:tab:allconfigs}
    \begin{tabular}{r||rrrr}
        \emph{$\mathbf{\nrhn{}}$} & {\nrhtuned{}} & {CBF Size} & {\nbl{}} & {\tbf{}} \\ \hline\hline
        \textbf{32K} & 16K & 1K & 8K & \SI{64}{\milli\second} \\
        \textbf{16K} &  8K & 1K & 4K & \SI{64}{\milli\second} \\
        \textbf{ 8K} &  4K & 1K & 2K & \SI{64}{\milli\second} \\
        \textbf{ 4K} &  2K & 2K & 1K & \SI{64}{\milli\second} \\
        \textbf{ 2K} &  1K & 4K & 512& \SI{64}{\milli\second} \\
        \textbf{ 1K} & 512 & 8K & 256& \SI{64}{\milli\second} \\
         \hline
    \end{tabular}
    
\end{table}

==> mainmatter/08_hira/00_abstract_clean.tex <==
\begin{abstract}
{DRAM is the building block of modern main memory systems. DRAM cells must be periodically refreshed to prevent data loss. Refresh operations degrade system performance by interfering with memory accesses.}
{{As} DRAM chip density increases with technology node scaling, refresh operations {also increase because}:}
1)~{the number of DRAM rows in a chip increases}; and 2)~DRAM cells {need additional refresh operations to mitigate bit failures caused by RowHammer, a {failure} mechanism that {becomes worse with technology node scaling}.} 
{Thus,} it is critical to {enable} refresh {operations} at low performance overhead.
{To {this end},} we propose {a new operation,} \gls{hira}, {and
{\gls{hirasched} to perform \gls{hira} operations.}
} 

{\gls{hira} hides a refresh operation's latency by refreshing a row {concurrently} with accessing or refreshing another row within the same bank. Unlike prior works, \gls{hira} achieves this parallelism without any modifications to off-the-shelf DRAM chips. To do so, it leverages}
{the new observation that two rows in the same bank can be activated without data loss if the rows are connected to different charge restoration circuitry.}
We experimentally demonstrate on \chipcnt{}
real off-the-shelf DRAM chips that {\gls{hira} {can} reliably parallelize} a DRAM row's {refresh operation} {with refresh or {activation of} {any of the}} \covref{} of the rows {within the same bank. By doing so,}
\gls{hira} reduces {the overall latency of two} refresh {operations} by \SI{51.4}{\percent}. 
\gls{hirasched} modifies the memory request scheduler to perform \gls{hira} when a refresh operation can be {performed concurrently} with a \memacc{} or another refresh.
{Our system-level evaluations show that}
{HiRA-MC {increases system performance by \SI{12.6}{\percent} and $3.73\times$ {as it reduces}} the performance degradation {due to} periodic refreshes and refreshes for RowHammer {protection} (preventive refreshes){, respectively,} for future DRAM chips with increased density and RowHammer vulnerability.
}
\end{abstract}

==> mainmatter/08_hira/01_introduction_clean.tex <==
\section{Introduction}
\label{sec:introduction}
DRAM~{\cite{dennard1968fieldeffect}} is the prevalent {main memory} technology used in a wide variety of computing systems from cloud servers to mobile devices {due to its high density and low latency}.
{A DRAM cell encodes a bit of data as electrical charge, {which} inherently leaks over time~\cite{keeth2001dram_circuit}. Therefore,}
to ensure reliable operation and data integrity, a DRAM cell needs to be periodically refreshed~\cite{jedec2008jesd79f, jedec2020jesd794c, jedec2020jesd795, jedec2017jesd2094b, jedec2020jesd2095a, jedec2021jesd235d}. 
Unfortunately, these refresh operations degrade system performance by interfering with memory accesses~\cite{liu2012raidr, chang2014improving}. {{During a} refresh operation{, which} is performed at row granularity (e.g., 8KB), the memory cannot service any {requests to} the DRAM bank~(e.g.,~512MB) or rank~(e.g.,~8GB) that contains the refreshed row~\cite{micron2014sdram, jedec2020jesd794c, jedec2017jesd2094b}.}

{As DRAM density increases with technology node scaling, the performance overhead of refresh also increases due to three major reasons.}
{First, as the {DRAM} chip density increases, more DRAM {rows} need to be {periodically} refreshed in a DRAM chip~\cite{jedec2008jesd79f, jedec2020jesd794c, jedec2020jesd795, jedec2017jesd2094b, jedec2020jesd2095a, jedec2021jesd235d}.
{Second, as {DRAM} technology node scales down, DRAM cells become smaller and thus can store less amount of charge, requiring them to be refreshed more frequently~{\perrefreshscaling{}}.}
{Third}, with increasing {DRAM} density, DRAM cells are placed closer to each other, exacerbating charge leakage via a disturbance error mechanism called RowHammer~\rhdefinition{}, and thus requiring additional refresh operations {(called \emph{preventive} refreshes)} to avoid data {corruption} due to RowHammer~\rhdefrefresh{}.}
Prior work shows that 1)~{RowHammer} can be exploited to escalate privilege, leak private data, and manipulate critical application outputs~\rhattacks{}; and 2)~modern DRAM chips, including the ones that are marketed as RowHammer-safe~\rhsafe{}, are more vulnerable to RowHammer than their predecessors~\rhworse{}. {Therefore, {defending against} RowHammer is critical for secure system operation and {doing so likely} requires aggressively refreshing the cells disturbed by RowHammer~\rhdefworse{}.
As a result of {these three major reasons, newer generations of} DRAM chips require performing more refresh operations compared to their predecessors{. T}hus{,} it is critical to reduce the performance overhead of refresh{es}.}

Prior works suggest reducing refresh latency by 1)~accelerating the charge restoration process~\cite{luo2020clrdram, hassan2019crow} and 2)~exploiting parallelism across subarrays within a DRAM bank~\salprefs{}. Unfortunately, these proposals require modifications to DRAM circuitry, making them {un}suitable for already deployed off-the-shelf DRAM chips.
{Therefore,} it is {important} to find alternative solutions to reduce the negative performance impact of {a} refresh operation {with no modifications to the DRAM chip circuitry}. 

\head{Our goal} is to reduce the refresh latency in off-the-shelf DRAM chips with \emph{no} modifications to DRAM circuitry. 
To this end, we propose {a new operation called} \gls{hira} {and {\gls{hirasched}}} to perform \gls{hira} operations.

\gls{hira} enables refreshing a DRAM row while refreshing or accessing another DRAM row within the same bank.
\gls{hira} leverages the new observation that opening two rows, {whose charge restoration circuitries are electrically isolated from each other{,} {in rapid succession}, allows refreshing one row while refreshing or accessing the other row.} 
{To {open two such rows in rapid succession},} \gls{hira} {uses a carefully{-}engineered sequence of} \gls{act} and \gls{pre} commands, already implemented in off-the-shelf DRAM chips for opening and closing DRAM rows, respectively.
We experimentally demonstrate on \chipcnt{} real off-the-shelf DRAM chips that \gls{hira} 1)~{reliably parallelizes a DRAM row's {refresh operation} {with refresh or {activation} of any of the} \covref{} of the rows within the same bank}
{and 2)~}effectively reduces the {overall} latency of refreshing two rows
by \param{\SI{51.4}{\percent}}.

{\Glsfirst{hirasched} leverages {the} \gls{hira} {operation} {to improve}} system {performance by performing} \emph{two} main {tasks}. First, {it} queues {each} refresh request {with a time slack before the refresh needs to be performed and assigns the refresh request} a deadline.
Second, {it} observes the \memaccs{} {at} real-time to find a \memacc{} that can be {performed concurrently} with a {queued} refresh {request}.
\gls{hirasched} ensures that each periodic and preventive refresh request is performed by its deadline. \gls{hirasched} achieves this by taking one of three possible actions, in {the following} order: 1)~refresh {a DRAM row} {concurrently} with a \memacc{} {(refresh-access parallelization)} before the refresh operation's deadline; 2)~refresh {a row} {concurrently} with another refresh operation {(refresh-refresh parallelization)} if {refresh-access parallelization is \emph{not} possible} until the refresh operation's deadline; or 3)~perform a refresh operation {right} at its deadline if neither 
{refresh-access nor refresh-refresh parallelization is possible.}
We evaluate \gls{hirasched}'s hardware complexity and show that it consumes only \param{{\SI{0.00923}{\milli\meter\squared}}} chip area and {responds to queries within {{\SI{6.31}{\nano\second}}} (in parallel to a \gls{pre} command with a latency of \SI{14.5}{\nano\second})}{.}
To evaluate \gls{hirasched}'s performance benefits, we conduct cycle-level simulations on \wlcnt{} multiprogrammed workloads.
Our analysis shows that {1)~\emph{without} \gls{hira}, periodic and preventive refresh operations cause \SI{26.3}{\percent} and \SI{96.0}{\percent} performance overhead for future DRAM chips with high density and high RowHammer vulnerability, respectively}, compared to an ideal memory controller that does \emph{not} perform periodic or preventive refreshes {and 2)~\gls{hirasched} {increases system performance by \SI{12.6}{\percent} and $3.73\times$ {as it reduces}} the performance degradation {due to} periodic refreshes and preventive refreshes{, respectively,} for future DRAM chips with increased density and RowHammer vulnerability.}

This paper makes the following contributions: 
\glsresetall
\squishlist
\item This is the first {work to} show that refresh-refresh and refresh-access parallelization within a bank is possible {in} off-the-shelf DRAM chips by issuing a carefully{-}engineered sequence of \gls{act} and \gls{pre} {commands}, which we call \gls{hira}.  
\item We experimentally demonstrate on \chipcnt{} real {DDR4} DRAM chips that {\gls{hira}} 1)~reduces the latency of refreshing two rows back-to-back by \param{\SI{51.4}{\percent}}, 
and 2)~{reliably parallelizes a DRAM row's {refresh operation} {with refresh or {activation} of any of the} \covref{}}
of the rows
in the same bank.
\item We {design} {\gls{hirasched} to perform \gls{hira} operations}. We show that {\gls{hirasched} significantly {improves system performance by \SI{12.6}{\percent} and $3.73\times$ {as it reduces}} the performance degradation {due to} periodic refreshes and {preventive} refreshes for RowHammer}{,}
respectively. 
 
\squishend





==> mainmatter/08_hira/02_background_clean.tex <==
\section{Background}
\label{sec:background}

This section describes the background required to understand the rest of the paper. For a more comprehensive description of DRAM organization and operation, we refer the reader to~\cite{kim2012acase,liu2012raidr,lee2013tieredlatency,keeth2001dram_circuit, lee2015decoupled}.
\subsection{DRAM Organization}
DRAM is organized hierarchically. The {memory controller} accesses DRAM modules {via a} memory channel.
{A} DRAM module {has} one or more ranks{, each of which contains multiple DRAM chips} that work in lock-step. 
{{Each DRAM chip consists of} multiple DRAM banks{, {which} share the I/O circuitry {of the chip (called \emph{{chip I/O}})}}.}

\head{Bank Organization} \figref{fig:DRAM_organization} shows a typical DRAM chip organization, {containing multiple banks.}
A DRAM bank is composed of multiple subarrays{, {which} share the I/O circuitry of the bank {(called \emph{{bank I/O}})}}. Each subarray contains a two{-}dimensional array of DRAM cells, organized as rows and columns {and a local row buffer}. A DRAM cell stores data as {electrical} charge in a capacitor, which is {accessed} via an access transistor.
{The gate of an access transistor is driven by a row-wide {wire}, called wordline. {T}he access transistor connects the cell capacitor to a column-wide structure, called bitline. {A} bitline is connected to a \emph{sense amplifier (SA)} and \emph{precharge} circuitry.}

\head{Open-bitline Architecture} To optimize the size and layout of subarrays, the common open-bitline architecture~\cite{chang2016low,keeth2007dram_circuit, luo2020clrdram} places the SAs {on} both {ends} (i.e., top and bottom) of the subarray (as depicted in \figref{fig:DRAM_organization}). In this architecture, {horizontally} adjacent DRAM cells are connected {via} bitlines to SAs {on both ends} of the subarray.

\begin{figure}[h]
    \centering
    \includegraphics[width=\linewidth]{figures/cr_DRAM_organization4-crop.pdf}
    \caption{DRAM organization}
    \label{fig:DRAM_organization}
\end{figure}

\subsection{DRAM Operation}
The memory controller {implements a memory request scheduler to issue} DDRx commands. We describe the four DDRx commands that are relevant to this work.


{\head{Precharge}} {A bitline needs to be precharged to half of {the} supply voltage ($V_{DD}/2$) before accessing a DRAM row {in a subarray}. To do so,} the \gls{pre} command prepares {the subarray} {for accessing data in DRAM cells} {using the precharge logic placed next to the sense amplifiers}.

{\head{Row Activation} To access a DRAM cell, the memory controller needs to open the DRAM row containing the cell. To do so, the memory controller issues an \gls{act} command.
An \gls{act} command is performed in \param{{four}} steps.
First, it drives {the target} wordline with a high voltage {level} to turn on the access transistors within the DRAM row {(i.e., open the DRAM row)}.
Second, turning on {an access transistor} initiates {the} \emph{charge sharing} process between the DRAM cell and its bitline.
Third, the charge sharing process causes a small deviation {in} the bitline voltage.
Fourth, {the sense amplifier is enabled to sense the voltage deviation on the bitline and amplify the bitline voltage to {the} level of {either the} \gls{vdd} or \gls{gnd} (depending on the voltage deviation {on the bitline}).} {In doing so, an \gls{act} command copies the data in the open DRAM row to the local row buffer.}

{\head{Column Access}}
{Once the open row is copied to the local row buffer, it can be accessed by \gls{rd} or {modified} by \gls{wr} column access commands in the local row buffer using the bank I/O {circuitry}.}
{Only one DRAM row in {a bank} can be open at a given time~\cite{jedec2020jesd794c, kim2012acase}.}

{\head{Timing Parameters}}
{DRAM specifications (e.g., DDR4~\cite{jedec2020jesd794c}) define timing parameters that the memory controller obeys while scheduling DRAM commands. {Four timing parameters are important to understand the rest of the paper. First,} consecutive row activation and column access commands (e.g., \gls{act} to \gls{rd}) must be separated in time by at least the \gls{trcd}. \gls{trcd} ensures that the deviation {i}n the bitline voltage exceeds the reliable sensing threshold of the sense amplifier during row activation~\cite{kim2019d,chang2016understanding}. {Second,} consecutive {\gls{act} and \gls{pre}} commands must be separated by at least the \gls{tras}. \gls{tras} ensures that the charge levels of all DRAM cells in the open row are fully restored before the row is closed. {Third,} consecutive precharge and row activation commands must be separated by at least the \gls{trp}. \gls{trp} ensures that the bitline is fully precharged to $V_{DD}/2$, so that the {next row activation} can be reliably performed{.}
{Fourth, {the} time window between two consecutive row activations targeting a DRAM bank, {i.e.,} \gls{trc} {must be at least} as large as the sum of \gls{tras} and \gls{trp}.}}}


\subsection{DRAM Refresh} 

Charge stored in the capacitor of a DRAM cell {leaks} over time. {Therefore, the charge in the cell's capacitor must be periodically restored (i.e., the DRAM cell must be \emph{refreshed}) to maintain data integrity.}
The time interval during which a cell can retain its charge without being refreshed is called the {cell's} \emph{retention time}. {A DRAM cell needs to be refreshed once every \gls{trefw}, which is typically \SI{64}{\milli\second} (e.g., in DDR4~\cite{jedec2020jesd794c}) or \SI{32}{\milli\second} (e.g., in DDR5~\cite{jedec2020jesd795}).}

{To perform refresh operations,} the memory controller {periodically issues} a \gls{ref} command {to a DRAM rank} {{after every} \gls{trefi} (e.g., \SI{7.8}{\micro\second}~\cite{jedec2020jesd794c} or {\SI{3.9}{\micro\second}~\cite{jedec2020jesd795}}).}
Each \gls{ref} command refreshes a {number} of rows in the DRAM chip {based on the chip's capacity. T}he DRAM chip
{internally decides} which rows {and how many rows} to refresh{, but does \emph{not} expose this information to the memory controller.} 

{Issuing a \gls{ref} command {makes the} DRAM rank unavailable for {a time window called \gls{trfc}, during which the rank {\emph{cannot}} receive any commands.}} {{Unfortunately,} \gls{trfc} needs to be large enough {(e.g., \SI{350}{\nano\second}~\cite{jedec2020jesd794c})} such that multiple rows can be refreshed with a \gls{ref} command.} {Thus, {issuing a \gls{ref} command can} increase {the access} latency {of memory requests} and cause system-wide slowdown.} With increasing DRAM chip density, more DRAM rows need to be refreshed, exacerbating the negative performance impact of DRAM refresh~\cite{nguyen2018nonblocking, liu2012raidr}. 

\subsection{RowHammer}
\label{sec:background_rowhammer}
Modern DRAM devices suffer from disturbance errors that happen when a DRAM row {(the aggressor row)} is repeatedly and rapidly activated~\cite{kim2014flipping, mutlu2017therowhammer, mutlu2019rowhammer_and}. These disturbance errors manifest {in DRAM rows neighboring the aggressor row (i.e., victim rows)} after the aggressor row's activation count {(i.e., hammer count)} reaches a certain threshold value within a refresh window, which we call {the \emph{RowHammer threshold ($N_{RH}$)}}~\cite{kim2020revisiting, kim2014flipping, orosa2021adeeper,yaglikci2022understanding}. {As} DRAM cells become smaller and closer to each other {with technology node scaling}, RowHammer vulnerability {becomes worse}~\rhworse{}.
Given the severity of {the} RowHammer {vulnerability}, {many prior works propose refreshing the potential victim rows to prevent RowHammer bitflips, which we call \emph{preventive refresh}~\rhdefrefresh{}}. 




==> mainmatter/08_hira/13_relatedwork_clean.tex <==
\section{Related Work}
\label{hira:sec:relatedwork}

{To our knowledge, this is the first work {to} demonstrate {that} 1)~real off-the-shelf DRAM chips are capable of {refreshing a DRAM row concurrently with refreshing or activating another row within the same DRAM bank,}
by {carefully} violating {DRAM} timing parameters and 2) {doing so} is beneficial {to reduce the performance overhead of both {\emph{periodic}} refresh operations {(required for reliable DRAM operation)} and {\emph{preventive}} refresh operations {(required for RowHammer bitflip prevention)}.}}
We classify the related work into {six} {main} categories. 




\noindent
{\textbf{Eliminating unnecessary refreshes~{(e.g., {\cite{liu2012raidr, lin2012secret, nair2013archshield,baek2013refresh, qureshi2015avatar,patel2017thereach,venkatesan2006retentionaware,khan2017detecting,khan2016parbor,khan2014theefficacy,isen2009eskimoenergy,liu2011flikker,khan2016acase, jung2015omitting,jafri2021refresh, katayama1999faulttolerant, wilkerson2010reducing, ghosh2007smart, song2000method, emma2008rethinking, mukhanov2019workloadaware, hong2018eareccaided, kraft2018improving, park2011power, wang2018content, kim2020chargeaware}}).}}
Various prior works eliminate unnecessary refresh operations by leveraging the heterogeneity in the retention time of DRAM cells to reduce the rate at which {some or all} DRAM rows are refreshed.
Our {work} differs from these {works} in {two} key aspects.
{First,} {most of} these works rely on identifying cells or rows with worst-case retention times, which is a difficult problem~\cite{mrozek2010analysis,mrozek2019multirun, patel2017thereach, liu2012raidr, qureshi2015avatar, liu2013anexperimental}. {In contrast,} our work} uses a {relatively simple} {and well-understood} one-time {experiment} to {1)~identify \gls{hira}'s coverage and 2)~verify that \gls{hira} reliably works, presented in \secref{hira:sec:experiments_coverage} and \secref{hira:sec:experiments_chargerestoration}, respectively. Second, these works} focus on reducing the performance overhead of periodic refreshes, {but \emph{not} the increasingly worsening performance overhead of preventive refresh {operations} of RowHammer defenses~\rhdefworse{}. In contrast, our work tackles the performance overheads of} \emph{both} periodic and preventive refreshes. 


\noindent
{\textbf{Circuit-level modifications to reduce the {performance impact} of refresh operation{s} {(e.g., \cite{hassan2019crow, luo2020clrdram, kim2000dynamic, kim2003blockbased,yanagisawa1988semiconductor,ohsawa1998optimizing,nair2014refresh,orosa2021codic, choi2020reducing})}.}}
{{These} works develop DRAM-based techniques that 1)~reduce the latency of a refresh operation~\cite{hassan2019crow, luo2020clrdram}, {2)~implement a new refresh command that can be interrupted to quickly perform main memory accesses~\cite{nair2014refresh}}, and 3)~reduce the rate at which some or all DRAM rows are refreshed~\cite{kim2000dynamic,kim2003blockbased,yanagisawa1988semiconductor,ohsawa1998optimizing}. {As opposed to \doduo{},} the{se techniques}} {1)} are \emph{not} compatible with {existing} DRAM chips as they require modifications {to} DRAM circuitry,
{and} 2) \emph{cannot} hide DRAM access latency in the presence of refresh operations. 


\noindent
{\textbf{Memory {access} scheduling techniques to reduce the performance impact of refresh operations (e.g.,~\cite{mukundan2013understanding,stuecheli2010elastic, chang2014improving, pan2019thecolored, pan2019hiding, kotra2017hardwaresoftware}).}}
{{Several} works {propose 
{issuing} $REF$ commands} during \emph{DRAM idle time} {(where no memory access requests {are} scheduled)} {to reduce the performance impact of refresh operations.} {{Most of these} works leverage} {the flexibility of delaying a $REF$ command for {multiple refresh intervals (e.g., for \SI{70.2}{\micro\second} in DDR4~\cite{jedec2020jesd794c})}}. In contrast, \gls{hira} overlaps the latency of a refresh operation with other refreshes or memory accesses and thus can reduce the performance impact of refresh operations \emph{without} relying on {DRAM} idle time.} 

\noindent
{\textbf{Modifications to the DRAM architecture to leverage subarray-level parallelism {(e.g.,~\salprefs{})}.} Several works
partially overlap the latency of refresh operations or \memaccs{} via modifications to the DRAM architecture. {The \gls{hira} operation builds on the basic idea{s} of subarray-level parallelism introduced in~\cite{kim2012acase} and {refresh-access parallelization introduced in}~\cite{chang2014improving,zhang2014cream}}. {However,} unlike \doduo{}, these works require modifications to DRAM chip design, {and} thus they are \emph{not} compatible with {off-the-shelf} DRAM chips.} In contrast, {\doduo{}} uses {existing} {\gls{act} and \gls{pre}} commands{, {and we demonstrate that it works on real off-the-shelf DRAM chips}}.

\noindent
{\textbf{RowHammer defense mechanisms {that use preventive refresh operations} {(e.g.,~\rhdefrefresh{})}.} {These works} propose} mechanisms that observe memory access patterns and speculatively schedule {preventive} refresh operations targeting potential victim rows of a RowHammer attack. {\doduo{} can be combined with all of these mechanisms to reduce the {performance} overhead{s of} preventive refresh {operations}.}  





{\head{{Reducing the latency of {major} DRAM operations} {(e.g.,~\cite{hassan2016chargecache, das2018vrldram, wang2018reducing, zhang2016restore, shin2014nuat, lee2013tieredlatency, lee2015adaptivelatency, kim2018solardram,chang2016understanding, chang2017understanding, lee2017designinduced,chandrasekar2014exploiting,shin2015dramlatency_optimization})}}} 
{{Many} {works}} {develop techniques that} {\emph{reduce}} the {latency of {major} DRAM operations (e.g., \gls{act}, \gls{pre}, \gls{rd}, \gls{wr}) by leveraging {1)}~temporal locality in workload access patterns~\cite{hassan2016chargecache,das2018vrldram,wang2018reducing,zhang2016restore,shin2014nuat}{,} 2)~the guardbands in manufacturer-recommended DRAM timing parameters~\cite{lee2013tieredlatency,lee2015adaptivelatency,kim2018solardram,chang2016understanding,lee2017designinduced, chang2017understanding}{, and 3)~variation in DRAM {latency} due to temperature dependence~\cite{chandrasekar2014exploiting,lee2015adaptivelatency,kim2018solardram}.}}
{{These latency reduction techniques} can improve system performance by alleviating the performance impact of refresh operations (e.g., a refresh can be performed {faster} with a reduced charge restoration latency).}
{These techniques can be combined with \doduo{} to further alleviate the performance impact of refresh operations, as \doduo{} \emph{overlaps} 
the latency of refreshing a DRAM row 
with the latency of refreshing or {activating} another row {in the same bank}.}






==> mainmatter/08_hira/15_acknowledgements_clean.tex <==
\section*{Acknowledgments}
We thank our shepherd and the reviewers of ASPLOS'22, ISCA'22, and MICRO'22 for valuable feedback. We thank the SAFARI Research Group members for {useful} feedback and the stimulating intellectual environment they provide. We acknowledge the generous gifts provided by our industrial partners{, including} Google, Huawei, Intel, Microsoft, and VMware{, and support from {the} Microsoft Swiss Joint Research Center}. 

==> mainmatter/08_hira/16_appdimmtable_clean.tex <==
\section{Tested DRAM Chips}
\label{hira:sec:appendix_chips}
\providecommand*{\myalign}[2]{\multicolumn{1}{#1}{#2}}

\agyarb{Table~\ref{hira:tab:detailed_info} shows the characteristics of the DDR4 DRAM modules we test and analyze. {We provide {the} access frequency (Freq.), manufacturing date (Date Code), {chip} capacity (Chip Cap.), die revision {(Die Rev.)}, and chip organization {(Chip Org.)} of tested DRAM modules. We report the manufacturing date of these modules in the form of $week-year$. For each DRAM module, Table~\ref{hira:tab:detailed_info} shows two \gls{hira} characteristics in terms of minimum (Min.), average (Avg.) and maximum (Max.) values across all tested rows: 
1)~HiRA Coverage: the fraction of DRAM rows
within a bank which HiRA can reliably activate concurrently
with refreshing a given row (\secref{hira:sec:experiments_coverage})
and 2)~Norm. $N_{RH}$: the increase in the RowHammer threshold when \gls{hira}'s second row activation is used for refreshing the victim row (\secref{hira:sec:experiments_chargerestoration}).}}
\setlength{\tabcolsep}{5.5pt}
\begin{table*}[ht]
\footnotesize
\centering
\caption{Characteristics of the tested DDR4 DRAM modules.}
\label{hira:tab:detailed_info}
\resizebox{\columnwidth}{!}{
\begin{tabular}{l|l|l||ccccc|ccc|ccc}
\head{Module} & \textbf{Module} & \textbf{Module Identifier} & \textbf{Freq} & \textbf{Date} & \textbf{Chip} & \textbf{Die} & \textbf{Chip} & \multicolumn{3}{c|}{\textbf{HiRA Coverage}} & \multicolumn{3}{c}{\textbf{Norm. $N_{RH}$}} \\ 
\head{Label}&\textbf{Vendor}&\textbf{Chip Identifier}&\textbf{(MT/s)}&\textbf{Code}&\textbf{Cap.}&\textbf{Rev.}&\textbf{Org.}&\textbf{Min.}&\textbf{Avg.}&\textbf{Max.}&\textbf{Min.}&\textbf{Avg.}&\textbf{Max.}\\
\hline
\hline
A0 & \multirow{2}{*}{G.SKILL} & \multirow{2}{*}{\begin{tabular}[l]{@{}l@{}}DWCW (Partial Marking)$^*$\\F4-2400C17S-8GNT~\cite{gskill2021f42400c17s8gnt}\end{tabular}} & \multirow{2}{*}{2400} & \multirow{2}{*}{42-20} & \multirow{2}{*}{4Gb} & \multirow{2}{*}{B} & \multirow{2}{*}{x8} & \SI{24.8}{\percent} & \SI{25.0}{\percent} & \SI{25.5}{\percent} & 1.75&1.90&2.52\\
A1 & & & & & & & & \SI{24.9}{\percent} & \SI{26.6}{\percent} & \SI{28.3}{\percent} & 1.72 & 1.94 & 2.55 \\ \hline
B0 & \multirow{2}{*}{Kingston} & \multirow{2}{*}{\begin{tabular}[l]{@{}l@{}}H5AN8G8NDJR-XNC\\KSM32RD8/16HDR~\cite{datasheetksm32rd8}\end{tabular}} & \multirow{2}{*}{2400} & \multirow{2}{*}{48-20} & \multirow{2}{*}{4Gb} & \multirow{2}{*}{D} & \multirow{2}{*}{x8} & \SI{25.1}{\percent} & \SI{32.6}{\percent} & \SI{36.8}{\percent} & 1.71&1.89&2.34\\
B1 & & & & & & & & \SI{25.0}{\percent} & \SI{31.6}{\percent} & \SI{34.9}{\percent} & 1.74&1.91&2.51\\ \hline
C0 & \multirow{3}{*}{SK Hynix} & \multirow{3}{*}{\begin{tabular}[l]{@{}l@{}}H5ANAG8NAJR-XN\\HMAA4GU6AJR8N-XN~\cite{memorynethmaa4gu6ajr8nxn}\end{tabular}} & \multirow{3}{*}{2400} & \multirow{3}{*}{51-20} & \multirow{3}{*}{4Gb} & \multirow{3}{*}{F} & \multirow{3}{*}{x8} & \SI{25.3}{\percent} & \SI{35.3}{\percent} & \SI{39.5}{\percent} & 1.47 & 1.89 & 2.23 \\ 
C1 & & & & & & & & \SI{29.2}{\percent} & \SI{38.4}{\percent} & \SI{49.9}{\percent} & 1.09 & 1.88 & 2.27\\ 
C2 & & & & & & & & \SI{26.5}{\percent} & \SI{36.1}{\percent} & \SI{42.3}{\percent} & 1.49 & 1.96 & 2.58\\ \hline
\hline
\end{tabular}
}
\begin{flushleft}
$^*$ The chip identifier is partially removed on these modules. We infer the chip manufacturer and die revision based on the remaining part of the chip identifier.

\end{flushleft}
\end{table*}

\iffalse
\section{Appendix II: Detailed Security Analysis for PARA {[STALE]}}
\label{hira:sec:appendix_para}


\subsection{Threat Model}
\label{hira:sec:appendix_threat_model}
We assume a comprehensive {RowHammer} threat model,\cqlabel{hira:CQ4} similar to {that assumed by} state-of-the-art works~\cite{kim2014flipping, park2020graphene, yaglikci2021blockhammer}, in which the attacker can 1)~fully utilize memory bandwidth, 2)~precisely time each memory request, and 3)~comprehensively and accurately know details of the memory controller and the DRAM chip. We do not consider any hardware or software component to be trusted or safe except {we assume that the DRAM commands issued by the memory controller are performed within the DRAM chip as intended.}

\subsection{Revisiting PARA's configuration methodology}
\label{hira:sec:appendix_revisitingpara}
Kim et al.~\cite{kim2014flipping} {configure} PARA's probability threshold (\gls{pth}), assuming {that} the attacker hammers an aggressor row {\emph{only enough times, but no more}}.
{With} more than an order of magnitude decrease in {the} {RowHammer threshold} in the last decade\cite{kim2020revisiting, frigo2020trrespass, hassan2021uncovering, orosa2021adeeper, yaglikci2022understanding}, an attacker can {complete a RowHammer attack 144 times {within a refresh window of \SI{64}{\milli\second}},\footnote{{\Gls{hcfirst} for modern DRAM chips is as low as 9600~\cite{kim2020revisiting}. Assuming a \gls{trc} of \SI{46.25}{\nano\second}, performing 9600 row activations can be completed \emph{only} in \SI{444}{\micro\second}, which is 1/144.14 of a nominal refresh window of \SI{64}{\milli\second}. {As such, an attacker can perform 9600 activations for 144 times within a \SI{64}{\milli\second} refresh window.}}}}
{requiring {a} revisit {of PARA's configuration methodology}.\footnote{A concurrent work also revisits PARA's configuration methodology~\cite{saroiu2022howto}.}}

{The rest of this section explains how we {calculate}} \gls{pth} for a given RowHammer threshold.
\figref{hira:fig:app_para_fsm} shows the probabilistic state machine that we use to 
calculate the {hammer count, which we define as the number of aggressor row activations} that may affect a victim row during a RowHammer attack.
Initially the {hammer count} is zero (state~0). When an {aggressor row} {is} activated, PARA {triggers a \emph{preventive} refresh with a probability of $\pth{}$. Since there are two rows that are adjacent to the activated row, PARA} refreshes {the} victim row with a probability of $\pth{}/2$, {in which case the {hammer} count is reset.} {Therefore,} the {hammer} count {{is incremented} with a probability of $1-\pth{}/2$ upon an {aggressor row} activation}. An attack is considered to be \emph{successful} if {its hammer count} reaches the RowHammer threshold {($N_{RH}$)} within a \glsfirst{trefw}. 

\begin{figure}[!ht]
    \centering
    \includegraphics[width=0.8\linewidth]{mainmatter/08_hira/figures/hira_fig9_low.png}
    \caption{Probabilistic state machine of an aggressor row's activation count in a PARA-protected system}
    \label{hira:fig:app_para_fsm}
\end{figure}

{Because the time delay between two row activations targeting the same {bank} \emph{cannot} be smaller than \gls{trc}, an} attacker can perform {a maximum of} $\trefw{}/\trc{}$ state transitions within a \gls{trefw}. 
To account for all possible access patterns, we model a successful RowHammer attack as a set of failed attempts (i.e., the victim row is refreshed before the {hammer} count reaches {the} RowHammer threshold), followed by a successful attempt {(i.e., the victim row is {\emph{not}} refreshed until the {hammer} count reaches {the} RowHammer threshold)}. {To {calculate} \gls{pth} we follow a {five-}step approach. First, we calculate the probability of a failed attempt ($p_f$) and a successful attempt ($p_s$). Second, we calculate the probability of a {\emph{successful}} RowHammer attack that consists of a number ($N_f$) of failed attempts, followed by a successful attempt, {denoted as $p_{success}(N_f)$}.
Third, we calculate the {overall} probability of a \emph{successful} RowHammer attack ($p_{RH}$) for all possible number of failed attempts ($N_f$). Fourth, we extend the probability calculation to account for \gls{trrslack}. Fifth, we calculate \gls{pth} for a given failure probability target.}

\subsubsection{{Step {1}: Failed and successful attempts}}
\label{hira:sec:}
Expression~\ref{hira:exp:app_failedattempt} {shows} $p_{f}(HC)$: the probability of a {\emph{failed} attempt with a given hammer count ($HC$). The attempt contains 1)~$HC$ consecutive aggressor row activations that do \emph{not} trigger a preventive} refresh, $(1-\pth{}/2)^{HC}$, {where $HC$ is smaller than the RowHammer threshold ($N_{RH}$)}, {and 2)~}an {aggressor row} activation {that triggers} a {preventive} refresh $(\pth{}/2)$.


\equ{p_{f}(HC) = (1-\pth{}/2)^{HC}\times\pth{}/2,~where~1\leq HC<N_{RH}}{exp:app_failedattempt}


{Similarly, we calculate the probability of a \emph{successful} attempt which has $N_{RH}$ consecutive aggressor row activations that do \emph{not} trigger a preventive refresh $p_{s} = (1-p_{th}/2)^{N_{RH}}$.}


\head{{Step {2}: Successful RowHammer attack with $N_f$ failed attempts}}
{We formulate the probability of a successful RowHammer attack that contains $N_f$ failed attempts{. Since a failed attempt may have a hammer count value in the range $[1, N_{RH})$, we account} for all possible hammer count {values} that {a failed attempt might have}.}
{Expression~\ref{hira:exp:app_nconsecutivefailedattempts} shows the probability of {a RowHammer attack to} experience {a given number of (}$N_f${)} consecutive failed attempts.}
\equ{\prod_{i=1}^{N_{f}} p_f(HC_i)=\prod_{i=1}^{N_{f}}((1-\pth{}/2)^{HC_i}\times\pth{}/2)~, where~1\leq HC_{i} < \hcfirst{}}{exp:app_nconsecutivefailedattempts}
    

{Using Expression~\ref{hira:exp:app_nconsecutivefailedattempts}, we calculate the probability of a successful RowHammer attack that contains $N_f$ failed attempts. To do so, we simplify Expression~\ref{hira:exp:app_nconsecutivefailedattempts} by 1)~evaluating the product on both terms: $(1-p_{th}/2)^{HC_i}$ and $p_{th}/2$ and 2)~multiplying the probability of $N_f$ failed attempts with the probability of a successful attempt ($p_s=(1-p_{th}/2)^{N_{RH}}$).}
{Expression}~\ref{hira:exp:app_successfulattack} shows the probability of a successful RowHammer attack {that contains $N_f$ failed attempts.}




\equ{p_{success}(N_{f}) = (1-{\pth{}}/{2})^{\sum_{i=1}^{N_{f}} {HC_{i}}} \times ({\pth{}}/{2})^{N_{f}} \times (1-{\pth{}}/{2})^{\hcfirst{}}}{exp:app_successfulattack}

To account for the worst-case, we maximize the probability of a successful RowHammer attack {that includes $N_{f}$ failed attempts} ($p_{success}(N_{f})$). {To do so, we choose} the worst possible value for each $HC_{i}$ {value}. \textbf{Intuitively}, {the number of activations in a failed attempt should be minimized. Since} a failed attempt {has to perform at least one activation,
we conclude that all failed attempts} fail after only one row activation in the worst case. 
\head{Mathematically,} {our goal is} to maximize $p_{success}(N_{f})$. {{Since} $\pth{}$ is a value between zero and one,} we minimize the term $\sum_{i=1}^{N_{f}} {HC_{i}}$ to maximize $p_{success}(N_{f})$. Thus, we derive Expression~\ref{hira:exp:app_prhn} {by choosing $HC_i=1$ to achieve} the maximum probability of a successful RowHammer attack with $N_{f}$ failed attempts. 

\equ{
p_{success}(N_{f}) = (1-{\pth{}}/{2})^{N_{f}+\hcfirst{}} \times ({\pth{}}/{2})^{N_{f}}}{exp:app_prhn}

\head{{Step 3: All possible successful RowHammer attacks}}
{Equation~\ref{hira:exp:app_prh} shows the probability of a successful RowHammer attack ($p_{RH}$), as the sum of all possible $p_{success}(N_f)$ values.}
{$N_{f}$ can be as small as 0 if {the} RowHammer attack does \emph{not} include any failed attempt and as large as} the maximum number of failed attempts that can fit in a refresh window {(\gls{trefw})} {if the RowHammer attack includes a successful attempt}.
{To find the maximum value that $N_{f}$ can {take}, we calculate the longest time that a successful RowHammer attack can take.} Since $HC_i=1$ in the worst case, each failed attempt {costs only two row} activations ($2\times\trc{}$){:} {one aggressor row activation and one activation for preventively refreshing the victim row}. Thus, the execution time of a successful RowHammer attack with $N_{f}$ attempts is $(2N_{f}+\hcfirst{})\times\trc{}$. {Therefore,} the maximum $N_{f}$ value is ${N_{f}}_{max} = ((\trefw{}/\trc{})-\hcfirst{})/2$.

\equ{p_{RH} = \sum_{N_{f}=0}^{{N_{f}}_{max}} p_{success}(N_{f}),~~~{N_{f}}_{max} = (\trefw{}/\trc{}-\hcfirst{})/2}{exp:app_prh}

Using {Expressions}~\ref{hira:exp:app_prhn} and~\ref{hira:exp:app_prh}, we compute the success probability of a RowHammer attack for a given probability threshold of PARA ($p_{th}$). 


\head{{Step 4: Accounting for \gls{trrslack}}}
The original PARA proposal~\cite{kim2014flipping} performs a {preventive} refresh immediately after the activated row is closed. However, \gls{hirasched} allows a {preventive} refresh to be queued until an assigned deadline. {Since the aggressor rows can be activated while a preventive refresh request is queued, we update Equations~\ref{hira:exp:app_prhn} and~\ref{hira:exp:app_prh}, assuming the worst case, where an aggressor row is activated as many times as possible {within \gls{trrslack} ({i.e.,} the maximum amount of time} the preventive refresh is queued).}
 guaranteed to be the max amount of time?\\Ata: Yes, HIRA-MC makes sure to issue preventive refreshes within \gls{trrslack}}To do so, we {update} Expression~\ref{hira:exp:app_prh}, {by} reducing {the RowHammer threshold ($N_{RH}$)} by {\gls{hcdeadline}}. Thus, we calculate ${N_{f}}_{max}$ and $\prh{}$ as shown in Expressions~\ref{hira:exp:app_nmax} and~\ref{hira:exp:app_prhdl}, respectively. 

\begin{equation}\footnotesize
{N_{f}}_{max} = ((\trefw{}/\trc{})-\hcfirst{}-{\hcdeadline{}})/2
\label{hira:exp:app_nmax}
\end{equation}

\equ{P_{RH} = \sum_{N_{f}=0}^{{N_{f}}_{max}} (1-{\pth{}}/{2})^{{N_{f}}+\hcfirst{}-{\hcdeadline{}}} \times ({\pth{}}/{2})^{N_{f}}}{exp:app_prhdl}



\head{{Step 5: Finding $p_{th}$}}
{We iteratively evaluate Expressions~\ref{hira:exp:app_nmax} and \ref{hira:exp:app_prhdl} to find} \gls{pth} for a {target} {RowHammer success probability of {$10^{-15}$}, as a typical consumer memory reliability target~\cite{cai2012error, cai2017error, jedec2012jep122g, luo2016enabling, patel2017thereach, yaglikci2021blockhammer, kim2020revisiting, micheloni2015apparatus}}.


\fi

==> mainmatter/08_hira/17_appsecurityproof_clean.tex <==
\section{Appendix II: Detailed Security Analysis for PARA}
\label{hira:sec:app_revisitingpara}

\head{Threat Model} We assume a comprehensive {RowHammer} threat model,\cqlabel{hira:CQ4} similar to {that assumed by} state-of-the-art works~\cite{kim2014flipping, park2020graphene, yaglikci2021blockhammer}, in which the attacker can 1)~fully utilize memory bandwidth, 2)~precisely time each memory request, and 3)~comprehensively and accurately know details of the memory controller and the DRAM chip. We do not consider any hardware or software component to be trusted or safe except {we assume that the DRAM commands issued by the memory controller are performed within the DRAM chip as intended.}


\head{PARA-Legacy} \agyarb{In this analysis we refer to the original design of PARA}~\cite{kim2014flipping} \agyarb{as \emph{PARA-Legacy}. PARA-Legacy} {configures} PARA's probability threshold (\gls{pth}), assuming {that} the attacker hammers an aggressor row {\emph{only enough times, but no more}}.
{With} more than an order of magnitude decrease in {the} {RowHammer threshold} in the last decade\cite{kim2020revisiting, frigo2020trrespass, hassan2021uncovering, orosa2021adeeper, yaglikci2022understanding}, \agyarb{it is possible for a memory access pattern to reach a hammer count as large as the RowHammer threshold 144 times} {within a refresh window of \SI{64}{\milli\second}},\footnote{{\Gls{hcfirst} for modern DRAM chips is as low as 9600~\cite{kim2020revisiting}. Assuming a \gls{trc} of \SI{46.25}{\nano\second}, performing 9600 row activations can be completed \emph{only} in \SI{444}{\micro\second}, which is 1/144.14 of a nominal refresh window of \SI{64}{\milli\second}. {As such, an attacker can perform 9600 activations for 144 times within a \SI{64}{\milli\second} refresh window.}}}
{requiring {a} revisit {of PARA's configuration methodology}.\footnote{A concurrent work also revisits PARA's configuration methodology~\cite{saroiu2022howto}.}}

\head{Our Approach in High Level}
\figref{hira:fig:app_para_fsm} shows the probabilistic state machine that we use to 
calculate the {hammer count, which we define as the number of aggressor row activations} that may affect a victim row during a RowHammer attack.
Initially the {hammer count} is zero (state~0). When an {aggressor row} {is} activated, PARA {triggers a \emph{preventive} refresh with a probability of $\pth{}$. Since there are two rows that are adjacent to the activated row, PARA} refreshes {the} victim row with a probability of $\pth{}/2$, {in which case the {hammer} count is reset.} {Therefore,} the {hammer} count {{is incremented} with a probability of $1-\pth{}/2$ upon an {aggressor row} activation}. A \agyarb{memory access pattern is considered to be \emph{a successful RowHammer access pattern} when} {the hammer count} reaches the RowHammer threshold {($N_{RH}$)} within a \glsfirst{trefw}. 

\begin{figure}[!ht]
    \centering
    \includegraphics[width=0.8\linewidth]{mainmatter/08_hira/figures/hira_fig9_low.png}
    \caption{Probabilistic state machine of {hammer} count in a PARA-protected system}
    \label{hira:fig:app_para_fsm}
\end{figure}

{Because the time delay between two row activations targeting the same {bank} \emph{cannot} be smaller than \gls{trc}, an} attacker can perform {a maximum of} $\trefw{}/\trc{}$ state transitions within a \gls{trefw}. 
To account for all possible access patterns, we model a \emph{successful RowHammer {access pattern}} as a set of failed attempts (i.e., the victim row is refreshed before the {hammer} count reaches {the} RowHammer threshold), followed by a successful attempt {(i.e., the victim row is {\emph{not}} refreshed until the {hammer} count reaches {the} RowHammer threshold)}. {To {calculate} \gls{pth}{,} we follow a {five-}step approach. First, we calculate the probability of a failed attempt ($p_f$) and a successful attempt. Second, we calculate {the probability of observing a number ($N_f$) of consecutive failed attempts.}Third, we calculate
{\emph{the {overall} RowHammer success probability ($p_{RH}$)} as the overall probability of {\emph{all} possible successful RowHammer access patterns.}}
Fourth, we extend the probability calculation to account for \gls{trrslack}. Fifth, we calculate \gls{pth} for a given failure probability target.}

\head{{Step {1}: Failed and successful attempts}}
\expref{hira:exp:app_failedattempt} {shows} $p_{f}(HC)$: the probability of a {\emph{failed} attempt with a given hammer count ($HC$). The attempt contains 1)~$HC$ consecutive aggressor row activations that do \emph{not} trigger a preventive} refresh, $(1-\pth{}/2)^{HC}$, {where $HC$ is smaller than the RowHammer threshold ($N_{RH}$)}, {and 2)~}an {aggressor row} activation {that triggers} a {preventive} refresh $(\pth{}/2)$.


\equ{p_{f}(HC) = (1-\pth{}/2)^{HC}\times\pth{}/2,~where~1\leq HC<N_{RH}}{hira:exp:app_failedattempt}

{Similarly, we calculate the probability of a \emph{successful} attempt which has $N_{RH}$ consecutive aggressor row activations that do \emph{not} trigger a preventive refresh {as} $(1-p_{th}/2)^{N_{RH}}$.}


\head{{Step {2}: {The probability of} ${\bm{N_f}}$ {consecutive} failed attempts}}
{{Since a failed attempt may have a hammer count value in the range $[1, N_{RH})$, we account} for all possible hammer count {values} that {a failed attempt might have}.}
{\expref{hira:exp:app_nconsecutivefailedattempts} shows the probability of {a given number of (}$N_f${)} consecutive failed attempts.}
\equ{\prod_{i=1}^{N_{f}} p_f(HC_i)=\prod_{i=1}^{N_{f}}((1-\pth{}/2)^{HC_i}\times\pth{}/2)~, where~1\leq HC_{i} < \hcfirst{}}{hira:exp:app_nconsecutivefailedattempts}
    


\head{{Step 3: {Overall} RowHammer success probability}}
{To find the overall RowHammer success probability, we 1)~calculate the probability of the \emph{successful RowHammer access pattern which consists of $N_f$ consecutive failed attempts and one successful attempt ($p_{success}(N_{f})$)} for each possible value that $N_f$ can take and 2)~sum up the probability of all possible successful RowHammer access patterns: $\sum{p_{success}(N_f)}$.}
To do so, {we} multiply \expref{hira:exp:app_nconsecutivefailedattempts} with the probability of a successful attempt: $(1-p_{th}/2)^{N_{RH}}$.
{\expref{hira:exp:app_successfulattack}} shows {how we calculate $p_{success}(N_{f})$.} We derive \expref{hira:exp:app_successfulattack} by evaluating the product on both terms in \expref{hira:exp:app_nconsecutivefailedattempts}: $p_{th}/2$ and $(1-p_{th}/2)^{HC_i}$.




\equ{p_{success}(N_{f}) = (1-{\pth{}}/{2})^{\sum_{i=1}^{N_{f}} {HC_{i}}} \times ({\pth{}}/{2})^{N_{f}} \times (1-{\pth{}}/{2})^{\hcfirst{}}}{hira:exp:app_successfulattack}

To account for the worst-case, we maximize 
$p_{success}(N_{f})$ {by choosing} the worst possible value for each $HC_{i}$ {value}. \textbf{Intuitively}, {the number of activations in a failed attempt should be minimized. Since} a failed attempt {has to perform at least one activation,
we conclude that all failed attempts} fail after only one row activation in the worst case. 
\head{Mathematically,} {our goal is} to maximize $p_{success}(N_{f})$. {{Since} $\pth{}$ is a value between zero and one,} we minimize the term $\sum_{i=1}^{N_{f}} {HC_{i}}$ to maximize $p_{success}(N_{f})$. Thus, we derive \expref{hira:exp:app_prhn} {by choosing $HC_i=1$ to achieve} {the maximum (worst-case) $p_{success}(N_{f})$.}

\equ{
p_{success}(N_{f}) = (1-{\pth{}}/{2})^{N_{f}+\hcfirst{}} \times ({\pth{}}/{2})^{N_{f}}}{hira:exp:app_prhn}

{{\expref{hira:exp:app_prh}} shows {{the overall} RowHammer success probability} ($p_{RH}$), as the sum of all possible $p_{success}(N_f)$ values.}
{$N_{f}$ can be as small as 0 if {the} RowHammer attack does \emph{not} include any failed attempt and as large as} the maximum number of failed attempts that can fit in a refresh window {(\gls{trefw}) {together with a successful attempt}}.
Since $HC_i=1$ in the worst case, each failed attempt {costs only two row} activations ($2\times\trc{}$){:} {one aggressor row activation and one activation for preventively refreshing the victim row}. Thus, the execution time of $N_{f}$ {failed} attempts, {followed by one successful attempt is} $(2N_{f}+\hcfirst{})\times\trc{}$. {Therefore,} the maximum {value $N_{f}$ can take within a refresh window (\gls{trefw})} is ${N_{f}}_{max} = ((\trefw{}/\trc{})-\hcfirst{})/2$.

\equ{p_{RH} = \sum_{N_{f}=0}^{{N_{f}}_{max}} p_{success}(N_{f}),~~~{N_{f}}_{max} = (\trefw{}/\trc{}-\hcfirst{})/2}{hira:exp:app_prh}

Using {\expsref{hira:exp:app_prhn}} and~\ref{hira:exp:app_prh}, we compute the {{overall} RowHammer success probability} for a given {PARA} probability threshold ($p_{th}$). 


\head{{Step 4: Accounting for \gls{trrslack}}}
The original PARA proposal~\cite{kim2014flipping} performs a {preventive} refresh immediately after the activated row is closed. However, \gls{hirasched} allows a {preventive} refresh to be queued {for a time window as long as \gls{trrslack}}. {Since the aggressor rows can be activated while a preventive refresh request is queued, we update {~\expsref{hira:exp:app_prhn}} and~\ref{hira:exp:app_prh}, assuming the worst case, where an aggressor row is activated as many times as possible {within \gls{trrslack} ({i.e.,} the maximum amount of time} the preventive refresh is queued).}
To do so, we {update} \expref{hira:exp:app_prh}: {we reduce} {the RowHammer threshold ($N_{RH}$)} by {\gls{hcdeadline}}. Thus, we calculate ${N_{f}}_{max}$ and $\prh{}$ as shown in \expsref{hira:exp:app_nmax} and~\ref{hira:exp:app_prhdl}, respectively. 

\begin{equation}\footnotesize
{N_{f}}_{max} = ((\trefw{}/\trc{})-\hcfirst{}-{\hcdeadline{}})/2
\label{hira:exp:app_nmax}
\end{equation}

\equ{p_{RH} = \sum_{N_{f}=0}^{{N_{f}}_{max}} (1-{\pth{}}/{2})^{{N_{f}}+\hcfirst{}-{\hcdeadline{}}} \times ({\pth{}}/{2})^{N_{f}}}{hira:exp:app_prhdl}



\head{{Step 5: Finding $\bf{p_{th}}$}}
{We iteratively evaluate \expsref{hira:exp:app_nmax} and \ref{hira:exp:app_prhdl} to find} \gls{pth} for a {target} {{overall} RowHammer success probability of {$10^{-15}$}, as a typical consumer memory reliability target {(see, e.g.,~\cite{cai2012error, cai2017error, jedec2012jep122g, luo2016enabling, patel2017thereach, yaglikci2021blockhammer, kim2020revisiting, micheloni2015apparatus})}}.

\subsubsection{{Results}}


{We refer to {the} original PARA work~\cite{kim2014flipping} as PARA-Legacy. PARA-Legacy calculates {{the overall} RowHammer success probability} as ${p_{RH_{Legacy}}=(1-p_{th}/2)^{N_{RH}}}$ with an optimistic assumption that the attacker hammers an aggressor row \emph{only enough times, but no more}. To mathematically compare {{the overall} RowHammer success probability} that we calculate ($p_{RH}$) with $p_{RH_{Legacy}}$, we reorganize \expref{hira:exp:app_prhdl}, which already includes ${p_{RH_{Legacy}}=(1-p_{th}/2)^{N_{RH}}}$, and derive \expref{hira:exp:app_prhdiff}.}

\equ{
p_{RH} =k \times p_{RH_{Legacy}},~where~k = (1-\frac{\pth{}}{2})^{-{\hcdeadline}}\sum_{N_{f}=0}^{{N_{f}}_{max}}(\frac{\pth{}}{2}(1-\frac{\pth{}}{2}))^{{N_{f}}}
}{hira:exp:app_prhdiff}

{
\expref{hira:exp:app_prhdiff} shows that $p_{RH}$ {is a multiple of} $p_{RH_{Legacy}}$ by a factor of $k$, {where $k$ depends on a given system's properties (e.g., $N_{f_{max}}$)} and PARA's configuration (e.g., \gls{pth}).
{To understand the difference between $p_{RH}$ and $p_{RH_{Legacy}}$, we evaluate \expref{hira:exp:app_prhdiff} for different RowHammer threshold values.\footnote{{We calculate for $N_{RefSlack}=0$, $t_{REFW}=64ms$, and $t_{RC}=46.25ns$.}}}
For {old DRAM chips (manufactured in} 2010-2013)~\cite{kim2014flipping}, $k$ is 1.0005 {(for $N_{RH}=50K$ and $p_{th}=0.001$~\cite{kim2014flipping})}, causing \emph{only} \SI{0.05}{\percent} variation in PARA's reliability target. {However,for future DRAM chips with $N_{RH}$ values of 1024 and 64 {($p_{th}$ values of 0.4730 and 0.8341)}, $k$ becomes 1.0331 and 1.3212, respectively. Therefore, the difference between {the two probabilities, $p_{RH}$ and $p_{RH_{Legacy}}$,} significantly increases as RowHammer worsens.}}

==> sorted_citationblocks.tex <==
\newcommand{\rhmemisolationrefs}[0]{\cite{aga2017when, agarwal2018rowhammer_for, barenghi2018softwareonly, bhattacharya2016curious, bhattacharya2018advanced, bosman2016dedup, brasser2017cant, burleson2016invited, carre2018openssl, cohen2022hammerscope, cojocar2019exploiting, cojocar2020arewe, deridder2021smash, fahrjr2022when, fournaris2017exploiting, frigo2018grand, frigo2020trrespass, genssler2022onthe, gruss2015rowhammerjs_a, gruss2018another, hassan2021uncovering, hong2019terminal, jang2017sgxbomb, jattke2022blacksmith, ji2019pinpoint, khan2018analysis, kim2014flipping, kim2020revisiting, kogler2022halfdouble, kwong2020rambleed, li2014write, lim2017active, lipp2018nethammer, liu2022generating, mutlu2017therowhammer, mutlu2019rowhammer_a, mutlu2023fundamentally, ni2018write, orosa2021adeeper, orosa2022spyhammer, park2016experiments, park2016statistical, pessl2016drama_exploiting, poddebniak2018attacking, qiao2016anew, rakin2022deepsteal, razavi2016flip, ryu2017overcoming, safari2014rowhammer, seaborn2015exploiting, tatar2018defeating, tatar2018throwhammer, tobah2022spechammer, tol2022toward, vanderveen2016drammer_deterministic, vanderveen2018guardion, walker2021ondram, weissman2020jackhammer, xiao2016onebit, yaglikci2022understanding, yang2019trapassisted, yao2020deephammer, yun2018study, zhang2018triggering, zhang2020pthammer, zhang2022implicit, zheng2023trojvit}}

\newcommand{\exploitingRowHammerAllCitations}[0]{\cite{aga2017when, aydin2022cyber, barenghi2018softwareonly, bhattacharya2016curious, bhattacharya2018advanced, bosman2016dedup, brasser2017cant, burleson2016invited, cai2022onthe, carre2018openssl, cohen2022hammerscope, cojocar2019exploiting, cojocar2020arewe, deridder2021smash, fahr2022theeffects, fahrjr2022when, fournaris2017exploiting, france2022modeling, frigo2018grand, frigo2020trrespass, gruss2015rowhammerjs_a, gruss2018another, hassan2021uncovering, hong2019terminal, islam2022signature, jang2017sgxbomb, jattke2022blacksmith, ji2019pinpoint, kaur2022workinprogress, kim2014flipping, kogler2022halfdouble, kwong2020rambleed, lefforge2023reverse, li2022cyberradar, li2023fphammer, lipp2018nethammer, liu2022generating, mus2022jolt, mutlu2017therowhammer, mutlu2019rowhammer_a, orosa2022spyhammer, pessl2016drama_exploiting, poddebniak2018attacking, qiao2016anew, rakin2022deepsteal, razavi2016flip, roohi2022efficient, safari2014rowhammer, seaborn2015exploiting, staudigl2022neurohammer, tatar2018defeating, tatar2018throwhammer, tobah2022spechammer, tol2022toward, tomita2022extracting, vanderveen2016drammer_deterministic, vanderveen2018guardion, wang2022research, weissman2020jackhammer, xiao2016onebit, yang2022sociallyaware, yao2020deephammer, zhang2018triggering, zhang2020pthammer, zhang2022implicit, zheng2023trojvit}}

\newcommand{\trrCitations}[0]{\cite{bennett2021panopticon, devaux2021method, jedec2020jesd2095a, jedec2020jesd794c, lee2014green, micron2016ddr4, yaglikci2021security}}

\newcommand{\understandingRowHammerAllCitations}[0]{\cite{agarwal2018rowhammer_for, baeg2022estimation, cohen2022hammerscope, frigo2020trrespass, gautam2019rowhammering, genssler2022onthe, he2023whistleblower, jiang2021quantifying, khan2018analysis, kim2014flipping, kim2020revisiting, li2014write, lim2017active, lim2018study, luo2023rowpress, mutlu2017therowhammer, mutlu2018rowhammer, mutlu2019rowhammer_a, mutlu2023fundamentally, ni2018write, olgun2023anexperimental, olgun2023dram_bender, orosa2022spyhammer, park2014activeprecharge, park2016experiments, park2016statistical, redeker2002aninvestigation, ryu2017overcoming, walker2021ondram, yang2016suppression, yang2017scanning, yang2019trapassisted, yun2018study, zhou2023doublesided, zhou2024unveiling, zhou2024understanding, li2023understanding}}

\newcommand{\understandingRowHammerNVMCitations}[0]{\cite{agarwal2018rowhammer_for, genssler2022onthe, khan2018analysis, li2014write, ni2018write}}

\newcommand{\understandingRowHammerSimulationCitataions}[0]{\cite{gautam2019rowhammering, jiang2021quantifying, redeker2002aninvestigation, ryu2017overcoming, walker2021ondram, yang2016suppression, yang2017scanning, yang2019trapassisted}}

\newcommand{\mitigatingRowHammerAllCitations}[0]{\cite{aichinger2015ddrmemory, ajorpaz2022evax, apple2015about, arikan2022processor, aweke2016anvil, bains2015method, bains2016distributed, bains2016rowhammer, bennett2021panopticon, bostanci2024comet, brasser2017cant, devaux2021method, didio2023copyonflip, enomoto2022efficient, enterprise2015hpmoonshot, fakhrzadehgan2022safeguard, france2022modeling, france2022reducing, frigo2020trrespass, gautam2019rowhammering, gomez2016dram_rowhammer, greenfield2012throttling, guderamarao2023defending, guha2022criticality, han2021surround, hassan2019crow, hassan2021uncovering, hassan2024acase, hong2023dsac, irazoqui2016mascat, jedec2020jesd794c, jedec2020jesd795, joardar2022learning, joardar2022machine, juffinger2023csirowhammercryptographic, kang2020cattwo, kim2014architectural, kim2014flipping, kim2022mithril, kim2023a11v, konoth2018zebram, lee2019twice, lee2021cryoguard, lenovo2015rowhammer, loughlin2021stop, loughlin2022moesiprime, manzhosov2022revisiting, marazzi2022rega, marazzi2023protrr, mutlu2023fundamentally, naseredini2022alarm, olgun2024abacus, park2020graphene, park2022rowhammer_reduction, qureshi2022hydra, ryu2017overcoming, saileshwar2022randomized, saroiu2022howto, saroiu2022theprice, saxena2022aqua, saxena2023ptguard, seyedzadeh2017counterbased, seyedzadeh2017mitigating, seyedzadeh2018mitigating, sharma2022areview, son2017making, tomita2022extracting, vanderveen2018guardion, vig2018rapid, wi2023shadow, woo2023scalable, yaglikci2021blockhammer, yaglikci2021security, yaglikci2022hira, yang2016suppression, yang2017scanning, you2019mrloc, zhang2020leveraging, zhang2022softtrr, zhou2022ltpim, zhou2023dnndefender}}

\newcommand{\hwBasedRowHammerMitigations}[0]{\cite{aichinger2015ddrmemory, ajorpaz2022evax, apple2015about, arikan2022processor, aweke2016anvil, bains2015method, bains2015rowhammer, bains2016distributed, bains2016rowhammer, bennett2021panopticon, bostanci2024comet, brasser2017cant, devaux2021method, didio2023copyonflip, enomoto2022efficient, enterprise2015hpmoonshot, fakhrzadehgan2022safeguard, france2022modeling, france2022reducing, frigo2020trrespass, gautam2019rowhammering, gomez2016dram_rowhammer, greenfield2012throttling, guderamarao2023defending, guha2022criticality, han2021surround, hassan2019crow, hassan2021uncovering, hassan2024acase, irazoqui2016mascat, joardar2022learning, joardar2022machine, juffinger2023csirowhammercryptographic, kang2020cattwo, kim2014architectural, kim2014flipping, kim2022mithril, kim2023a11v, konoth2018zebram, lee2019twice, lee2021cryoguard, lenovo2015rowhammer, loughlin2021stop, loughlin2022moesiprime, manzhosov2022revisiting, marazzi2023protrr, mutlu2023fundamentally, olgun2024abacus, park2020graphene, park2022rowhammer_reduction, qureshi2022hydra, ryu2017overcoming, saileshwar2022randomized, saroiu2022howto, saroiu2022theprice, saxena2022aqua, saxena2023ptguard, seyedzadeh2017counterbased, seyedzadeh2017mitigating, seyedzadeh2018mitigating, sharma2022areview, son2017making, tomita2022extracting, vanderveen2018guardion, vig2018rapid, wang2021discreetpara, wi2023shadow, woo2023scalable, woo2023scalable, yaglikci2021blockhammer, yaglikci2021security, yaglikci2022hira, yang2016suppression, yang2017scanning, you2019mrloc, zhang2020leveraging, zhang2022softtrr, zhou2022ltpim, zhou2023dnndefender}}



\newcommand{\swBasedRowHammerMitigations}[0]{\cite{aweke2016anvil, bock2019riprh, brasser2017cant, enomoto2022efficient, konoth2018zebram, vanderveen2018guardion, zhang2022softtrr}}



\newcommand{\mcBasedRowHammerMitigations}[0]{\cite{aichinger2015ddrmemory, ajorpaz2022evax, apple2015about, arikan2022processor, aweke2016anvil, bains2015method, bains2016distributed, bains2016rowhammer, brasser2017cant, devaux2021method, didio2023copyonflip, enomoto2022efficient, enterprise2015hpmoonshot, fakhrzadehgan2022safeguard, france2022modeling, france2022reducing, frigo2020trrespass, gautam2019rowhammering, greenfield2012throttling, guderamarao2023defending, guha2022criticality, han2021surround, hassan2021uncovering, hassan2024acase, irazoqui2016mascat, joardar2022learning, joardar2022machine, juffinger2023csirowhammercryptographic, kang2020cattwo, kim2014architectural, kim2014flipping, kim2022mithril, kim2023a11v, konoth2018zebram, lee2019twice, lee2021cryoguard, lenovo2015rowhammer, loughlin2021stop, loughlin2022moesiprime, manzhosov2022revisiting, mutlu2023fundamentally, park2020graphene, park2022rowhammer_reduction, qureshi2022hydra, ryu2017overcoming, saileshwar2022randomized, saroiu2022howto, saroiu2022theprice, saxena2022aqua, saxena2023ptguard, seyedzadeh2017counterbased, seyedzadeh2017mitigating, seyedzadeh2018mitigating, sharma2022areview, son2017making, vanderveen2018guardion, vig2018rapid, wi2023shadow, woo2023scalable, yaglikci2021blockhammer, yaglikci2022hira, yang2017scanning, you2019mrloc, zhang2020leveraging, zhang2022softtrr, zhou2022ltpim, zhou2023dnndefender}}



\newcommand{\inDRAMRowHammerMitigations}[0]{\cite{bennett2021panopticon, gomez2016dram_rowhammer, hassan2019crow, hong2023dsac, jedec2017jesd794b, jedec2020jesd794c, marazzi2022rega, marazzi2023protrr, seyedzadeh2017counterbased, seyedzadeh2017mitigating, seyedzadeh2018mitigating, yaglikci2021security, yang2016suppression}}





\newcommand{\deterministicRowHammerDefenseCitations}[0]{\cite{bains2016rowhammer, kang2020cattwo, kim2014architectural, kim2022mithril, lee2019twice, park2020graphene, saileshwar2022randomized, saxena2022aqua, seyedzadeh2017counterbased, seyedzadeh2017mitigating, seyedzadeh2018mitigating, yaglikci2021blockhammer}}



\newcommand{\probabilisticRowHammerDefenseCitations}[0]{\cite{kim2014flipping, son2017making, you2019mrloc}}



\newcommand{\refreshBasedRowHammerDefenseCitations}[0]{\cite{apple2015about, aweke2016anvil, bains2015method, bains2016distributed, bains2016rowhammer, bostanci2024comet, devaux2021method, enterprise2015hpmoonshot, frigo2020trrespass, hassan2021uncovering, irazoqui2016mascat, joardar2022learning, joardar2022machine, kang2020cattwo, kim2014architectural, kim2014flipping, kim2022mithril, lee2019twice, lenovo2015rowhammer, loughlin2021stop, marazzi2023protrr, olgun2024abacus, park2020graphene, qureshi2022hydra, saroiu2022howto, seyedzadeh2017counterbased, seyedzadeh2017mitigating, seyedzadeh2018mitigating, son2017making, vig2018rapid, wang2021discreetpara, yaglikci2021security, yaglikci2022hira, you2019mrloc, zhang2022softtrr}}



\newcommand{\throttlingBasedRowHammerDefenseCitations}[0]{\cite{greenfield2012throttling, yaglikci2021blockhammer}}



\newcommand{\integrityBasedRowHammerDefenseCitations}[0]{\cite{ajorpaz2022evax, didio2023copyonflip, fakhrzadehgan2022safeguard, guderamarao2023defending, juffinger2023csirowhammercryptographic, manzhosov2022revisiting, saxena2023ptguard}}



\newcommand{\isolationBasedRowHammerDefenseCitations}[0]{\cite{bock2019riprh, brasser2017cant, hassan2019crow, konoth2018zebram, loughlin2021stop, saileshwar2022randomized, saxena2022aqua, vanderveen2018guardion, wi2023shadow, woo2023scalable, woo2023scalable, zhou2023dnndefender}}

\newcommand{\migrationBasedRowHammerDefenseCitations}[0]{\cite{hassan2019crow, saileshwar2022randomized, saxena2022aqua, wi2023shadow, woo2023scalable}}


\newcommand{\circuitBasedRowHammerDefenseCitations}[0]{\cite{gautam2019rowhammering, gomez2016dram_rowhammer, han2021surround, hassan2019crow, hassan2024acase, kim2023a11v, lee2021cryoguard, park2022rowhammer_reduction, ryu2017overcoming, yang2016suppression, yang2017scanning, zhou2022ltpim}}



\newcommand{\detectionOnlyCitations}[0]{\cite{arikan2022processor, france2022reducing, zhang2020leveraging, zhou2022ltpim}}



\newcommand{\surveyCitations}[0]{\cite{aichinger2015ddrmemory, mutlu2023fundamentally, saroiu2022theprice, sharma2022areview}}



\newcommand{\systemImprovementBasedDefenseCitations}[0]{\cite{guha2022criticality, loughlin2021stop, loughlin2022moesiprime}}



\newcommand{\dramStandardCitations}[0]{\cite{jedec2008ddr3, jedec2008jesd79f, jedec2010jesd218, jedec2010jesd219, jedec2012ddr4, jedec2013standard, jedec2014lowpower, jedec2016jesd232a, jedec2020jesd795, jedec2021jesd235d, jedec2021jesd250c, jedec2022high, micron2014sdram, micron2014tn4003}}





\newcommand{\inDRAMRowAddressMappingCitations}[0]{\cite{barenghi2018softwareonly, cojocar2020arewe, horiguchi1997redundancy, itoh2001vlsi, keeth2001dram_circuit, keeth2007dram_circuit, khan2016parbor, khan2017detecting, kim2014flipping, lee2017designinduced, liu2013anexperimental, patel2020bitexact, seshadri2015gatherscatter, smith1981laser, tatar2018defeating}}



\newcommand{\rowHammerGetsWorseCitations}[0]{\cite{cojocar2020arewe, frigo2020trrespass, kim2014flipping, kim2020revisiting, luo2023rowpress, mutlu2017therowhammer, mutlu2018rowhammer, mutlu2019rowhammer_a, mutlu2023fundamentally}}



\newcommand{\rowHammerDefenseScalingProblemsCitations}[0]{\cite{hassan2021uncovering, kim2020revisiting, mutlu2017therowhammer, mutlu2018rowhammer, mutlu2019rowhammer_a, mutlu2023fundamentally, park2020graphene}}



\newcommand{\rhdefinition}[0]{\cite{kim2014flipping, kim2020revisiting, mutlu2017therowhammer, mutlu2019rowhammer_a, park2016experiments, park2016statistical, walker2021ondram, yaglikci2022understanding, yang2019trapassisted}}

\newcommand{\rhdefrefresh}[0]{\cite{apple2015about, aweke2016anvil, bains2015method, bains2016distributed, bains2016rowhammer, devaux2021method, frigo2020trrespass, hassan2021uncovering, joardar2022learning, kang2020cattwo, kim2014architectural, kim2014flipping, kim2022mithril, lee2019twice, lee2021cryoguard, marazzi2023protrr, park2020graphene, qureshi2022hydra, seyedzadeh2017counterbased, seyedzadeh2017mitigating, seyedzadeh2018mitigating, son2017making, yaglikci2021security, you2019mrloc, zhang2022softtrr}}

\newcommand{\rhdef}[0]{\cite{apple2015about, aweke2016anvil, bains2015method, bains2016distributed, bains2016rowhammer, brasser2017cant, frigo2020trrespass, greenfield2012throttling, hassan2021uncovering, joardar2022learning, juffinger2023csirowhammercryptographic, kang2020cattwo, kim2014architectural, kim2014flipping, kim2022mithril, konoth2018zebram, lee2019twice, lee2021cryoguard, marazzi2023protrr, park2020graphene, qureshi2022hydra, saileshwar2022randomized, seyedzadeh2017counterbased, seyedzadeh2017mitigating, seyedzadeh2018mitigating, son2017making, vanderveen2018guardion, yaglikci2021blockhammer, yaglikci2021security, you2019mrloc, zhang2022softtrr}}

\newcommand{\perrefreshscaling}[0]{\cite{baumann2005radiationinduced, chang2014improving, kang2014coarchitecting, liu2012raidr, liu2013anexperimental, mukundan2013understanding, nair2013archshield, nair2014refresh, nguyen2018nonblocking}}

\newcommand{\rhsafe}[0]{\cite{frigo2020trrespass, lee2014green, micron2014sdram}}

\newcommand{\rhworse}[0]{\cite{deridder2021smash, frigo2020trrespass, hassan2021uncovering, jattke2022blacksmith, kim2014flipping, kim2020revisiting, mutlu2017therowhammer, mutlu2019rowhammer_a, orosa2021adeeper, yaglikci2022understanding}}

\newcommand{\rhdefworse}[0]{\cite{hassan2021uncovering, kim2020revisiting, orosa2021adeeper, park2020graphene, qureshi2022hydra, yaglikci2021blockhammer, yaglikci2021security}}

\newcommand{\rhattacks}[0]{\cite{aga2017when, bhattacharya2016curious, bosman2016dedup, brasser2017cant, burleson2016invited, cojocar2019exploiting, cojocar2020arewe, deridder2021smash, frigo2018grand, frigo2020trrespass, gruss2015rowhammerjs_a, gruss2018another, hassan2021uncovering, hong2019terminal, jang2017sgxbomb, jattke2022blacksmith, ji2019pinpoint, kim2014flipping, kogler2022halfdouble, kwong2020rambleed, lipp2018nethammer, mutlu2017therowhammer, mutlu2019rowhammer_a, pessl2016drama_exploiting, qiao2016anew, razavi2016flip, safari2014rowhammer, seaborn2015exploiting, tatar2018defeating, tol2022toward, vanderveen2016drammer_deterministic, vanderveen2018guardion, weissman2020jackhammer, xiao2016onebit, yao2020deephammer, zhang2020pthammer}}

\newcommand{\salprefs}[0]{\cite{chang2014improving, kim2012acase, wang2020figaro, zhang2014cream}}

